Vertex Lattice Models Simulated with Quantum Circuits

Classical planar vertex models afford transfer matrices with real and positive entries, which makes this class of models suitable for quantum simulations. In this work, we support this statement by building explicit quantum circuits that implement the actions of the transfer matrices on arbitrary many-qubit states. The number of qubits and the depth of the circuits grow linearly with the size of the system. Furthermore, we present tests using quantum simulators and demonstrate that important physical quantities can be extracted, such as the eigen-vector corresponding to the largest eigenvalue of the transfer matrix and the ratio of the second to first largest eigenvalue. Challenges steaming from the non-unitarity of the transfer matrix are discussed.

==> yquant-circuit.tex <==
% BEGIN_FOLD Drawing wires
% extends the wire of register #1. Assumes a node called yquantbox is set up, and the \pgfshapeclippathhorzresult was set up appropriately for this node.
\protected\def\yquant@circuit@extendwire#1#2{%
   \begingroup%
      \ifx*#2%
         \edef\wirexpos{\the\dimen0}%
      \else%
         \pgfpointanchor{yquantbox}{#2}%
         \edef\wirexpos{\the\pgf@x}%
      \fi%
      \ifdim\wirexpos>0pt % may be negative for init gates
         \yquant@register@get@typeywire{#1}\wiretype\wireypos\wirelast%
         \edef\wirexprevpos{\expandafter\@firstoffour\wirelast}%
         \ifnum\wiretype=\yquant@register@type@none%
            % the clippings of the previous operator will for sure not be needed, but the type might be turned into an active one, so we need the last clipping.
            \yquant@register@set@lastwire{#1}{%
               {\wirexprevpos}{\wirexpos}{}%
               {\unexpanded\expandafter{\pgfshapeclippathhorzresult}}%
            }%
         \else%
            % append the previous `last' clipping to the old list and insert the new one
            \yquant@register@set@lastwire{#1}{%
               {\wirexprevpos}{\wirexpos}%
               {\unexpanded\expandafter\expandafter\expandafter{%
                   \expandafter\@thirdandfourthoffour\wirelast%
                }%
               }%
               {\unexpanded\expandafter{\pgfshapeclippathhorzresult}}%
            }%
         \fi%
      \fi%
   \endgroup%
}

% finishes the wires of all registers
\protected\def\yquant@circuit@endwires{%
   \expandafter\expandafter\expandafter\yquant@register@get@maxxrange%
      \expandafter\expandafter\expandafter\yquant@circuit@endwires@x%
      \expandafter\expandafter\expandafter1%
      \expandafter\expandafter\expandafter{\csname\yquant@prefix registers\endcsname}%
   % to have a symmetric situation, we extend again one separation at the end, unless this is supposed to be seamless and we don't have outputs (for seamless circuits with outputs, extend - since this extension will be between last register and output)
   \ifyquant@env@seamless{%
      \expandafter\unless\expandafter\ifx\csname\yquant@prefix outputs\endcsname\relax%
         \dimdef\yquant@circuit@endwires@x{\yquant@circuit@endwires@x+\yquant@config@operator@sep}%
      \fi%
   }{%
      \dimdef\yquant@circuit@endwires@x{\yquant@circuit@endwires@x+\yquant@config@operator@sep}%
   }%
   \let\yquant@circuit@endwires@finalize=\relax%
   \yquant@for \yquant@circuit@endwires@i := 1 to \csname\yquant@prefix registers\endcsname {%
      % we only extend the wire if it does not come from the outer circuit - this one would be responsible for the extension.
      \ifcsname\yquant@prefix registermap@\yquant@circuit@endwires@i\endcsname%
         \xifinlistcs\yquant@circuit@endwires@i{\yquant@prefix inonly}{%
            % however, the wire is to be discarded after this circuit
            \edef\storedleft{\the\pgf@picminx}%
            \yquant@draw@wire\yquant@circuit@endwires@i1%
            \global\pgf@picminx=\storedleft%
            \eappto\yquant@circuit@endwires@finalize{%
               \yquant@register@set@type%
                  \yquant@circuit@endwires@i\noexpand\yquant@register@type@none%
            }%
         }\relax%
      \else%
         \yquant@draw@wire\yquant@circuit@endwires@i1%
      \fi%
   }%
}

% outputs the wire according to its previous instructions and prepares for a change in the wire style
\protected\def\yquant@circuit@flushwire#1{%
   \yquant@draw@wire{#1}0%
   \begingroup%
      \yquant@register@get@lastwire{#1}\wirelast%
      \yquant@register@set@lastwire{#1}{%
         {\expandafter\@secondoffour\wirelast}{\expandafter\@secondoffour\wirelast}{}%
         {\unexpanded\expandafter\expandafter\expandafter{%
             \expandafter\@fourthoffour\wirelast%
          }}%
      }%
   \endgroup%
}
% END_FOLD

% BEGIN_FOLD Drawing control lines
% populates a drawing macro with the current control line with style #1 at position #2. Assumes a node called yquantbox is set up, and the \pgfshapeclippathvertresult was set up appropriately for this node. At the first call, \yquant@circuit@extendcontrolline@cmd must be \let to \empty and \yquant@circuit@extendcontrolline@prev to \relax.
\protected\def\yquant@circuit@extendcontrolline#1#2{%
   \eappto\yquant@circuit@extendcontrolline@clip{%
      \unexpanded\expandafter{\pgfshapeclippathvertresult}%
   }%
   \begingroup%
      \tikzset{/yquant/every control line}%
      \expandafter%
   \endgroup%
   \expandafter\@tempdima\the\pgflinewidth%
   \ifcase#1%
      % no control (or to a discarded target, which we don't do)
   \or%
      % qubit
      \pgfpointanchor{yquantbox}{center}%
      \unless\ifx\yquant@circuit@extendcontrolline@prev\relax%
         \eappto\yquant@circuit@extendcontrolline@cmd{%
            \expandafter\@secondofthree\yquant@circuit@extendcontrolline@prev%
            -- (#2,\the\pgf@y)%
         }%
      \fi%
      \yquant@circuit@extendcontrolline@store{#2}%
   \or%
      % cbit
      \pgfpointanchor{yquantbox}{center}%
      \unless\ifx\yquant@circuit@extendcontrolline@prev\relax%
         \eappto\yquant@circuit@extendcontrolline@cmd{%
            \expandafter\@firstofthree\yquant@circuit@extendcontrolline@prev%
            -- (\the\dimexpr#2-2\@tempdima\relax,\the\pgf@y)%
            \expandafter\@thirdofthree\yquant@circuit@extendcontrolline@prev%
            -- (\the\dimexpr#2+2\@tempdima\relax,\the\pgf@y)%
         }%
      \fi%
      \yquant@circuit@extendcontrolline@store{#2}%
   \or%
      % quantum-bundle (very unusual, but perhaps for transversal operations?)
      \pgfpointanchor{yquantbox}{center}%
      \unless\ifx\yquant@circuit@extendcontrolline@prev\relax%
         \eappto\yquant@circuit@extendcontrolline@cmd{%
            \expandafter\@firstofthree\yquant@circuit@extendcontrolline@prev%
            -- (\the\dimexpr#2-2\@tempdima\relax,\the\pgf@y)%
            \expandafter\@secondofthree\yquant@circuit@extendcontrolline@prev%
            -- (\the\dimexpr#2\relax,\the\pgf@y)%
            \expandafter\@thirdofthree\yquant@circuit@extendcontrolline@prev%
            -- (\the\dimexpr#2+2\@tempdima\relax,\the\pgf@y)%
         }%
      \fi%
      \yquant@circuit@extendcontrolline@store{#2}%
   \else%
      \PackageError{yquant.sty}{Invalid control line type `#1'}%
                   {yquant encountered an internal error.}%
   \fi%
}

\protected\def\yquant@circuit@extendcontrolline@store#1{%
   \edef\yquant@circuit@extendcontrolline@prev{%
      {(\the\dimexpr#1-2\@tempdima\relax,\the\pgf@y)}%
      {(\the\dimexpr#1\relax,\the\pgf@y)}%
      {(\the\dimexpr#1+2\@tempdima\relax,\the\pgf@y)}%
   }%
}

% populates a drawing macro with the multi operation connector at position #2. Assumes a node called yquantbox is set up, and the \pgfshapeclippathvertresult was set up appropriately for this node. At the first call, \yquant@circuit@extendmultiline@cmd must be \let to \empty and \yquant@circuit@extendmultiline@prev to \relax.
\protected\def\yquant@circuit@extendmultiline#1{%
   \begingroup%
      \tikzset{/yquant/every multi line}%
      \expandafter%
   \endgroup%
   \eappto\yquant@circuit@extendmultiline@clip{%
      \unexpanded\expandafter{\pgfshapeclippathvertresult}%
   }%
   \expandafter\@tempdima\the\pgflinewidth%
   \pgfpointanchor{yquantbox}{center}%
   \unless\ifx\yquant@circuit@extendmultiline@prev\relax%
      \eappto\yquant@circuit@extendmultiline@cmd{%
         \yquant@circuit@extendmultiline@prev -- (#1,\the\pgf@y)%
      }%
   \fi%
   \edef\yquant@circuit@extendmultiline@prev{%
      (\the\dimexpr#1\relax,\the\pgf@y)%
   }%
}
% END_FOLD

\newif\ifyquant@circuit@operator@hasControls%
% sets up the relevant variables associated with an operator
% #1: positive controls
% #2: negative controls
% #3: targets
\protected\def\yquant@circuit@operator#1#2#3{%
   % convert all names to indices
   % targets
   \yquant@register@get@ids{#3}%
   \let\yquant@circuit@operator@targets=\yquant@register@get@ids@list%
   \let\yquant@circuit@operator@mintarget=\yquant@register@get@ids@min%
   \let\yquant@circuit@operator@maxtarget=\yquant@register@get@ids@max%
   \let\yquant@circuit@operator@numtarget=\yquant@register@get@ids@count%
   % make sure to reset this for subcircuits
   \yquant@circuit@operator@hasControlsfalse%
   % For the targets, multi-qubit registers might have been allowed, but certainly not for
   % the controls!
   \yquant@register@get@allowmultifalse%
   % positive controls
   \yquant@register@get@ids{#1}%
   \let\yquant@circuit@operator@pctrls=\yquant@register@get@ids@list%
   \let\yquant@circuit@operator@minpctrl=\yquant@register@get@ids@min%
   \let\yquant@circuit@operator@maxpctrl=\yquant@register@get@ids@max%
   \let\yquant@circuit@operator@numpctrl=\yquant@register@get@ids@count%
   \ifnum\yquant@register@get@ids@count>0 %
      \yquant@circuit@operator@hasControlstrue%
   \fi%
   % negative controls
   \yquant@register@get@ids{#2}%
   \let\yquant@circuit@operator@nctrls=\yquant@register@get@ids@list%
   \let\yquant@circuit@operator@minnctrl=\yquant@register@get@ids@min%
   \let\yquant@circuit@operator@maxnctrl=\yquant@register@get@ids@max%
   \let\yquant@circuit@operator@numnctrl=\yquant@register@get@ids@count%
   \ifnum\yquant@register@get@ids@count>0 %
      \yquant@circuit@operator@hasControlstrue%
   \fi%
   % determine the qubits spanned
   \yquant@min\yquant@circuit@operator@minctrl%
      \yquant@circuit@operator@mintarget%
      \yquant@circuit@operator@minpctrl%
      \yquant@circuit@operator@minnctrl%
      \relax%
   \yquant@max\yquant@circuit@operator@maxctrl%
      \yquant@circuit@operator@maxtarget%
      \yquant@circuit@operator@maxpctrl%
      \yquant@circuit@operator@maxnctrl%
      \relax%
}

% restores the data captured for an uncontrolled operator and starts preparation
% #1: \yquant@attrs@remaining
% #2: \yquant@circuit@operator@targets
% #3: \yquant@circuit@operator@mintarget
% #4: \yquant@circuit@operator@maxtarget
% #5: \yquant@circuit@operator@numtarget
\protected\def\yquant@circuit@restore#1#2#3#4#5{%
   \def\yquant@attrs@remaining{#1}%
   \def\yquant@circuit@operator@targets{#2}%
   \def\yquant@circuit@operator@mintarget{#3}%
   \def\yquant@circuit@operator@maxtarget{#4}%
   \def\yquant@circuit@operator@numtarget{#5}%
   \yquant@circuit@operator@hasControlsfalse%
   \let\yquant@circuit@operator@pctrls=\empty%
   \def\yquant@circuit@operator@minpctrl{2147483647}%
   \def\yquant@circuit@operator@maxpctrl{0}%
   \let\yquant@circuit@operator@numpctrl=\yquant@circuit@operator@maxpctrl%
   \let\yquant@circuit@operator@nctrls=\empty%
   \let\yquant@circuit@operator@minnctrl=\yquant@circuit@operator@minpctrl%
   \let\yquant@circuit@operator@maxnctrl=\yquant@circuit@operator@maxpctrl%
   \let\yquant@circuit@operator@numnctrl=\yquant@circuit@operator@numpctrl%
   \let\yquant@circuit@operator@minctrl=\yquant@circuit@operator@mintarget%
   \let\yquant@circuit@operator@maxctrl=\yquant@circuit@operator@maxtarget%
}

% creates a subcircuit. Parameter registers must be filled in \yquant@circuit@subcircuit@params.
% #1: style
\protected\def\yquant@circuit@subcircuit#1{%
   \numdef\yquant@circuit@subcircuit@id{\yquant@env+1}%
   \listcsxadd{\yquant@prefix subcircuits}{\yquant@circuit@subcircuit@id}%
   \begingroup%
      \tikzset{/yquant/every operator, #1,%
               /yquant/this operator, /yquant/operators/this subcircuit box/.style={}}%
      % execute the subcircuit
      \expandafter%
      \yquant@env@begin@noarg%
         \yquant@lang@attr@value% this contains the subcircuit's content
         \expandafter\unless\expandafter\ifx\csname\yquant@prefix parameters\endcsname\empty%
            \PackageError{yquant.sty}{Invalid subcircuit parameters count}%
                         {Too many parameters given.}%
         \fi%
      \yquant@env@end%
   \endgroup%
}

% BEGIN_FOLD Helpers for operator callbacks
% turn a wire into a different type
\def\yquant@circuit@settype#1{%
   \unless\if\yquant@register@get@type{#1}\yquant@circuit@settype@to %
      \yquant@circuit@flushwire{#1}%
      \yquant@register@set@type{#1}{\yquant@circuit@settype@to}%
   \fi%
}

\protected\def\yquant@circuit@settype@prepare#1{%
   \yquant@register@set@type{#1}{\yquant@circuit@settype@to}%
}

\protected\long\def\yquant@circuit@setstyle#1#2{%
   \yquant@circuit@flushwire{#1}%
   \yquant@register@set@style{#1}{#2}%
}

\protected\long\def\yquant@circuit@addstyle#1#2{%
   \yquant@circuit@flushwire{#1}%
   \yquant@register@set@style{#1}{\yquant@register@get@style{#1},#2}%
}

% performs an alignment of all registers specified in the argument; that is, the next operation on any of the listed registers will be after the maximum position of all of them
% #1: arbitrary register list
\protected\def\yquant@circuit@align#1{%
   \csxappto{\yquant@prefix draw}{%
      \yquant@draw@hspace{#1}{0pt}%
   }%
}

% introduces a horizontal skip (= invisible operator of given width) among the registers; that is, those registers are first aligned, then skipped by the given amount.
% #1: arbitrary register list
% #2: skip width
\protected\def\yquant@circuit@hspace#1#2{%
   \csxappto{\yquant@prefix draw}{%
      \yquant@draw@hspace{#1}{#2}%
   }%
}

% applies an action to wires a list of registers and causes them to be redrawn
% #1: action for prepare
% #2: action for draw
% #3: arbitrary register list
% #4: parameter(s)
\protected\def\yquant@circuit@actonwires#1#2#3#4{%
   \begingroup%
      \let\tmp=\empty%
      \def\do##1{%
         % We do not extend the wire: a register that is discarded somewhere does not make
         % sense, only right after some application (which is supposed to already have
         % extended the wire appropriately).
         \eappto\tmp{#2{##1}#4}%
         #1{##1}#4%
      }%
      \dolistloop{#3}%
      \csxappto{\yquant@prefix draw}{\tmp}%
   \endgroup%
}

% sets the output of wires
% #1: arbitrary register list
\protected\def\yquant@circuit@output{%
   \protected\def\idx{}%
   \protected@csxappto{\yquant@prefix outputs}%
            {\yquant@circuit@restore%
               {\yquant@attrs@remaining}%
               {\unexpanded\expandafter{\yquant@circuit@operator@targets}}%
               {\yquant@circuit@operator@mintarget}{\yquant@circuit@operator@maxtarget}%
               {\yquant@circuit@operator@numtarget}%
             \yquant@prepare{\yquant@lang@attr@value}{}%
            }%
}
% END_FOLD

==> yquant-config.tex <==
\pgfdeclaremetadecoration{tikz@internal}{pre}{%
   \state{pre}[width=\pgfkeysvalueof{/pgf/decoration/pre length}+\pgfkeysvalueof{/pgf/decoration/post length}, next state=main]{%
      \appto\tikz@dec@shift{\pgftransformxshift{-\pgfkeysvalueof{/pgf/decoration/post length}}}%
      \tikz@dec@trans%
      \decoration{\pgfkeysvalueof{/pgf/decoration/pre}}%
   }%
   \state{main}[width=\pgfmetadecoratedremainingdistance, next state=final]{%
      \tikz@dec@trans%
      \decoration{\tikz@decoration@name}%
   }%
   \state{final}{%
      \tikz@dec@trans%
      \decoration{\pgfkeysvalueof{/pgf/decoration/post}}%
   }%
}

% BEGIN_FOLD Circuit layout
\ifnum\yquant@compat<2 %
   \pgfqkeys{/yquant}{%
      register/minimum height/.code=%
         {\dimdef\yquant@config@register@minimum@height{.5\dimexpr#1\relax}%
          \let\yquant@config@register@minimum@depth=\yquant@config@register@minimum@height}%
   }
\else%
   \pgfqkeys{/yquant}{%
      register/minimum height/.code=%
         {\dimdef\yquant@config@register@minimum@height{#1}},%
      register/minimum depth/.code=%
         {\dimdef\yquant@config@register@minimum@depth{#1}}%
   }
\fi
\pgfqkeys{/yquant}{%
   register/separation/.code=%
      {\dimdef\yquant@config@register@sep{#1}},%
   operator/minimum width/.code=%
      {\dimdef\yquant@config@operator@minimum@width{#1}},%
   operator/separation/.code=%
      {\dimdef\yquant@config@operator@sep{#1}},%
   operator/multi warning/.is if=%
      yquant@config@operator@multi@warn%
}%
% END_FOLD
% BEGIN_FOLD Register creation
\pgfqkeys{/yquant}{%
   register/default name/.store in=%
      \yquant@config@register@default@name%
}
\ifnum\yquant@compat<2 %
   \pgfqkeys{/yquant}{%
      every label/.style=%
         {shape=yquant-init, anchor=center, align=right, outer xsep=2pt},%
      every multi label/.style=%
         {draw, decoration={gapped brace, mirror, raise=2pt}, decorate}%
   }
\else
   \pgfqkeys{/yquant}{%
      every label/.style=%
         {shape=yquant-init, anchor=center, align=right, outer xsep=2pt,%
          /yquant/operator/if multi={draw, decoration={gapped brace, mirror, raise=2pt}, decorate}}%
    }
\fi
\pgfqkeys{/yquant}{
   every initial label/.style=%
      {anchor=east},%
   every qubit label/.style=%
      {},%
   every cbit label/.style=%
      {},%
   every qubits label/.style=%
      {}%
}
\ifnum\yquant@compat<2 %
   \pgfqkeys{/yquant}{%
      every input label/.style=%
         {}%
   }%
\fi%
% END_FOLD
% BEGIN_FOLD Register outputs
\ifnum\yquant@compat<2 %
   \pgfqkeys{/yquant}{%
      every output/.style=%
         {shape=yquant-output, anchor=west, align=left, outer xsep=2pt},%
      every multi output/.style=%
         {draw, decoration={gapped brace, raise=2pt}, decorate}%
   }
\else
   \pgfqkeys{/yquant}{%
      every output/.style=%
         {shape=yquant-output, anchor=west, align=left, outer xsep=2pt,%
          /yquant/operator/if multi={draw, decoration={gapped brace, raise=2pt}, decorate}}%
   }
\fi
\pgfqkeys{/yquant}{%
   every qubit output/.style=%
      {},%
   every cbit output/.style=%
      {},%
   every qubits output/.style=%
      {}%
}
% END_FOLD
% BEGIN_FOLD General styling
\pgfqkeys{/yquant}{%
   every circuit/.style={%
      every node/.prefix style={transform shape}
   }%
}
\@ifpackagelater{pgf}{2020/09/31}\relax{
   \pgfkeys{/yquant/every circuit/.append style={%
      every label/.prefix style={transform shape=false}%
   }}
}
\pgfqkeys{/yquant}{%
   every wire/.style=%
      {draw},%
   every qubit wire/.style=%
      {},%
   every cbit wire/.style=%
      {},%
   every qubits wire/.style=%
      {},%
   every control line/.style=%
      {draw},%
   every control/.style=%
      {shape=yquant-circle, anchor=center, radius=.5mm},%
   every positive control/.style=%
      {fill=black},%
   every negative control/.style=%
      {draw},%
   every operator/.style=%
      {anchor=center},%
   every multi line/.style=%
      {draw, decoration={snake, amplitude=.25mm, segment length=5pt}, decorate},%
   this operator/.style=%
      {},%
   this control/.style=%
      {},%
   operator style/.style=%
      {/yquant/this operator/.append style={#1}},%
   control style/.style=%
      {/yquant/every control line/.append style={#1},%
       /yquant/this control/.append style={#1}},%
   style/.style=%
      {/yquant/this operator/.append style={#1},%
       /yquant/every control line/.append style={#1},%
       /yquant/this control/.append style={#1}},%
   operator/multi as single/.style=%
      {/yquant/every multi line/.style=/yquant/every control line},%
   operator/if multi/.code=%
      {\ifyquant@config@operator@multi\pgfkeysalso{#1}\fi},%
   circuit/seamless/.is if=yquant@config@circuit@seamless,%
   every post measurement control/.is choice,
   every post measurement control/indirect/.code={%
      \undef\yquant@lang@attr@directcontrol%
   },%
   every post measurement control/direct/.code={%
      \let\yquant@lang@attr@directcontrol=\relax%
   }%
}
% END_FOLD
% BEGIN_FOLD Styles for operators
\ifnum\yquant@compat<2 %
   \pgfqkeys{/yquant}{%
      operators/every barrier/.style=%
         {shape=yquant-line, dashed, draw}%
   }
\else
   \pgfqkeys{/yquant}{%
      operators/every barrier/.style=%
         {shape=yquant-line, dashed, draw, shorten <= -1mm, shorten >= -1mm}
   }
\fi
\pgfqkeys{/yquant}{%
   operators/every box/.style=%
      {shape=yquant-rectangle, draw, align=center, inner xsep=1mm, x radius=2mm, y radius=2.47mm},%
}
\ifnum\yquant@compat<2 %
   \pgfqkeys{/yquant}{%
      operators/every custom gate/.style=%
         {/yquant/operators/subcircuit/frameless, /yquant/register/default name=}%
   }
\else
   \pgfqkeys{/yquant}{%
      operators/every custom gate/.style=%
         {/yquant/operators/subcircuit/seamless}%
   }
\fi
\pgfqkeys{/yquant}{%
   operators/every dmeter/.style=%
      {shape=yquant-dmeter, x radius=2mm, y radius=2mm, draw},
   % every h is implicitly defined during gate declaration
   operators/every inspect/.style=%
      {shape=yquant-output, align=left, outer xsep=.3333em, y radius=2.47mm,%
       /yquant/operator/if multi={draw, decoration={gapped brace, raise=2pt}, decorate}},%
   operators/every measure/.style=%
      {shape=yquant-measure, x radius=4mm, y radius=2.5mm, draw},%
   operators/every measure meter/.style=%
      {draw, -{Latex[length=2.5pt]}},%
   operators/every not/.style=%
      {shape=yquant-oplus, radius=1.3mm, draw},%
   operators/every pauli/.style=%
      {/yquant/operators/every box},%
   operators/every phase/.style=%
      {shape=yquant-circle, radius=.5mm, fill},%
   operators/every slash/.style=%
      {shape=yquant-slash, x radius=.5mm, y radius=.7mm, draw},%
   operators/every subcircuit/.style=%
      {},%
   operators/every subcircuit box/.style=%
      {/yquant/operators/every box},%
   subcircuit box style/.style=%
      {/yquant/operators/every subcircuit box/.append style={#1}},%
   operators/this subcircuit box/.style=%
      {},%
   this subcircuit box style/.style=%
      {/yquant/operators/this subcircuit box/.append style={#1}},%
   operators/subcircuit/frameless/.style=
      {/yquant/operators/this subcircuit box/.append style={draw=none, inner sep=0pt}},%
   operators/subcircuit/seamless/.code=%
      {\pgfkeysalso{/yquant/operators/subcircuit/frameless, /yquant/register/default name=}%
       \letcs\yquant@prevseamless{\yquant@prefix seamless}%
       \yquant@config@circuit@seamlesstrue},
   operators/subcircuit/name mangling/.is choice,%
   operators/subcircuit/name mangling/prefix or discard/.code=%
      {\def\yquant@config@operator@subcircuit@mangling{0}},%
   operators/subcircuit/name mangling/prefix or transparent/.code=%
      {\def\yquant@config@operator@subcircuit@mangling{1}},%
   operators/subcircuit/name mangling/transparent/.code=%
      {\def\yquant@config@operator@subcircuit@mangling{2}},%
   operators/subcircuit/name mangling/discard/.code=%
      {\def\yquant@config@operator@subcircuit@mangling{3}},%
   operators/subcircuit/name mangling reset/.is if=%
      yquant@config@operator@subcircuit@manglingreset,
   operators/every swap/.style=%
      {shape=yquant-swap, radius=.75mm, draw},%
   operators/every wave/.style=%
      {shape=yquant-circle, radius=.5mm, fill},%
   % every x is implicitly defined during gate declaration
   operators/every xx/.style=%
      {shape=yquant-rectangle, radius=.75mm, draw},%
   % every y is implicitly defined during gate declaration
   % every z is implicitly defined during gate declaration
   operators/every zz/.style=%
      {shape=yquant-circle, radius=.5mm, fill},%
}
% END_FOLD
% BEGIN_FOLD Internal styles (undocument, do not use!)
\pgfqkeys{/yquant}{%
   internal/move label/.code=%
      {\yquant@config@operator@position@rightaligntrue},
   internal/no advance/.code=%
      {\unless\ifyquantmeasuring% We don't draw subcircuits during measuring time, but we need their advancement
          \yquant@config@operator@position@advancefalse%
       \fi},
   internal/multi main/.is if=%
      yquant@config@internal@multi@main,%
}
\ifnum\yquant@compat<2 %
   \pgfqkeys{/yquant}{%
      internal/squeeze slash/.code=%
         {\dimdef\yquant@config@operator@sep{.5\dimexpr\yquant@config@operator@sep-\pgflinewidth\relax}%
          \yquant@config@operator@position@advancefalse},%
   }
\else%
   \pgfqkeys{/yquant}{%
      internal/squeeze slash/.code={}%
   }
\fi
% END_FOLD

\def\yquant@config@register@default@name{\regidx}
\def\yquant@config@register@minimum@height{1.5mm}
\def\yquant@config@register@minimum@depth{1.5mm}
\def\yquant@config@register@sep{1mm}
\def\yquant@config@operator@sep{1mm}
\def\yquant@config@operator@minimum@width{5mm}
\newif\ifyquant@config@internal@multi@main%
\yquant@config@internal@multi@maintrue
\newif\ifyquant@config@operator@multi@warn
\yquant@config@operator@multi@warntrue
\newif\ifyquant@config@operator@position@rightalign
\newif\ifyquant@config@operator@position@advance
\yquant@config@operator@position@advancetrue
\newif\ifyquant@config@circuit@seamless
\def\yquant@config@operator@subcircuit@mangling{0}
\newif\ifyquant@config@operator@subcircuit@manglingreset
\yquant@config@operator@subcircuit@manglingresettrue
\newif\ifyquant@config@operator@multi

\protected\def\yquant@config@operator@subcircuit@mangling@set#1{%
   \ifyquant@config@operator@subcircuit@manglingreset%
      \def\yquant@config@operator@subcircuit@mangling{#1}%
   \fi%
}

==> yquant-draw.tex <==
\newcount\yquant@draw@@currentcontroltype%

\protected\def\yquant@draw@init#1#2{%
   \ifcsname\yquant@prefix registermap@#1\endcsname%
      % for connected subcircuit wires, check if this actually changes the type [happens for formerly discarded output wires] and flush the wire if necessary
      \edef\yquant@draw@init@type{\yquant@register@get@type{#1}}%
      \unless\if\yquant@draw@init@type#2\relax%
         \yquant@circuit@flushwire{#1}%
         \ifx\yquant@draw@init@type\yquant@register@type@none%
            % in case the wire was discarded before, forget about the lastx position, it should always start with the others
            \yquant@register@get@lastwire{#1}\wirelast%
            \yquant@register@set@lastwire{#1}{%
               {\yquant@draw@subcircuit@wirestart}{\yquant@draw@subcircuit@wirestart}{}%
               {\unexpanded\expandafter\expandafter\expandafter{%
                   \expandafter\@fourthoffour\wirelast%
                }}%
            }%
         \fi%
         \yquant@register@set@type{#1}{#2}%
      \fi%
   \else%
      % for new wires, reset the type, and if this a subcircuit, put the appropriate x position in place. It might have changed from its initial value during preparation stage
      \yquant@register@set@type{#1}{#2}%
      \ifdefined\yquant@draw@subcircuit@wirestart%
         \yquant@register@set@x{#1}{\yquant@draw@subcircuit@wirestart}%
         \yquant@register@set@lastwire{#1}{%
            {\yquant@draw@subcircuit@wirestart}{\yquant@draw@subcircuit@wirestart}{}{}%
         }%
      \fi%
   \fi%
}

\def\yquant@draw@subcircuit@leftpos{0pt}% outermost circuit: 0pt
\protected\long\def\yquant@draw@group#1#2#3#4#5#6{%
   \begingroup%
      \yquant@register@get@maxxlist\yquant@draw@@x{#6}%
      \ifx F#2%
         \yquant@draw@@currentcontroltype=0 %
      \else%
         \yquant@draw@@currentcontroltype=#2 %
      \fi%
      \let\yquant@circuit@extendcontrolline@cmd=\empty%
      \let\yquant@circuit@extendcontrolline@prev=\relax%
      \let\yquant@circuit@extendcontrolline@clip=\empty%
      \let\yquant@circuit@extendmultiline@total=\empty%
      \def\yquant@draw@@width{#1}%
      \def\yquant@draw@@style{#4}%
      \def\yquant@draw@@content{#5}%
      \def\yquant@draw@@idx@content{0}%
      \def\yquant@draw@@idx@pcontrol{0}%
      \def\yquant@draw@@idx@ncontrol{0}%
      % If the quotes library is loaded, activate it. (else, this is by default \relax)
      \tikz@enable@node@quotes%
      \yquant@config@operator@position@rightalignfalse%
      \yquant@config@operator@position@advancetrue%
      \yquant@set{#3}%
      % if the operator is right-aligned, we will not advance, as we must assume that the x position is already chosen appropriately
      \ifyquant@config@operator@position@rightalign%
         % for rightalign, we instead overwrite the lastx configurations, so that the outgoing wire starts after the operator.
         \forlistloop\yquant@draw@group@rightadvance{#6}%
      \else%
         \ifyquant@env@seamless{%
            \unless\ifdim\yquant@draw@@x=\yquant@draw@subcircuit@leftpos%
               \dimdef\yquant@draw@@x{%
                  \yquant@draw@@x+\yquant@config@operator@sep%
               }%
            \fi%
         }{%
            \dimdef\yquant@draw@@x{%
               \yquant@draw@@x+\yquant@config@operator@sep%
            }%
         }%
         \ifyquant@config@operator@position@advance%
            \dimdef\newx{\yquant@draw@@x+#1}%
            \forlistloop\yquant@draw@group@advance{#6}%
         \fi%
         \dimdef\yquant@draw@@x{\yquant@draw@@x+.5\dimexpr#1\relax}%
      \fi%
}

\protected\def\yquant@draw@group@advance#1{%
   \yquant@register@set@x{#1}\newx%
}

\protected\def\yquant@draw@group@rightadvance#1{%
   \ifcsname\yquant@prefix registermap@#1\endcsname%
      % for connected subcircuit wires, make sure to flush the wire until the beginning.
      \yquant@circuit@flushwire{#1}%
   \fi%
}

\protected\def\yquant@draw@endgroup#1#2#3{%
      \unless\ifx F#1%
         \yquant@draw@cline%
      \fi%
      \ifcase#3\relax%
      \or%
         \yquant@draw@alias@ctrl{#2}n%
      \or%
         \yquant@draw@alias@ctrl{#2}p%
      \or%
         \yquant@draw@alias@ctrl{#2}p%
         \yquant@draw@alias@ctrl{#2}n%
      \or%
         \yquant@draw@alias{#2}%
      \or%
         \yquant@draw@alias{#2}%
         \yquant@draw@alias@ctrl{#2}n%
      \or%
         \yquant@draw@alias{#2}%
         \yquant@draw@alias@ctrl{#2}p%
      \or%
         \yquant@draw@alias{#2}%
         \yquant@draw@alias@ctrl{#2}p%
         \yquant@draw@alias@ctrl{#2}n%
      \fi%
      \yquant@circuit@extendmultiline@total%
   \endgroup%
}

\protected\def\yquant@draw@injectiongroup#1#2\yquant@draw@endinjectiongroup#3#4#5{%
   \csdef{yquant@draw@@injection@#1}{%
      \yquant@draw@begininjection#2\yquant@draw@stopinjection{#3}{#4}{#5}%
   }%
}

\protected\long\def\yquant@draw@begininjection#1#2#3#4#5#6{%
   % this is called within another draw group, so lots of things are already set up
   \begingroup%
      \def\yquant@draw@@style{#4}%
      \def\yquant@draw@@content{#5}%
      \let\yquant@draw@@idx@content=\yquant@draw@@idx@pcontrol%
      \yquant@set{#3}% this will accumulate with outer styles from the enclosing draw group, but there is nothing we can do about it
}

\protected\def\yquant@draw@stopinjection#1#2#3{%
   \ifcase#3\relax%
   \or%
      \yquant@draw@alias@ctrl{#2}n%
   \or%
      \yquant@draw@alias@ctrl{#2}p%
   \or%
      \yquant@draw@alias@ctrl{#2}p%
      \yquant@draw@alias@ctrl{#2}n%
   \or%
      \yquant@draw@alias{#2}%
   \or%
      \yquant@draw@alias{#2}%
      \yquant@draw@alias@ctrl{#2}n%
   \or%
      \yquant@draw@alias{#2}%
      \yquant@draw@alias@ctrl{#2}p%
   \or%
      \yquant@draw@alias{#2}%
      \yquant@draw@alias@ctrl{#2}p%
      \yquant@draw@alias@ctrl{#2}n%
   \fi%
   \edef\process{%
         \endgroup%
         \def\noexpand\yquant@circuit@extendcontrolline@clip{%
            \unexpanded\expandafter{\yquant@circuit@extendcontrolline@clip}%
         }%
         \def\noexpand\yquant@circuit@extendcontrolline@prev{%
            \unexpanded\expandafter{\yquant@circuit@extendcontrolline@prev}%
         }%
         \def\noexpand\yquant@circuit@extendcontrolline@cmd{%
            \unexpanded\expandafter{\yquant@circuit@extendcontrolline@cmd}%
         }%
         \def\noexpand\yquant@circuit@extendmultiline@total{%
            \unexpanded\expandafter{\yquant@circuit@extendmultiline@total}%
         }%
         \def\noexpand\yquant@draw@@idx@pcontrol{\yquant@draw@@idx@content}%
      }%
   \process%
}

\protected\def\yquant@draw@inject#1{%
   \csname yquant@draw@@injection@#1\endcsname%
   \csgundef{yquant@draw@@injection@#1}%
}

\protected\def\yquant@draw@inject@outer#1{%
   % we thought we wanted to inject #1, however, this was not valid; so now insert it directly.
   \expandafter\expandafter\expandafter\yquant@draw@inject@outer@helper%
      \csname yquant@draw@@injection@#1\endcsname%
   \csgundef{yquant@draw@@injection@#1}%
}

\def\yquant@draw@inject@outer@helper\yquant@draw@begininjection#1\yquant@draw@stopinjection{%
   \yquant@draw@group%
      #1%
   \yquant@draw@endgroup%
}

\protected\def\yquant@draw@single#1#2{%
   \let\idx=\yquant@draw@@idx@content%
   \yquant@config@operator@multifalse%
   \edef\cmd{%
      \noexpand\path (\yquant@draw@@x, \yquant@register@get@y{#1})%
         node[/yquant/every operator, \yquant@draw@@style, /yquant/this operator,%
              name prefix=, name suffix=, name=yquantbox]%
         {\unexpanded\expandafter{\yquant@draw@@content}};%
      \pgfshapeclippath{yquantbox}%
                       {/yquant/every operator, \yquant@draw@@style,%
                        /yquant/this operator}%
   }%
   \cmd%
   \yquant@circuit@extendwire{#1}{center}%
   \expandafter\yquant@circuit@extendcontrolline\expandafter%
      {\the\yquant@draw@@currentcontroltype}\yquant@draw@@x%
   % check for empty name parameter
   \ifstrempty{#2}\relax{%
      \pgfnodealias{\tikz@pp@name{#2}}{yquantbox}%
   }%
   \numdef\yquant@draw@@idx@content{\yquant@draw@@idx@content+1}%
}

\protected\def\yquant@draw@multi#1#2#3#4#5{%
   \yquant@config@operator@multitrue%
   \let\idx=\yquant@draw@@idx@content%
   \edef\yquant@draw@multi@@name{#5}%
   \def\yquant@draw@@idx@multipart{0}%
   \let\yquant@circuit@extendmultiline@cmd=\empty%
   \let\yquant@circuit@extendmultiline@prev=\relax%
   \let\yquant@circuit@extendmultiline@clip=\empty%
   \let\yquant@register@multi@contiguous=\yquant@draw@multi@contiguous%
   #4%
   \ifnum\yquant@draw@@idx@multipart>1 %
      % make sure also the first split part is available via the "-s0" suffix
      \unless\ifx\yquant@draw@multi@@name\empty%
         \pgfnodealias{\tikz@pp@name{\yquant@draw@multi@@name-s0}}%
                      {\tikz@pp@name{\yquant@draw@multi@@name}}%
      \fi%
      \yquant@draw@mline@prep%
   \fi%
   \numdef\yquant@draw@@idx@content{\yquant@draw@@idx@content+1}%
}

\protected\def\yquant@draw@multi@contiguous#1#2#3{%
   % We need to somehow extract the y radius
   \edef\cmd{%
      \noexpand\path (\yquant@draw@@x, \the\dimexpr.5\dimexpr%
                         \yquant@register@get@y{#1}+\yquant@register@get@y{#2}\relax%
                      \relax)%
         node[/yquant/every operator, \yquant@draw@@style, /yquant/this operator,%
              /yquant/internal/multi main=\ifnum#3=1 true\else false\fi\unless\ifnum#1=#2 ,%
              y radius/.expanded=\the\dimexpr.5\dimexpr\yquant@register@get@ydist{#1}{#2}\relax\relax+%
                     .5*\noexpand\pgfkeysvalueof{/tikz/y radius}\fi,%
              name prefix=, name suffix=, name=yquantbox]%
            {\unexpanded\expandafter{\yquant@draw@@content}};%
      \pgfshapeclippath{yquantbox}%
                       {/yquant/every operator, \yquant@draw@@style,%
                        /yquant/this operator}%
   }%
   \cmd%
   \yquant@for \i := #1 to #2 {%
      \yquant@circuit@extendwire\i{center}%
   }%
   \yquant@circuit@extendmultiline\yquant@draw@@x%
   \expandafter\yquant@circuit@extendcontrolline\expandafter%
      {\the\yquant@draw@@currentcontroltype}\yquant@draw@@x%
   \unless\ifx\yquant@draw@multi@@name\empty%
      \ifnum\yquant@draw@@idx@multipart=0 %
         \pgfnodealias{\tikz@pp@name{\yquant@draw@multi@@name}}{yquantbox}%
      \else%
         \pgfnodealias{\tikz@pp@name{\yquant@draw@multi@@name-s\yquant@draw@@idx@multipart}}{yquantbox}%
      \fi%
   \fi%
   \numdef\yquant@draw@@idx@multipart{\yquant@draw@@idx@multipart+1}%
}

\protected\def\yquant@draw@multiinit#1#2#3#4#5{%
   \let\idx=\yquant@draw@@idx@content%
   \@tempdima=-.5\dimexpr\yquant@config@register@sep\relax%
   \dimdef\yquant@draw@multiinit@@min{\yquant@register@get@y{#1}-\@tempdima}%
   \dimdef\yquant@draw@multiinit@@max{\yquant@register@get@y{#2}+\@tempdima}%
   \dimdef\yquant@draw@multiinit@@total{%
      \yquant@draw@multiinit@@max-\yquant@draw@multiinit@@min%
   }%
   \def\pgfdecorationsegmentaspect{0}%
   \let\yquant@register@multi@contiguous=\yquant@draw@multiinit@contiguous%
   \let\pgfdecorationsegmentfromto=\empty%
   #4%
   \edef\pgfdecorationsegmentfromto{\expandafter\@gobble\pgfdecorationsegmentfromto}%
   \yquant@config@operator@multitrue%
   % We need to somehow extract the y radius
   \edef\cmd{%
      \noexpand\path (\yquant@draw@@x, \the\dimexpr.5\dimexpr%
                         \yquant@draw@multiinit@@min+\yquant@draw@multiinit@@max\relax%
                      \relax)%
         node[/yquant/every operator, \yquant@draw@@style,
              \ifnum\yquant@compat<2 /yquant/every multi label,\fi%
              /yquant/this operator,%
              y radius=\yquant@abs{\the\dimexpr.5\dimexpr\yquant@draw@multiinit@@total\relax\relax},%
              name prefix=, name suffix=, name=yquantbox]%
            {\unexpanded\expandafter{\yquant@draw@@content}};%
      \pgfshapeclippath{yquantbox}%
                       {/yquant/every operator, \yquant@draw@@style,%
                        \ifnum\yquant@compat<2 /yquant/every multi label,\fi%
                        /yquant/this operator}%
   }%
   \cmd%
   \yquant@for \i := #1 to #2 {%
      \yquant@circuit@extendwire\i{center}%
   }%
   % no control line (init doesn't allow for those, so just save the no-op), no multi line
   % check for empty name parameter
   \ifstrempty{#5}\relax{%
      \pgfnodealias{\tikz@pp@name{#5}}{yquantbox}%
   }%
   \numdef\yquant@draw@@idx@content{\yquant@draw@@idx@content+1}%
}

\protected\def\yquant@draw@multiinit@contiguous#1#2#3{%
   \edef\yquant@draw@multiinit@@from{%
      \pgfmath@tonumber{\dimexpr%
         \dimexpr\yquant@register@get@y{#1}-\@tempdima-\yquant@draw@multiinit@@min\relax*65536/%
         \dimexpr\yquant@draw@multiinit@@total\relax%
      \relax}%
   }%
   \edef\yquant@draw@multiinit@@to{%
      \pgfmath@tonumber{\dimexpr%
         \dimexpr\yquant@register@get@y{#2}+\@tempdima-\yquant@draw@multiinit@@min\relax*65536/%
         \dimexpr\yquant@draw@multiinit@@total\relax%
      \relax}%
   }%
   \eappto\pgfdecorationsegmentfromto{,%
      \yquant@draw@multiinit@@from-\yquant@draw@multiinit@@to%
   }%
   % We need to decide where to put the brace arch.
   \ifdim\yquant@draw@multiinit@@from pt<.5pt %
      \ifdim\yquant@draw@multiinit@@to pt>.5 pt%
         % This segment covers the true 1/2 position, take it
         \def\pgfdecorationsegmentaspect{.5}%
      \else%
         % We are not there yet, so the end of this segment is the closest we can get to the mid so far
         \edef\pgfdecorationsegmentaspect{\yquant@draw@multiinit@@to}%
      \fi%
   \else%
      % We are already beyond the mid...
      \ifdim\pgfdecorationsegmentaspect pt<.5pt %
         % ...but we did not find an ideal position yet
         \ifdim\dimexpr\yquant@draw@multiinit@@from pt-.5pt\relax<%
            \dimexpr.5pt-\pgfdecorationsegmentaspect pt\relax%
            % this one is closer to the mid than anything found before
            \edef\pgfdecorationsegmentaspect{\yquant@draw@multiinit@from}%
         \fi%
      \fi%
   \fi%
}

\protected\long\def\yquant@draw@output@single#1#2{%
   \let\idx=\yquant@draw@@idx@content%
   \yquant@config@operator@multifalse%
   \edef\cmd{%
      \noexpand\path (\yquant@circuit@endwires@x, \yquant@register@get@y{#1})%
         node[\ifnum\yquant@compat>1 /yquant/every operator,\fi%
              /yquant/every output,%
              /yquant/every \yquant@register@type@tostring{\yquant@register@get@type{#1}} output,%
              \yquant@draw@@style, /yquant/this operator,%
              name prefix=, name suffix=, name=yquantbox]%
         {\unexpanded\expandafter{\yquant@draw@@content}};%
      \ifdefined\yquant@parent%
         \pgfshapeclippath{yquantbox}%
                          {\ifnum\yquant@compat>1 /yquant/every operator,\fi%
                           /yquant/every output,%
                           /yquant/every \yquant@register@type@tostring{\yquant@register@get@type{#1}} output,%
                           \yquant@draw@@style,%
                           /yquant/this operator}%
      \fi%
   }%
   \cmd%
   % only extend for subcircuits
   \ifdefined\yquant@parent%
      \yquant@circuit@extendwire{#1}{center}%
   \fi%
   % check for empty name parameter
   \ifstrempty{#2}\relax{%
      \pgfnodealias{\tikz@pp@name{#2}}{yquantbox}%
   }%
   \numdef\yquant@draw@@idx@content{\yquant@draw@@idx@content+1}%
}

\protected\long\def\yquant@draw@output@multi#1#2#3#4#5{%
   \let\idx=\yquant@draw@@idx@content%
   \@tempdima=-.5\dimexpr\yquant@config@register@sep\relax%
   \dimdef\yquant@draw@multiinit@@min{\yquant@register@get@y{#1}-\@tempdima}%
   \dimdef\yquant@draw@multiinit@@max{\yquant@register@get@y{#2}+\@tempdima}%
   \dimdef\yquant@draw@multiinit@@total{%
      \yquant@draw@multiinit@@max-\yquant@draw@multiinit@@min%
   }%
   \def\pgfdecorationsegmentaspect{0}%
   \let\yquant@register@multi@contiguous=\yquant@draw@multiinit@contiguous%
   \let\pgfdecorationsegmentfromto=\empty%
   #4%
   \edef\pgfdecorationsegmentfromto{\expandafter\@gobble\pgfdecorationsegmentfromto}%
   \yquant@config@operator@multitrue%
   % We need to somehow extract the y radius
   \edef\cmd{%
      \noexpand\path (\yquant@circuit@endwires@x, \the\dimexpr.5\dimexpr%
                         \yquant@draw@multiinit@@min+\yquant@draw@multiinit@@max\relax%
                      \relax)%
         node[\ifnum\yquant@compat>1 /yquant/every operator,\fi /yquant/every output,%
              \yquant@draw@@style,%
              \ifnum\yquant@compat<2 /yquant/every multi output,\fi%
              /yquant/this operator,%
              y radius=\yquant@abs{\the\dimexpr.5\dimexpr\yquant@draw@multiinit@@total\relax\relax},%
              name prefix=, name suffix=, name=yquantbox]%
            {\unexpanded\expandafter{\yquant@draw@@content}};%
      \ifdefined\yquant@parent%
         \pgfshapeclippath{yquantbox}%
                          {\ifnum\yquant@compat>1 /yquant/every operator,\fi /yquant/every output,%
                           \yquant@draw@@style,
                           \ifnum\yquant@compat<2 /yquant/every multi output,\fi%
                           /yquant/this operator}%
      \fi%
   }%
   \cmd%
   % only extend for subcircuits
   \ifdefined\yquant@parent%
      \yquant@for \i := #1 to #2 {%
         \yquant@circuit@extendwire\i{center}%
      }%
   \fi%
   % check for empty name parameter
   \ifstrempty{#5}\relax{%
      \pgfnodealias{\tikz@pp@name{#5}}{yquantbox}%
   }%
   \numdef\yquant@draw@@idx@content{\yquant@draw@@idx@content+1}%
}

\protected\def\yquant@draw@subcircuit@nodecallback#1{%
   \ifstrequal{#1}{yquantbox}\relax{%
      \listcsxadd{\yquant@prefix draw@subcircuit@nodelist}{#1}%
   }%
}

% #1: id of subcircuit
% #2: name
% #3: 1 if aliasing of the name should be done (remove -0), 0 else
% #4: {width of subcircuit (excluding outer box)}{including outer box}{left margin}
% #5: affected wires
\protected\long\def\yquant@draw@subcircuit@prepare#1#2#3#4#5{%
   \let\idx=\yquant@draw@@idx@content%
   % In order to wrap the inner circuit in a proper box operator and clip outer paths appropriately (which was not possible yet, as we didn't know the exact vertical positions), we first place it within a box.
   % First, we anticipate the macro that is used by our subcircuit to store the node
   % names.
   \edef\yquant@draw@subcircuit@nodelist{yquant@env#1@draw@subcircuit@nodelist}%
   \global\cslet\yquant@draw@subcircuit@nodelist\empty%
   % \pgfinterruptboundingbox, but just for y
   \begingroup%
      \edef\pgf@interrupt@savemaxy{\the\pgf@picmaxy}%
      \edef\pgf@interrupt@saveminy{\the\pgf@picminy}%
      \pgf@picmaxy=-16000pt %
      \pgf@picminy=16000pt %
      \pgf@size@hookedfalse%
      \let\pgf@path@size@hook=\pgfutil@empty%
      % now we must take care of extending all the wires appropriately until the beginning of the box. #4 contains width of this box, #5 contains registers affected by this box. Note that for subcircuits, x extension by the group is disabled.
      \dimdef\newx{%
         \yquant@draw@@x-.5\dimexpr\@secondofthree#4\relax%
      }%
      \dimen0=\newx%
      \let\yquant@draw@subcircuit@leftpos=\newx% seamless subcircuits: do not add another separation if we are there
      \let\pgfshapeclippathhorzresult=\empty%
      \forlistloop\yquant@draw@move@loop{#5}%
      % but the new positions are not at the beginning of the box, but inside (with possible margin)
      \dimdef\newx{%
         \yquant@draw@@x-.5\dimexpr\@firstofthree#4\relax-\@thirdofthree#4%
      }%
      \forlistloop\yquant@draw@group@advance{#5}%
      \setbox\yquant@prepare@subcircuit@box=\hbox{{%
         \let\yquant@draw@subcircuit@wirestart=\newx%
         \let\yquant@parent=\yquant@prefix%
         \def\yquant@prefix{yquant@env#1@}%
         \pgfkeysgetvalue{/tikz/name prefix}\yquant@draw@subcircuit@prevprefix%
         % name mangling
         \ifcase\yquant@config@operator@subcircuit@mangling\relax%
            % prefix or discard: if we have an outer name, use it as the prefix; if not, discard all names
            \ifstrempty{#2}{%
               % we make sure there are no conflicts by prefixing any named nodes in any case.
               \pgfkeys{/tikz/name prefix/.expanded={sub\yquant@prefix-}}%
               \let\pgf@nodecallback=\yquant@draw@subcircuit@nodecallback%
            }{%
               \pgfkeys{/tikz/name prefix/.expanded={\yquant@draw@subcircuit@prevprefix#2-}}%
               \ifnum#3=1 %
                  \let\pgf@nodecallback=\yquant@draw@subcircuit@nodecallback%
               \fi%
            }%
         \or%
            % prefix or transparent: if we have an outer name, use it as a prefix; if not, directly use the outer namespace
            \ifstrempty{#2}\relax{%
               \pgfkeys{/tikz/name prefix/.expanded={\yquant@draw@subcircuit@prevprefix#2-}}%
               \ifnum#3=1 %
                  \let\pgf@nodecallback=\yquant@draw@subcircuit@nodecallback%
               \fi%
            }%
         \or%
            % transparent: all names go directly in the outer namespace
         \or%
            % discard: no name will be visible in the outer namespace whatsoever
            \pgfkeys{/tikz/name prefix/.expanded={sub\yquant@prefix-}}%
            \let\pgf@nodecallback=\yquant@draw@subcircuit@nodecallback%
         \else%
            \PackageError{yquant.sty}{Assertion failure}{Unknown value for name mangling.}%
         \fi%
         \pgfkeys{/yquant/operators/this subcircuit box/.style={}}%
         \edef\yquant@draw@subcircuit@style{%
            /yquant/every operator, \yquant@draw@@style,%
            /yquant/this operator, /yquant/internal/multi main=true,%
         }%
         \expandafter\tikzset\expandafter{\yquant@draw@subcircuit@style}%
         \begingroup%
            \csname\yquant@prefix draw\endcsname%
         \endgroup%
         % BEGIN_FOLD bounding box
         % Completely empty wires did not yet affect the bounding box
         % Problem: we compare an user-mode TikZ position (register y position) with a system-level pgf position (picture boundary box). If shifts or scalings are in effect, we must first transform the point appropriately. Note that negative scalings may upset our assumption of which is the minimum and which is the maximum! If additionally rotations are in effect, we must even consider those transformations for the leftmost and the rightmost point, which makes all of this far more complicated than it should be. For this reason, we have a shortcut in action in case no nontranslation transformations are present.
         \ifpgf@pt@identity%
            \dimen0=\dimexpr\yquant@register@get@y1+\pgf@pt@y\relax%
            \ifdim\dimen0>\pgf@picmaxy %
               \global\pgf@picmaxy=\dimen0 %
            \fi%
            \dimen0=\dimexpr\yquant@register@get@y{\csname\yquant@prefix registers\endcsname}+\pgf@pt@y\relax%
            \ifdim\dimen0<\pgf@picminy %
               \global\pgf@picminy=\dimen0 %
            \fi%
         \else%
            % first wire, left end
            \pgfpointtransformed{\pgfqpoint{\yquant@draw@@x-.5\dimexpr\@firstofthree#4\relax}{\yquant@register@get@y1\relax}}%
            \ifdim\pgf@y>\pgf@picmaxy %
               \global\pgf@picmaxy=\pgf@y %
            \fi%
            \ifdim\pgf@y<\pgf@picminy % negative scaling
               \global\pgf@picminy=\pgf@y %
            \fi%
            % first wire, right end
            \pgfpointtransformed{\pgfqpoint{\yquant@draw@@x+.5\dimenxpr\@firstofthree#4\relax}{\yquant@register@get@y1\relax}}%
            \ifdim\pgf@y>\pgf@picmaxy %
               \global\pgf@picmaxy=\pgf@y %
            \fi%
            \ifdim\pgf@y<\pgf@picminy % negative scaling
               \global\pgf@picminy=\pgf@y %
            \fi%
            % last wire, left end
            \pgfpointtransformed{\pgfqpoint{\yquant@draw@@x-.5\dimexpr\@firstofthree#4\relax}{\yquant@register@get@y{\csname\yquant@prefix registers\endcsname}\relax}}%
            \ifdim\pgf@y>\pgf@picmaxy %
               \global\pgf@picmaxy=\pgf@y %
            \fi%
            \ifdim\pgf@y<\pgf@picminy % negative scaling
               \global\pgf@picminy=\pgf@y %
            \fi%
            % last wire, right end
            \pgfpointtransformed{\pgfqpoint{\yquant@draw@@x+.5\dimenxpr\@firstofthree#4\relax}{\yquant@register@get@y{\csname\yquant@prefix registers\endcsname}\relax}}%
            \ifdim\pgf@y>\pgf@picmaxy %
               \global\pgf@picmaxy=\pgf@y %
            \fi%
            \ifdim\pgf@y<\pgf@picminy % negative scaling
               \global\pgf@picminy=\pgf@y %
            \fi%
         \fi%
         % END_FOLD
         \ifnum\yquant@config@operator@subcircuit@mangling<2 %
            % only bother with aliasing if the prefix is present at all
            \ifnum#3=1 %
               \ifstrempty{#2}\relax{%
                  % we must apply the aliasing to all the included nodes. We do this in this group, which still has the callback available, so that the aliased nodes will also be added to the list and can propagate (note that the number of node names is then exponential in the number of nested subcircuits)
                  \pgfkeysgetvalue{/tikz/name prefix}\yquant@draw@subcircuit@alias@prefix%
                  \expandafter\protected\expandafter\edef\expandafter%
                     \yquant@draw@subcircuit@alias@do\expandafter##\expandafter1\yquant@draw@subcircuit@alias@prefix##2\relax##3\relax{%
                     \noexpand\ifstrempty{##1}{%
                        \noexpand\pgfnodealias{\yquant@draw@subcircuit@prevprefix\yquant@draw@subcircuit@alias@removezero#2-##2}{\yquant@draw@subcircuit@alias@prefix##2}%
                        \noexpand\@gobble% there is an additional \relax
                     }\relax%
                  }%
                  \expandafter\forlistcsloop\expandafter%
                     {\expandafter\yquant@draw@subcircuit@alias\expandafter{%
                        \yquant@draw@subcircuit@alias@prefix}%
                     }\yquant@draw@subcircuit@nodelist%
               }%
            \fi%
         \fi%
      }}%
      \ifpgf@pt@identity%
         \dimen0=\dimexpr.5\pgf@picminy+.5\pgf@picmaxy-\pgf@pt@y\relax%
         \dimen2=\dimexpr\pgf@picmaxy-\pgf@picminy\relax%
      \else%
         \begingroup%
            \pgftransforminvert%
            \pgfpointtransformed{\pgfqpoint{\pgf@picminx}{\pgf@picminy}}%
            \@tempdima=\pgf@y%
            \pgfpointtransform{\pgfqpoint{\pgf@picmaxx}{\pgf@picmaxy}}%
            \edef\cmd{\@tempdima=\the\@tempdima\space\@tempdimb=\the\@tempdimb\space}%
            \expandafter%
         \endgroup%
         \cmd%
         \pgfpointtransformed{\pgfqpoint{\yquant@draw@@x}%
                                        {.5\dimexpr\@tempdima+\@tempdimb\relax}}%
         \dimen0=\pgf@y%
         \pgfpointtransformed{\pgfqpoint{\yquant@draw@@x}%
                                        {\dimexpr\@tempdimb-\@tempdima\relax}}%
         \dimen2=\pgf@y%
      \fi%
      \edef\cmd{%
         \noexpand\path (\yquant@draw@@x, \the\dimen0)%
            node[/yquant/every operator, \yquant@draw@@style,%
                 /yquant/operators/every subcircuit box, /yquant/this operator,%
                 /yquant/operators/this subcircuit box,%
                 /yquant/internal/multi main=true,%
                 name prefix=, name suffix=, name=yquantbox]%
            {\vbox to \the\dimen2 {\hbox to \@firstofthree#4 {}}};%
      }%
      \cmd%
      \unhbox\yquant@prepare@subcircuit@box%
   % \endpgfinterruptboundingbox + increase
      \ifdim\pgf@interrupt@savemaxy>\pgf@picmaxy%
         \global\pgf@picmaxy=\pgf@interrupt@savemaxy%
      \fi%
      \ifdim\pgf@interrupt@saveminy<\pgf@picminy%
         \global\pgf@picminy=\pgf@interrupt@saveminy%
      \fi%
   \endgroup%
   % Now that the subcircuit is finished, we need advance all the wires
   \dimdef\newx{\yquant@draw@@x+.5\dimexpr\yquant@draw@@width\relax}%
   \forlistloop\yquant@draw@group@advance{#5}%
   % name mangling
   \ifcase\yquant@config@operator@subcircuit@mangling\relax%
      % prefix or discard
      \ifstrempty{#2}{%
         % However, if the outer node was not named, no access to the inner nodes is desired, so we delete all nodes again.
         \def\do##1{%
            \csgundef{pgf@sh@ns@##1}%
            \csgundef{pgf@sh@np@##1}%
            \csgundef{pgf@sh@nt@##1}%
            \csgundef{pgf@sh@pi@##1}%
            \csgundef{pgf@sh@ma@##1}%
         }%
         \dolistcsloop{\yquant@draw@subcircuit@nodelist}%
         \csgundef\yquant@draw@subcircuit@nodelist%
      }{%
         \ifcsname\yquant@prefix draw@subcircuit@nodelist\endcsname%
            \csxappto{\yquant@prefix draw@subcircuit@nodelist}%
                     {\csname\yquant@draw@subcircuit@nodelist\endcsname}%
         \fi%
      }%
   \or%
      % prefix or transparent: in any case, make everything available for mangling in the outer circuit
      \ifcsname\yquant@prefix draw@subcircuit@nodelist\endcsname%
         \csxappto{\yquant@prefix draw@subcircuit@nodelist}%
                  {\csname\yquant@draw@subcircuit@nodelist\endcsname}%
      \fi%
   \or%
      % transparent: same
      \ifcsname\yquant@prefix draw@subcircuit@nodelist\endcsname%
         \csxappto{\yquant@prefix draw@subcircuit@nodelist}%
                  {\csname\yquant@draw@subcircuit@nodelist\endcsname}%
      \fi%
   \or%
      % discard: remove them all
      \def\do##1{%
         \csgundef{pgf@sh@ns@##1}%
         \csgundef{pgf@sh@np@##1}%
         \csgundef{pgf@sh@nt@##1}%
         \csgundef{pgf@sh@pi@##1}%
         \csgundef{pgf@sh@ma@##1}%
      }%
      \dolistcsloop{\yquant@draw@subcircuit@nodelist}%
      \csgundef\yquant@draw@subcircuit@nodelist%
   \else%
      \PackageError{yquant.sty}{Assertion failure}{Unknown value for name mangling (2).}%
   \fi%
}

\def\yquant@draw@subcircuit@alias@removezero#1-0{#1}

\def\yquant@draw@subcircuit@alias#1#2{%
   \yquant@draw@subcircuit@alias@do#2\relax#10-\relax\relax%
}

\protected\long\def\yquant@draw@subcircuit@single#1#2#3#4#5{%
   \yquant@config@operator@multifalse%
   \yquant@draw@subcircuit@prepare{#2}{#3}{#4}{#5}{#1}%
   \edef\cmd{%
      \pgfshapeclippath{yquantbox}{%
          /yquant/every operator, \yquant@draw@@style,%
          /yquant/operators/every subcircuit box, /yquant/this operator,%
          /yquant/operators/this subcircuit box,%
      }%
   }%
   \cmd%
   % see comment in draw@subcircuit@multi
   \yquant@softpath@extractmaxxat\pgfshapeclippathhorzresult{\yquant@register@get@y{#1}}%
   \let\pgfshapeclippathhorzresult=\empty%
   \yquant@circuit@extendwire{#1}*%
   \expandafter\yquant@circuit@extendcontrolline\expandafter%
      {\the\yquant@draw@@currentcontroltype}\yquant@draw@@x%
   % check for empty name parameter
   \ifstrempty{#3}\relax{%
      \pgfnodealias{\tikz@pp@name{#3}}{yquantbox}%
   }%
   \numdef\yquant@draw@@idx@content{\yquant@draw@@idx@content+1}%
}

\protected\long\def\yquant@draw@subcircuit@multi#1#2#3#4#5#6#7#8{%
   \yquant@config@operator@multitrue%
   % there is no contiguous slicing for subcircuits, as they may have all kinds of wire operations that can extend beyond the individual slices, let alone ancillas
   \yquant@draw@subcircuit@prepare{#5}{#6}{#7}{#8}{#4}%
   \edef\cmd{%
      \pgfshapeclippath{yquantbox}{%
          /yquant/every operator, \yquant@draw@@style,%
          /yquant/operators/every subcircuit box, /yquant/this operator,%
          /yquant/operators/this subcircuit box,%
          /yquant/internal/multi main=true,%
      }%
   }%
   \cmd%
   % install the clippings - but only on wires that are visually between the first and list while not being part of the circuit.
   \let\nonaffectedpgfshapeclippathhorzresult=\pgfshapeclippathhorzresult%
   \yquant@for \i := #1 to #2 {%
      \xifinlist{\i}{#4}{%
         % Usually, we always begin with a wire from the center of the operator shape and clip the inner parts away. This can't be done here, as the wire needs to be drawn _inside_ of the outer box operator here. Instead of clipping against the clip path, we extract its maximum x position at the position of the wire (which is an overkill for simple shapes, but allows to specify even more complicated ones) and place the wire at this position without clipping.
         % Note: this works very well for lines joining at perpendicular angles; but if the shape of the box is more fancy, while the position will be calculated correctly, the wire has a rectangular (or rounded, depending on the line cap) shape that is drawn on top of the operator. While \yquant@softpath@extractmaxxat could without much effort determine exactly the segment of the path that corresponds to the rightmost line, we would then have to convert this single line into a closed path that fills the linewidth and clip against it to get proper joiners. Since most likely, no-one will ever need this, we don't do it. But file a feature request if desired.
         \yquant@softpath@extractmaxxat\nonaffectedpgfshapeclippathhorzresult%
                                       {\yquant@register@get@y\i}%
         \let\pgfshapeclippathhorzresult=\empty%
         \yquant@circuit@extendwire\i*%
      }{%
         \let\pgfshapeclippathhorzresult=\nonaffectedpgfshapeclippathhorzresult%
         \yquant@circuit@extendwire\i{center}%
      }%
   }%
   \expandafter\yquant@circuit@extendcontrolline\expandafter%
      {\the\yquant@draw@@currentcontroltype}\yquant@draw@@x%
   \ifstrempty{#6}\relax{%
      \pgfnodealias{\tikz@pp@name{#6}}{yquantbox}%
   }%
   \numdef\yquant@draw@@idx@content{\yquant@draw@@idx@content+1}%
}

\protected\def\yquant@draw@control#1#2#3{%
   \edef\cmd{%
      \noexpand\path (\yquant@draw@@x, \yquant@register@get@y{#2})%
         node[/yquant/every control, /yquant/every #1 control, /yquant/this control,%
              name prefix=, name suffix=, name=yquantbox]%
         {};%
      \pgfshapeclippath{yquantbox}%
                       {/yquant/every control, /yquant/every #1 control,%
                        /yquant/this control}%
   }%
   \cmd%
   \yquant@circuit@extendwire{#2}{center}%
   \yquant@draw@@currentcontroltype=\yquant@register@get@type{#2}\relax%
   \expandafter\yquant@circuit@extendcontrolline\expandafter%
      {\yquant@draw@@currentcontroltype}\yquant@draw@@x%
   % check for empty name parameter
   \ifstrempty{#3}\relax{%
      \pgfnodealias{\tikz@pp@name{#3}}{yquantbox}%
   }%
}

\protected\def\yquant@draw@pcontrol#1#2{%
   \let\idx=\yquant@draw@@idx@pcontrol%
   \yquant@draw@control{positive}{#1}{#2}%
   \numdef\yquant@draw@@idx@pcontrol{\yquant@draw@@idx@pcontrol+1}%
}

\protected\def\yquant@draw@ncontrol#1#2{%
   \let\idx=\yquant@draw@@idx@ncontrol%
   \yquant@draw@control{negative}{#1}{#2}%
   \numdef\yquant@draw@@idx@ncontrol{\yquant@draw@@idx@ncontrol+1}%
}

\protected\def\yquant@draw@cline{%
   \pgfscope%
      % install the clipping
      \pgfsyssoftpath@setcurrentpath\yquant@circuit@extendcontrolline@clip%
      % and invert it. It is sufficient to cover the current bounding box, as the wire will be drawn between existing operators.
      \ifyquantdebug%
         \pgfsetfillcolor{teal}%
         \pgfsetfillopacity{.3}%
         \pgfusepathqfill%
      \else%
         \begingroup%
            \pgftransformreset%
            \pgfpathrectanglecorners%
               {\pgfqpoint{\pgf@picminx}{\pgf@picminy}}%
               {\pgfqpoint{\pgf@picmaxx}{\pgf@picmaxy}}%
            \pgfseteorule% even-odd to properly invert the clipping
            \pgfusepathqclip%
         \endgroup%
      \fi%
      \edef\cmd{%
         \noexpand\path[/yquant/every control line]%
            \yquant@circuit@extendcontrolline@cmd;%
      }%
      \cmd%
   \endpgfscope%
}

\protected\def\yquant@draw@mline@prep{%
   \eappto\yquant@circuit@extendmultiline@total{%
      \yquant@draw@mline%
         {\unexpanded\expandafter{\yquant@circuit@extendmultiline@clip}}%
         {\yquant@circuit@extendmultiline@cmd}%
   }%
}

\protected\def\yquant@draw@mline#1#2{%
   \pgfscope%
      % install the clipping
      \def\pgfsyssoftpath@thepath{#1}%
      \pgfsyssoftpath@setcurrentpath\pgfsyssoftpath@thepath%
      % and invert it. It is sufficient to cover the current bounding box, as the wire will be drawn between existing operators.
      \ifyquantdebug%
         \pgfsetfillcolor{teal}%
         \pgfsetfillopacity{.3}%
         \pgfusepathqfill%
      \else%
         \begingroup%
            \pgftransformreset%
            \pgfpathrectanglecorners%
               {\pgfqpoint{\pgf@picminx}{\pgf@picminy}}%
               {\pgfqpoint{\pgf@picmaxx}{\pgf@picmaxy}}%
            \pgfseteorule% even-odd to properly invert the clipping
            \pgfusepathqclip%
         \endgroup%
      \fi%
      \path[/yquant/every multi line] #2;%
   \endpgfscope%
}

\protected\def\yquant@draw@alias#1{%
   \pgfnodealias{\tikz@pp@name{#1}}{\tikz@pp@name{#1-0}}%
}

\protected\def\yquant@draw@alias@ctrl#1#2{%
   \pgfnodealias{\tikz@pp@name{#1-#2}}{\tikz@pp@name{#1-#20}}%
}

\protected\def\yquant@draw@wire#1#2{%
   \begingroup%
      \yquant@register@get@typeywire{#1}\wiretype\wireypos\wirelast%
      \unless\ifnum\wiretype=\yquant@register@type@none%
         \edef\wirexprevpos{\expandafter\@firstoffour\wirelast}%
         \ifx0#2%
            \edef\wirexpos{\expandafter\@secondoffour\wirelast}%
         \else%
            \let\wirexpos=\yquant@circuit@endwires@x%
         \fi%
         \ifdim\wirexpos>\wirexprevpos %
            \edef\wirestyle{\noexpand\tikzset{%
               /yquant/this wire/.style={%
                  /yquant/every wire,%
                  /yquant/every \yquant@register@type@tostring\wiretype\space wire,%
                     \yquant@register@get@style{#1}%
               }, /yquant/this wire%
            }}%
            \wirestyle%
            % load all clippings
            \edef\wireclipping{%
               \unexpanded\expandafter\expandafter\expandafter{%
                  \expandafter\@thirdandfourthoffour\wirelast%
               }%
            }%
            \pgfscope%
               \unless\ifx\wireclipping\empty% may happen if the style is altered to be invisible, though the type is not none
                  % install the clipping
                  \pgfsyssoftpath@setcurrentpath\wireclipping%
                  % invert the clipping
                  \ifyquantdebug%
                     \pgfsetfillcolor{orange}%
                     \pgfsetfillopacity{.3}%
                     \pgfusepathqfill%
                  \else%
                     % We need to access the current bounding box as well as other positions in the local coordinate frame. For this, transform the bounding box to the current frame (though this is expensive). Does this capture rotations correctly?
                     \begingroup%
                        \ifdim\pgf@picminx>\pgf@picmaxx%
                           % nothing drawn yet (or bounding box reset)
                           \pgf@picminx=0pt %
                           \pgf@picmaxx=0pt %
                        \fi%
                        \ifdim\pgf@picminy>\pgf@picmaxy%
                           \pgf@picminy=0pt %
                           \pgf@picmaxy=0pt %
                        \fi%
                        \pgftransforminvert%
                        \pgfpointtransformed{\pgfqpoint{\pgf@picminx}{\pgf@picminy}}%
                        \global\@tempdima=\pgf@y%
                        \pgfpointtransformed{\pgfqpoint{\pgf@picmaxx}{\pgf@picmaxy}}%
                        \global\@tempdimb=\pgf@y%
                     \endgroup%
                     % To avoid rendering artifacts at all zoom levels with all renderers, we need to make the clipping region large. Let's try the current bounding box first.
                     % This may be insufficient if there no or a tiny wire label and only registers of a small height. In this case, take ten times the line width or at least 1cm, but don't let it affect the bounding box.
                     \ifdim\dimexpr\@tempdimb-\@tempdima\relax<10\pgflinewidth %
                        \@tempdima=\dimexpr\wireypos-5\pgflinewidth\relax%
                        \@tempdimb=\dimexpr\wireypos+5\pgflinewidth\relax%
                     \fi%
                     \ifdim\dimexpr\@tempdimb-\@tempdima\relax<1cm %
                        \@tempdima=\dimexpr\wireypos-5mm\relax%
                        \@tempdimb=\dimexpr\wireypos+5mm\relax%
                     \fi%
                     \pgf@relevantforpicturesizefalse%
                        \pgfpathrectanglecorners%
                           {\pgfqpoint{\dimexpr\wirexprevpos-2\pgflinewidth\relax}%
                                      {\@tempdima}}%
                           {\pgfqpoint{\dimexpr\wirexpos+2\pgflinewidth\relax}%
                                      {\@tempdimb}}%
                     \pgf@relevantforpicturesizetrue%
                     \pgfseteorule% even-odd to properly invert the clipping
                     \pgfusepathqclip%
                  \fi%
               \fi%
               % the clip inversion is left to the drawing commands (clip two \pgflinewidth more to avoid renderer artifacts)
               \csname yquant@draw@wire@\wiretype\endcsname{#1}%
            \endpgfscope%
         \fi%
      \fi%
   \endgroup%
}

% quantum wire
\protected\csdef{yquant@draw@wire@\yquant@register@type@q}#1{%
   \edef\cmd{%
      \noexpand\path [/yquant/this wire]%
         (\wirexprevpos,\wireypos) -- (\wirexpos,\wireypos);%
   }%
   \cmd%
}

% classical wire
\protected\csdef{yquant@draw@wire@\yquant@register@type@c}#1{%
   \edef\cmd{%
      \noexpand\path [/yquant/this wire]%
         (\wirexprevpos,\wireypos+2\pgflinewidth)--(\wirexpos,\wireypos+2\pgflinewidth)%
         (\wirexprevpos,\wireypos-2\pgflinewidth)--(\wirexpos,\wireypos-2\pgflinewidth);%
   }%
   \cmd%
}

% quantum-bundle
\protected\csdef{yquant@draw@wire@\yquant@register@type@qs}#1{%
   \edef\cmd{%
      \noexpand\path [/yquant/this wire]%
         (\wirexprevpos,\wireypos+2\pgflinewidth)--(\wirexpos,\wireypos+2\pgflinewidth)%
         (\wirexprevpos,\wireypos)--(\wirexpos,\wireypos)%
         (\wirexprevpos,\wireypos-2\pgflinewidth)--(\wirexpos,\wireypos-2\pgflinewidth);%
   }%
   \cmd%
}

\protected\def\yquant@draw@hspace#1#2{%
   \begingroup%
      \yquant@register@get@maxxlist\newx{#1}%
      \dimdef\newx{\newx+#2}%
      \dimen0=\newx%
      \let\pgfshapeclippathhorzresult=\empty%
      \forlistloop\yquant@draw@move@loop{#1}%
   \endgroup%
}

\protected\def\yquant@draw@move@loop#1{%
   \yquant@register@set@x{#1}\newx%
   \yquant@circuit@extendwire{#1}*%
}

==> yquant-env.tex <==
\newif\ifyquant@env@lazy
\newif\ifyquantmeasuring

\protected\def\yquant@envunstar{%
   \yquant@env@lazyfalse%
   \yquant@env@begin%
}

\protected\def\yquant@envstar{%
   \yquant@env@lazytrue%
   \yquant@env@begin%
}

\protected\def\yquant@env@begin{%
   % We check for an optional argument, but if it is in a new line, we don't take it - it
   % might well be the square brace of an argument. Temporary change newlines to ordinary
   % characters.
   \catcode`\^^M=12 %
   \yquant@futurenonspacelet\yquant@env@begin@next\yquant@env@begin@checkarg%
}

{\catcode`\^^M=12 \global\let\yquant@env@linebreak=^^M}

\protected\def\yquant@env@begin@checkarg{%
   \catcode`\^^M=5 %
   \ifx\yquant@env@begin@next[%
      \expandafter\yquant@env@begin@arg%
   \else%
      \ifx\yquant@env@begin@next\yquant@env@linebreak%
         % In this case we don't really want to inject the wrong-catcode linebreak back,
         % which would produce an error.
         \afterassignment\yquant@env@begin@noarg%
         \expandafter\expandafter\expandafter\let%
         \expandafter\expandafter\expandafter\@eattoken%
         % since ^^M is an ordinary character, no need for "= ".
      \else%
         \expandafter\expandafter\expandafter\yquant@env@begin@noarg%
      \fi%
   \fi%
}

\def\yquant@env@begin@noarg{%
   \yquant@env@begin@arg[]%
}

\def\yquant@env@begin@arg{%
   \let\yquant@env@check=\yquant@env@check@%
   \yquant@env@begin@generic\yquant%
}

% sync with yquantlanguage-groups
\long\protected\def\yquant@env@begin@generic#1[#2]{%
   \begingroup%
      \let\yquant@parent=\yquant@prefix%
      \global\advance\yquant@env by 1 %
      \edef\yquant@prefix{yquant@env\the\yquant@env @}%
      \ifnum\yquant@env=1 %
         \yquantmeasuringtrue%
         \yquant@env@substikz#1%
         \global\cslet{\yquant@prefix parameters}\empty%
      \else%
         \let\yquant@lang@reset@attrs@inputoutput=\yquant@lang@reset@attrs@inputoutput@subcircuit%
         \global\cslet{\yquant@prefix parameters}\yquant@circuit@subcircuit@param%
         \yquant@env@lazyfalse% forbid lazy register creation in subcircuits. We need a proper and in-order declaration of the subcircuit's interface.
      \fi%
      \let#1=\yquant@env@scan%
      \yquant@env@reset@commands%
      \csgdef{\yquant@prefix registers}{0}%
      \global\cslet{\yquant@prefix draw}\relax%
      \global\cslet{\yquant@prefix outputs}\relax%
      \global\cslet{\yquant@prefix subcircuits}\empty%
      \global\cslet{\yquant@prefix inonly}\empty%
      \global\csletcs{\yquant@prefix seamless}{ifyquant@config@circuit@seamless}%
      \ifdefined\yquant@prevseamless%
         \cslet{ifyquant@config@circuit@seamless}\yquant@prevseamless%
         \undef\yquant@prevseamless%
      \fi%
      \csxdef{\yquant@prefix cleanup}{%
         \expandafter\noexpand\csname\yquant@prefix registers\endcsname%
         \expandafter\noexpand\csname\yquant@prefix draw\endcsname%
         \expandafter\noexpand\csname\yquant@prefix outputs\endcsname%
         \expandafter\noexpand\csname\yquant@prefix parameters\endcsname%
         \expandafter\noexpand\csname\yquant@prefix subcircuits\endcsname%
         \expandafter\noexpand\csname\yquant@prefix inonly\endcsname%
         \expandafter\noexpand\csname\yquant@prefix seamless\endcsname%
         \expandafter\noexpand\csname\yquant@prefix cleanup\endcsname%
      }%
      \scope[{/yquant/.cd, #2, /tikz/.cd, /yquant/every circuit}]%
}

\protected\def\yquant@env@end{%
         \ifnum\csname\yquant@prefix registers\endcsname>0 %
            \begingroup%
               \let\yquant@circuit@operator@pctrls=\empty%
               \yquant@for \i := 1 to \csname\yquant@prefix registers\endcsname {%
                  \yquant@register@execclear@lastgate{\i}{@end}%
               }%
            \endgroup%
            \csgappto{\yquant@prefix draw}{%
               \yquant@circuit@endwires%
            }%
            \expandafter\unless\expandafter\ifx\csname\yquant@prefix outputs\endcsname\relax%
               \begingroup%
                  \def\yquant@config@operator@minimum@width{0pt}%
                  \let\yquant@prepare@single=\yquant@prepare@output@single%
                  \let\yquant@prepare@multi=\yquant@prepare@output@multi%
                  \csname\yquant@prefix outputs\endcsname%
               \endgroup%
            \fi%
            \csgappto{\yquant@prefix draw}{%
               \yquant@circuit@endwires@finalize%
            }%
            % also calculate the true y positions
            \unless\ifdefined\yquant@parent%
               \yquant@env@end@calcypositions%
            \fi%
         \else%
            \ifdefined\yquant@parent%
               \PackageError{yquant.sty}{Empty subcircuit}%
                            {Subcircuits must contain registers.}%
            \else%
               \PackageWarning{yquant.sty}{Empty quantum circuit}%
            \fi%
         \fi%
         \global\let\yquant@env@scan=\relax% don't rescan after the scope
      \endscope% this will exit five to seven groups (depending on the transparency group state, and it might even be driver-dependent, though it is not at the moment), so better make the relax global
      \global\let\yquant@env@scan=\yquant@env@scan@%
      \ifdefined\yquant@parent%
         % We are in a subcircuit. The drawing and cleanup is delayed until the end.
         \csxappto{\yquant@parent cleanup}%
            {\unexpanded\expandafter\expandafter\expandafter{%
               \csname\yquant@prefix cleanup\endcsname%
            }}%
         \ifyquantdebug%
            \csshow{\yquant@prefix draw}%
         \fi%
      \else%
         % Now we actually carry out the tikz commands which were previously stored in the draw command. But before this, we get rid of all \yquant@env@scan calls and also restore the scope command, since this would add itself once again. And get@y needs to expand.
         \let\path=\tikz@command@path%
         \let\tikz@lib@scope@check=\yquant@env@substikz@scopecheck%
         \let\tikz@scope@opt=\yquant@env@substikz@scope%
         \let\endtikz@scope@env=\yquant@env@substikz@endscope%
         \let\endscope=\endtikz@scope@env%
         \let\stopscope=\endscope%
         \yquant@register@get@y@@expandable%
         \ifyquantdebug%
            \csshow{\yquant@prefix draw}%
         \fi%
         \yquantmeasuringfalse%
         \csname\yquant@prefix draw\endcsname%
         \expandafter\expandafter\expandafter\yquant@cleanup\csname\yquant@prefix cleanup\endcsname|%
         \global\yquant@env=0 %
      \fi%
   \endgroup%
}

\protected\def\ifyquant@env@seamless{%
   \csname\yquant@prefix seamless\endcsname%
      \expandafter\@firstoftwo%
   \else%
      \expandafter\@secondoftwo%
   \fi%
}

\newif\ifyquant@env@end@calcypositions@godeep
\protected\def\yquant@env@end@calcypositions{%
   \begingroup%
      \dimen4=\yquant@config@register@sep %
      \yquant@sort@clear%
      % Setup...
      \yquant@env@end@calcypositions@setup1%
      % and go!
      \let\redolist=\empty%
      \yquant@env@end@calcypositions@godeeptrue%
      \yquant@env@end@calcypositions@run1%
      \yquant@env@end@calcypositions@godeepfalse%
      \yquant@env@end@calcypositions@redo%
%      % The macros now set up performed all the proper and unambiguous justification. After that, we will also need to take care of the multi gates. We expect that for most of all multi gates, we already have enough space. But sometimes, this may not be the case, so we need to increase overall spacing and re-evaluate all spacing. In order to get a proper balanced layout, we start with the largest enlargement that is required. Every enlargement step will equally distribute the registers in between. Starting with the largest one, this is likely to also solve issues with smaller ones.
      \yquant@env@end@calcypositions@multi%
      % Turn the preliminary positions into true ones at every level.
      \yquant@env@end@setypositions1%
   \endgroup%
}

\protected\def\yquant@env@end@calcypositions@setup#1{%
   \def\yquant@prefix{yquant@env#1@}%
   % Our problem is a linear program. To solve it, we proceed iteratively: We define macros for each subcircuit that, based on the current positions, calculate the allowed positions.
   \letcs\max{\yquant@prefix registers}%
   % BEGIN_FOLD find out about the first and last register with maps
   \let\firstinout=\relax%
   \let\lastinout=\relax%
   \yquant@for \i := 1 to \max {%
      \ifcsname\yquant@prefix registermap@\i\endcsname%
         \ifx\firstinout\relax%
            \let\firstinout=\i%
         \fi%
         \let\lastinout=\i%
      \fi%
   }%
   % END_FOLD
   % BEGIN_FOLD Take care with internal registers before the first inout
   % We could in principle merge the loop to define \firstinout/\lastinout, but nested for loops are problematic.
   \ifx\firstinout\relax%
      \dimen0=\yquant@register@get@height1 %
      \def\i{1}%
   \else%
      \edef\outerlevel{\yquant@register@get@parent{\firstinout}}%
      \dimen0=\csname yquant@env\expandafter\@firstoftwo\outerlevel @env@endy@\expandafter\@secondoftwo\outerlevel\endcsname\relax%
      \ifnum\firstinout>1 %
         % We need to take special care with internal registers if the first one is not a connected one. In this case, the internal registers will grow upwards instead... Since the y position may change in both upward and downward direction, we need to have an additional bookkeeping value that stores the last y position of the first item in this subcircuit.
         \csedef{\yquant@prefix env@endyprev}{\the\dimen0}%
         \yquant@fordown \i := \numexpr\firstinout-1\relax downto 1 {%
            \advance \dimen0 by -\dimexpr%
               \expandafter\yquant@register@get@height\expandafter{\the\numexpr\i+1\relax}+%
               \dimen4+%
               \yquant@register@get@depth\i%
            \relax%
            % We know for sure there's none with a parent in this loop
            \csedef{\yquant@prefix env@endy@\i}{\the\dimen0}%
            \csedef{yquant@env@end@calcypositions@#1@\i}{%
               \advance\dimen0 by -\dimexpr%
                  \noexpand\yquant@register@get@height{\the\numexpr\i+1\relax}+%
                  \dimen4+%
                  \noexpand\yquant@register@get@depth{\i}%
               \relax%
               % The first connected wire might have been re-aligned, which destroys all our knowledge. \dimen2 will contain the relative shift that we must take into account.
               % Make sure the current y position is at most the previous y position + previous depth + separation + current height.
               \noexpand\ifdim\dimexpr\dimen0-\dimen2\relax<\expandafter\noexpand\csname\yquant@prefix env@endy@\i\endcsname\space%
                  \edef\expandafter\noexpand\csname\yquant@prefix env@endy@\i\endcsname{\noexpand\the\dimen0}%
                  \ifinlist{#1}\noexpand\redolist\relax{%
                     \listadd\noexpand\redolist{#1}%
                  }%
               \noexpand\else%
                  \noexpand\ifdim\dimen2=0pt %
                     % No change at all
                     \dimen0=\expandafter\noexpand\csname\yquant@prefix env@endy@\i\endcsname\space%
                  \noexpand\else%
                     % We must still overwrite the position macro due to the shift
                     \dimen0=\dimexpr\expandafter\noexpand\csname\yquant@prefix env@endy@\i\endcsname+\dimen2\relax%
                     \edef\expandafter\noexpand\csname\yquant@prefix env@endy@\i\endcsname{\noexpand\the\dimen0}%
                     \ifinlist{#1}\noexpand\redolist\relax{%
                        \listadd\noexpand\redolist{#1}%
                     }%
                  \noexpand\fi
               \noexpand\fi%
               \unless\ifx\i1%
                  \expandafter\noexpand\csname yquant@env@end@calcypositions@#1@\the\numexpr\i-1\relax\endcsname%
               \fi%
            }%
         }%
      \fi%
      \let\i=\firstinout%
   \fi%
   % END_FOLD
   % BEGIN_FOLD Define initial macro
   \csedef{yquant@env@end@calcypositions@#1}{%
      \def\noexpand\yquant@prefix{\yquant@prefix}%
      \dimen0=\expandafter\noexpand\csname\yquant@prefix env@endy@\i\endcsname\relax%
      \listremove\noexpand\redolist{#1}%
      \expandafter\noexpand\csname yquant@env@end@calcypositions@#1@\i\endcsname%
      \expandafter\unless\expandafter\ifx\csname\yquant@prefix subcircuits\endcsname\empty%
         \ifinlist{#1}\noexpand\redolist{%
            \noexpand\forlistloop%
               \yquant@env@end@calcypositions@run%
               \expandafter\noexpand\csname\yquant@prefix subcircuits\endcsname%
         }{%
            \noexpand\ifyquant@env@end@calcypositions@godeep%
               \noexpand\forlistloop%
                  \yquant@env@end@calcypositions@run%
                  \expandafter\noexpand\csname\yquant@prefix subcircuits\endcsname%
            \noexpand\fi%
         }%
      \fi%
   }%
   % END_FOLD
   % BEGIN_FOLD Set up chain of other macros
   % We set up a chain of position evaluation macros. We start with the first [external] register in the outermost circuit; it is supposed to call the evaluation macro of its successor. Next, we iterate through all subcircuits (recursively). Whenever we find a register that is mapped to an outer one, we take appropriate measures.
   \yquant@for \i := \i to \max {%
      \ifcsname\yquant@prefix registermap@\i\endcsname%
         % \outery = env@endy macro of parent wire
         \edef\outerlevel{\yquant@register@get@parent{\i}}%
         \edef\outery{%
            \expandafter\noexpand\csname yquant@env\expandafter\@firstoftwo\outerlevel @env@endy@\expandafter\@secondoftwo\outerlevel\endcsname%
         }%
         % in this initialization step, we only check in one direction
         \ifdim\dimen0<\outery\space%
            \dimen0=\outery\space%
         \fi%
      \fi%
      \csedef{\yquant@prefix env@endy@\i}{\the\dimen0}%
      \unless\ifx\i\max%
         \advance \dimen0 by \dimexpr%
            \yquant@register@get@depth\i+%
            \dimen4+%
            \expandafter\yquant@register@get@height\expandafter{\the\numexpr\i+1\relax}%
         \relax%
      \fi%
      \csedef{yquant@env@end@calcypositions@#1@\i}{%
         % make sure the current y position is at least the previous y position + previous depth + separation + current height
         \noexpand\ifdim\dimen0>\expandafter\noexpand\csname\yquant@prefix env@endy@\i\endcsname\space%
            \edef\expandafter\noexpand\csname\yquant@prefix env@endy@\i\endcsname{\noexpand\the\dimen0}%
            \ifinlist{#1}\noexpand\redolist\relax{%
               \listadd\noexpand\redolist{#1}%
            }%
         \noexpand\else%
            \dimen0=\expandafter\noexpand\csname\yquant@prefix env@endy@\i\endcsname\space%
         \noexpand\fi%
         % now \dimen0 holds the current y position of register \i
         % BEGIN_FOLD map
         \ifcsname\yquant@prefix registermap@\i\endcsname%
            % if this is an in/out register, put it at the same position as the outer one
            \noexpand\ifdim\dimen0<\expandafter\noexpand\outery\space%
               \dimen0=\expandafter\noexpand\outery\space%
               \let\expandafter\noexpand\csname\yquant@prefix env@endy@\i\endcsname\expandafter\noexpand\outery%
               \ifinlist{#1}\noexpand\redolist\relax{%
                  \listadd\noexpand\redolist{#1}%
               }%
            \noexpand\fi%
            \noexpand\ifdim\dimen0>\expandafter\noexpand\outery\space%
               \let\expandafter\noexpand\outery\expandafter\noexpand\csname\yquant@prefix env@endy@\i\endcsname%
               \ifinlist{\expandafter\@firstoftwo\outerlevel}\noexpand\redolist\relax{%
                  \listadd\noexpand\redolist{\expandafter\@firstoftwo\outerlevel}%
               }%
            \noexpand\fi%
            \ifx\i\firstinout%
               % This is the first in/out register. Find all previous internal registers and make sure the parent has enough height.
               \ifnum\i>1 %
                  % Here, we must now call the (backwards-running) alignment macros of the previous registers. First fill \dimen2 with the relative shift of this wire's position with respect to the last iteration.
                  \dimen2=\dimexpr\dimen0-\expandafter\noexpand\csname\yquant@prefix env@endyprev\endcsname\relax%
                  % Store \dimen0...
                  \dimen6=\dimen0 %
                  % ...call previous calculations...
                  \expandafter\noexpand\csname yquant@env@end@calcypositions@#1@\the\numexpr\i-1\relax\endcsname%
                  % ...restore...
                  \dimen0=\dimen6 %
                  % ...and backup its value for the next iteration.
                  \edef\expandafter\noexpand\csname\yquant@prefix env@endyprev\endcsname{\noexpand\the\dimen0}%
                  \expandafter\noexpand\csname ifdim\endcsname\noexpand\yquant@register@peek@height\outerlevel<\dimexpr%
                     \noexpand\yquant@register@get@height1+%
                     \expandafter\noexpand\csname\yquant@prefix env@endy@\i\endcsname-%
                     \expandafter\noexpand\csname\yquant@prefix env@endy@1\endcsname%
                  \relax%
                     \yquant@register@set@height@remote\outerlevel{\noexpand\the\dimexpr%
                        \noexpand\yquant@register@get@height1+%
                        \expandafter\noexpand\csname\yquant@prefix env@endy@\i\endcsname-%
                        \expandafter\noexpand\csname\yquant@prefix env@endy@1\endcsname%
                     }%
               \else%
                  \expandafter\noexpand\csname ifdim\endcsname\noexpand\yquant@register@peek@height\outerlevel<%
                     \noexpand\yquant@register@get@height1 %
                     \yquant@register@set@height@remote\outerlevel{%
                        \noexpand\yquant@register@get@height1%
                     }%
               \fi%
                     \ifinlist{\expandafter\@firstoftwo\outerlevel}\noexpand\redolist\relax{%
                        \listadd\noexpand\redolist{\expandafter\@firstoftwo\outerlevel}%
                     }%
                  \expandafter\noexpand\csname fi\endcsname%
            \fi%
            \ifx\i\lastinout%
               % this is the last in/out register. Find all following internal registers and make sure the parent has enough depth.
               \ifnum\i<\max\space%
                  \expandafter\noexpand\csname ifdim\endcsname\noexpand\yquant@register@peek@depth\outerlevel<\dimexpr%
                     \noexpand\yquant@register@get@depth{\max}+%
                     \expandafter\noexpand\csname\yquant@prefix env@endy@\max\endcsname-%
                     \expandafter\noexpand\csname\yquant@prefix env@endy@\i\endcsname%
                  \relax%
                     \yquant@register@set@depth@remote\outerlevel{\noexpand\the\dimexpr%
                        \noexpand\yquant@register@get@depth{\max}+%
                        \expandafter\noexpand\csname\yquant@prefix env@endy@\max\endcsname-%
                        \expandafter\noexpand\csname\yquant@prefix env@endy@\i\endcsname%
                     }%
               \else%
                  \expandafter\noexpand\csname ifdim\endcsname\noexpand\yquant@register@peek@depth\outerlevel<%
                     \noexpand\yquant@register@get@depth{\max} %
                     \yquant@register@set@depth@remote\outerlevel{%
                        \noexpand\yquant@register@get@depth{\max}%
                     }%
               \fi%
                     \ifinlist{\expandafter\@firstoftwo\outerlevel}\noexpand\redolist\relax{%
                        \listadd\noexpand\redolist{\expandafter\@firstoftwo\outerlevel}%
                     }%
                  \expandafter\noexpand\csname fi\endcsname%
            \fi%
         \fi%
         % END_FOLD
         \unless\ifx\i\max%
            \advance\dimen0 by \dimexpr%
               \noexpand\yquant@register@get@depth{\i}+%
               \dimen4+%
               \noexpand\yquant@register@get@height{\the\numexpr\i+1\relax}%
            \relax%
            \expandafter\noexpand\csname yquant@env@end@calcypositions@#1@\the\numexpr\i+1\relax\endcsname%
         \fi%
      }%
      % for every multi-register space requirement, install the requirement in the sortlist
      \edef\multidata{\yquant@register@get@multispace\i}%
      \forlistloop{\yquant@env@end@calcypositions@setupmulti{#1}}\multidata%
   }%
   % END_FOLD
   \forlistcsloop\yquant@env@end@calcypositions@setup{\yquant@prefix subcircuits}%
}

\protected\def\yquant@env@end@calcypositions@setupmulti#1#2{%
   \yquant@sort@eadd{%
      {#1}%
      {\i}%
      {\expandafter\@firstoftwo\yquant@env@end@calcypositions@setupmulti@group#2\yquant@end}%
      {\expandafter\@secondoftwo\yquant@env@end@calcypositions@setupmulti@group#2\yquant@end}%
   }%
}

\def\yquant@env@end@calcypositions@setupmulti@group#1:#2\yquant@end{{#1}{#2}}

\protected\def\yquant@env@end@calcypositions@run#1{%
   \csname yquant@env@end@calcypositions@#1\endcsname%
}

\protected\def\yquant@env@end@calcypositions@redo{%
   \forlistloop\yquant@env@end@calcypositions@run\redolist%
   \unless\ifx\redolist\empty%
      \expandafter\yquant@env@end@calcypositions@redo%
   \fi%
}

\def\yquant@env@end@calcypositions@multiheight#1#2#3#4{%
   \dimexpr%
      \csname yquant@env#1@env@endy@#3\endcsname-
      \csname yquant@env#1@env@endy@#2\endcsname+%
      \yquant@register@peek@height{#1}{#2}+%
      \yquant@register@peek@depth{#1}{#3}%
   \relax%
}

\def\yquant@env@end@calcypositions@sortmulti#1#2{%
   % sort, in descending order, by the amount of missing space
   \ifdim\dimexpr\@fourthoffour#2-\yquant@env@end@calcypositions@multiheight#2\relax>%
      \dimexpr\@fourthoffour#1-\yquant@env@end@calcypositions@multiheight#1\relax%
      \expandafter\@firstoftwo%
   \else%
      \expandafter\@secondoftwo%
   \fi%
}

\protected\def\yquant@env@end@calcypositions@multi{%
   % We will always only operate on the first item in the sortlist, which is determined anew in each iteration - as changes due to this first item will potentially affect all others, including which one is the next...
   \yquant@sort@findfirst\yquant@env@end@calcypositions@sortmulti\first%
   \unless\ifx\first\empty%
      \dimdef\missing{%
         \expandafter\@fourthoffour\first-%
         \expandafter\yquant@env@end@calcypositions@multiheight\first%
      }%
      % maybe this was already resolved?
      \ifdim\missing>0pt %
         \edef\yquant@prefix{yquant@env\expandafter\@firstoffour\first @}%
         \numdef\divisor{\expandafter\@thirdoffour\first-\expandafter\@secondoffour\first}% not +1, since we will not move the first element
         \dimdef\add{1sp+\dimexpr\missing-1sp\relax/\divisor}%
         \let\inc=\add%
         \edef\max{\expandafter\@thirdoffour\first}%
         \ifnum\expandafter\@secondoffour\first<\max\relax%
            \yquant@for \i := \numexpr\expandafter\@secondoffour\first+1\relax to \max {%
               \csdimdef{\yquant@prefix env@endy@\i}{\csname\yquant@prefix env@endy@\i\endcsname+\add}%
               \dimdef\add{\add+\inc}%
            }%
         \fi%
         \yquant@env@end@calcypositions@godeeptrue%
         \csname yquant@env@end@calcypositions@\expandafter\@firstoffour\first\endcsname%
         \yquant@env@end@calcypositions@godeepfalse%
         \yquant@env@end@calcypositions@redo%
         \expandafter\expandafter\expandafter\yquant@env@end@calcypositions@multi%
      \fi%
   \fi%
}

\protected\def\yquant@env@end@setypositions#1{%
   \def\yquant@prefix{yquant@env#1@}%
   \ifyquantdebug%
      \yquant@for \i := 1 to \csname\yquant@prefix registers\endcsname {%
         \ifcsname\yquant@prefix registermap@\i\endcsname%
            \message{^^J y(#1, \i): external}%
         \else%
            \message{^^J y(#1, \i): \csname\yquant@prefix env@endy@\i\endcsname}%
            \yquant@register@set@y\i{-\csname\yquant@prefix env@endy@\i\endcsname}%
         \fi%
      }%
   \else%
      \yquant@for \i := 1 to \csname\yquant@prefix registers\endcsname {%
         \unless\ifcsname\yquant@prefix registermap@\i\endcsname%
            \yquant@register@set@y\i{-\csname\yquant@prefix env@endy@\i\endcsname}%
         \fi%
      }%
   \fi%
   \forlistcsloop\yquant@env@end@setypositions{\yquant@prefix subcircuits}%
}

\tikzaddtikzonlycommandshortcutlet\yquant\yquant@envunstar
\expandafter\tikzaddtikzonlycommandshortcutlet\csname yquant*\endcsname\yquant@envstar
\tikzaddtikzonlycommandshortcutlet\endyquant\yquant@env@end
\expandafter\tikzaddtikzonlycommandshortcutlet\csname endyquant*\endcsname\yquant@env@end

\protected\def\yquantset{%
   \pgfqkeys{/yquant}%
}
\let\yquant@set=\yquantset%

% In order to allow nested environments and also grouping (without the need to smuggle definitions out of the groups whenever necessary), we count the number of nested environments.
\newcount\yquant@env

% Some commands may be overwritten while a subcircuit is processed, in particular attributes, but also some others. However, within the subcircuit, they need to have their original (un)definition.
\protected\def\yquant@env@reset@commands{%
   \yquant@lang@reset@attrs%
   \yquant@register@reset@multi%
}

\protected\def\yquant@env@substikz@finish{%
   % Rendering pipeline
   \endgroup%
   \global\pgflinewidth=\tikzscope@linewidth\relax%
   \tikz@path@do@at@end%
}

% first undoes the substikz commands, next turns the \path command into a virtual one that does not produce any output.
\protected\def\yquant@env@virtualize@path{%
   \yquant@register@get@y@@expandable%
   \let\path=\tikz@command@path%
   \let\tikz@finish=\yquant@env@substikz@finish%
   \let\tikz@lib@scope@check=\yquant@env@substikz@scopecheck%
   % we will often access the bounding box, which is never transformed
   \pgftransformreset%
}

% substitute the tikz commands (defined in \tikz@installcommands) so that they can be arbitrarily interleaved with yquant code. We patch \path, \scope, \endscope, \stopscope, their internal complements, and also patch \yquantset.
\protected\def\yquant@env@substikz#1{%
   % \tikz@path@do@at@end is called after a path. Hence, it is an ideal candidate to re-invoke \yquant@env@scan. However, it is by default defined to be \tikz@lib@scope@check, and we need this definition for the scopes library to work correctly. But since \tikz@lib@scope@check is also called after a scope and the end of a scope, this is even better. Yet, we need to check whether the scopes library is present or not.
   \let\yquant@env@substikz@scopecheck=\tikz@lib@scope@check%
   \ifx\tikz@lib@scope@check\pgfutil@empty%
      % no, it is not. This is simple.
      \def\tikz@lib@scope@check{\yquant@env@scan}%
   \else%
      % yes, it is. Call it after the special behavior is done.
      \patchcmd\tikz@lib@scope@check{{}}{\yquant@env@scan}\relax{%
         \PackageWarning{yquant.sty}{Patching \string\tikz@lib@scope@check\space failed; you must invoke \string\yquant\space manually after every tikz command to switch back to yquant code.}%
      }%
   \fi%
   % We not only need to re-invoke yquant after the tikz command, but we must also make sure that the tikz command is not actually drawn now, but at the end. However, what happens if some macros are used within the command? Here, we choose to expand the macros to the values they have _now_, but protected (which should prevent bad things for formatting commands). If you find this to be an issue, please report.
   \def\path##1;{%
      \protected@csxappto{\yquant@prefix draw}{%
         \noexpand\path##1;%
      }%
      #1%
   }%
   % no need for \scoped, because it internally calls \scope.
   % We need to hack into \scope, but this is a bit tricky due to its argument handling. In order to get all optional arguments, including the possible animations library, correct, we change \tikz@scope@opt.
   \ifdefined\tikz@scope@opt%
      \let\yquant@env@substikz@scope=\tikz@scope@opt%
      \def\tikz@scope@opt[##1]{%
         \protected@csxappto{\yquant@prefix draw}{%
            \noexpand\tikz@scope@env[{##1}]%
         }%
         \yquant@env@substikz@scope[{##1}]%
      }%
   \else%
      % this is for the arXiv, which has a very outdated version of TikZ
      \let\yquant@env@substikz@scope=\tikz@@scope@env%
      \def\tikz@@scope@env[##1]{%
         \protected@csxappto{\yquant@prefix draw}{%
            \noexpand\tikz@@scope@env[{##1}]%
         }%
         \yquant@env@substikz@scope[{##1}]%
      }%
   \fi%
   \let\yquant@env@substikz@endscope=\endtikz@scope@env%
   \def\endtikz@scope@env{%
      \csgappto{\yquant@prefix draw}{%
         \yquant@env@substikz@endscope%
      }%
      \yquant@env@substikz@endscope%
   }%
   \let\endscope=\endtikz@scope@env%
   \let\stopscope=\endscope%
   % We define \yquantset as a pgfkeys-like macro. Anything else would deteriorate performance badly, as \pgfkeys, \pgfqkeys, or \tikzset are used a lot internally.
   \protected\def\yquantset##1{%
      \protected@csxappto{\yquant@prefix draw}{%
         \noexpand\pgfqkeys{/yquant}{##1}%
      }%
      \pgfqkeys{/yquant}{##1}%
      \yquant@env@scan%
   }%
}

% Scan until the next non-space token is found and execute it as a csname
\def\yquant@env@scan{%
   \begingroup%
      \yquant@env@contscan%
}
\let\yquant@env@scan@=\yquant@env@scan

\protected\def\yquant@env@contscan{%
   \yquant@futurenonspacelet\yquant@env@nextchar\yquant@env@check%
}

\def\yquant@env@rescan{%
   \endgroup%
   \yquant@env@scan%
}

\protected\def\yquant@env@check@{%
   \let\next=\relax%
   % Here we assume standard catcodes for A and [, but our language specification also requires this implicitly.
   \ifx\yquant@env@nextchar[%
      \let\next=\yquant@langhelper@check@attrs%
   \else%
      \ifcat\noexpand\yquant@env@nextchar A% letter
         \let\next=\yquant@langhelper@check@name%
      \else%
         \ifcat\noexpand\yquant@env@nextchar\bgroup%
            \endgroup%
            \let\next=\yquant@env@opengroup%
         \else%
            \ifcat\noexpand\yquant@env@nextchar\egroup%
               \endgroup%
               \let\next=\yquant@env@closegroup%
            \else%
               \ifx\yquant@env@nextchar\par%
                  \let\next=\yquant@env@gobblepar%
               \else%
                  \ifcat\noexpand\yquant@env@nextchar\relax%
                     \endgroup%
                     \let\next=\relax%
                  \else%
                     \PackageError{yquant.sty}%
                        {Invalid yquant syntax: `\meaning\yquant@env@nextchar'}%
                        {Adhere to the specs!}%
                  \fi%
               \fi%
            \fi%
         \fi%
      \fi%
   \fi%
   \next%
}

\protected\def\yquant@env@opengroup{%
   \afterassignment\yquant@env@opengroup@aux%
   \let\@eattoken= %
}

\def\yquant@env@opengroup@aux{%
   \bgroup%
      \csgappto{\yquant@prefix draw}{\begingroup}%
      \yquant@env@scan%
}

\def\yquant@env@closegroup{%
   \csgappto{\yquant@prefix draw}{\endgroup}%
   \aftergroup\yquant@env@scan%
}

\def\yquant@env@gobblepar{%
   \afterassignment\yquant@env@contscan%
   \let\@eattoken= %
}

\def\yquantimport@now#1{%
   \expandafter\yquant\@@input #1\relax%
}

\def\yquantimportcommand{\yquantimport@now}%

\AtBeginDocument{%
   % do we have the import package?
   \ifdefined\@doimport%
      \providecommand\yquantimportpath{./}%
      \def\yquantimportcommand{\@doimport\yquantimport@now{\yquantimportpath}}%
   \fi%
}

\def\yquantimport{%
   \@ifstar{\yquantimport@i{*}}{\yquantimport@i{}}%
}

\def\yquantimport@i#1{%
   \@ifnextchar[{\yquantimport@ii{#1}}{\yquantimport@ii{#1}[]}%
}%

\def\yquantimport@ii#1[#2]#3{%
   \ifpgfpicture%
      \ifnum\yquant@env>0 %
         \begingroup%
            \ifstrequal{#1}{*}{%
               \yquant@env@lazytrue%
            }{%
               \yquant@env@lazyfalse%
            }%
            \ifstrempty{#2}{%
               \yquantimportcommand{#3}%
            }{%
               \scope%
                  \yquantset{#2}%
                  \yquantimportcommand{#3}%
               \endscope%
            }%
         \endgroup%
         \expandafter\expandafter\expandafter\yquant%
      \else%
         \begin{yquant#1}[{#2}]
            \yquantimportcommand{#3}%
         \end{yquant#1}%
      \fi%
   \else%
      \begin{tikzpicture}%
         \begin{yquant#1}[{#2}]
            \yquantimportcommand{#3}%
         \end{yquant#1}%
      \end{tikzpicture}
   \fi%
}

==> yquant-lang.tex <==
% BEGIN_FOLD Attributes
\yquant@langhelper@declare@attr{%
   value/.store in=\yquant@lang@attr@value,%
   after/.code={%
      \yquant@register@get@ids{#1}%
      \let\yquant@lang@attr@after=\yquant@register@get@ids@list%
   },%
   type/.store in=\yquant@lang@attr@type,%
   ancilla/.code={%
      \undef\yquant@lang@attr@input%
      \undef\yquant@lang@attr@output%
   },%
   in/.code={%
      \let\yquant@lang@attr@input=\relax%
      \undef\yquant@lang@attr@output%
   },%
   out/.code={%
      \undef\yquant@lang@attr@input%
      \let\yquant@lang@attr@output=\relax%
   },%
   inout/.code={%
      \let\yquant@lang@attr@input=\relax%
      \let\yquant@lang@attr@output=\relax%
   },%
   frameless/.code={%
      \pgfkeysalso{/yquant/operators/subcircuit/frameless}%
      \appto\yquant@attrs@remaining{,/yquant/operators/subcircuit/frameless}%
   },%
   seamless/.code={%
      \pgfkeysalso{/yquant/operators/subcircuit/seamless}%
      \appto\yquant@attrs@remaining{,/yquant/operators/subcircuit/seamless}%
   },%
   direct control/.code={%
      \let\yquant@lang@attr@directcontrol=\relax%
   },%
   indirect control/.code={%
      \undef\yquant@lang@attr@directcontrol%
   },%
   name mangling/.code={%
      \pgfkeysalso{/yquant/operators/subcircuit/name mangling={#1}}%
      \appto\yquant@attrs@remaining{,/yquant/operators/subcircuit/name mangling={#1}}%
   }%
}
\yquant@langhelper@declare@attr@global{%
   name/.store in=\yquant@lang@attr@name,%
   overlay/.code={%
      \ifstrequal{#1}{true}{%
         \yquant@lang@attr@overlay@multitrue%
         \yquant@lang@attr@overlay@heighttrue%
         \yquant@lang@attr@overlay@depthtrue%
      }{%
         \ifstrequal{#1}{false}{%
            % Why??? This is the default and should always be reset automatically!
            \yquant@lang@attr@overlay@multifalse%
            \yquant@lang@attr@overlay@heightfalse%
            \yquant@lang@attr@overlay@depthfalse%
         }{%
            \pgfqkeys{/yquant/global attrs/overlay}{#1}%
         }%
      }%
   },%
   overlay/.default=true,%
   overlay/multi/.is if=yquant@lang@attr@overlay@multi,%
   overlay/m/.forward to=/yquant/global attrs/overlay/multi,%
   overlay/height/.is if=yquant@lang@attr@overlay@height,%
   overlay/ht/.forward to=/yquant/global attrs/overlay/height,%
   overlay/h/.forward to=/yquant/global attrs/overlay/height,%
   overlay/depth/.is if=yquant@lang@attr@overlay@depth,%
   overlay/dp/.forward to=/yquant/global attrs/overlay/depth,%
   overlay/d/.forward to=/yquant/global attrs/overlay/depth,%
   overlay/single/.code={\pgfkeysalso{%
      /yquant/global attrs/overlay/height={#1},%
      /yquant/global attrs/overlay/depth={#1}%
   }},%
   overlay/single/.default=true,%
   overlay/s/.forward to=/yquant/global attrs/overlay/single,%
}
\newif\ifyquant@lang@attr@overlay@multi%
\newif\ifyquant@lang@attr@overlay@height%
\newif\ifyquant@lang@attr@overlay@depth%

\protected\def\yquant@lang@reset@attrs{%
   \undef\yquant@lang@attr@value%
   \undef\yquant@lang@attr@after%
   \undef\yquant@lang@attr@type%
   \yquant@lang@reset@attrs@inputoutput%
   \let\yquant@lang@attr@name=\empty%
   \yquant@lang@attr@overlay@multifalse%
   \yquant@lang@attr@overlay@heightfalse%
   \yquant@lang@attr@overlay@depthfalse%
}

\protected\def\yquant@lang@reset@attrs@inputoutput{%
   \undef\yquant@lang@attr@input%
   \undef\yquant@lang@attr@output%
}

\protected\def\yquant@lang@reset@attrs@inputoutput@subcircuit{%
   \let\yquant@lang@attr@input=\relax%
   \let\yquant@lang@attr@output=\relax%
}
% END_FOLD

% BEGIN_FOLD Declaration of registers
\yquant@langhelper@declare@command@create{nobit}\yquant@lang@@nobit
\yquant@langhelper@setup@attrs{nobit}{}{ancilla,out}
\def\yquant@lang@@nobit#1{%
   \let\yquant@lang@create@type=\yquant@register@type@none%
   \def\yquant@lang@create@style{initial}% there is no separate style, just duplicate
   \ifdefined\yquant@lang@attr@value%
      \PackageError{yquant.sty}{Placeholder initialization must not have value}%
                   {You must not provide a description for an invisible register.}
   \else%
      \let\yquant@lang@attr@value=\empty%
   \fi%
   \yquant@lang@create@parse@name#1[;%
}

\yquant@langhelper@declare@command@create{qubit}\yquant@lang@@qubit
\yquant@langhelper@setup@attrs{qubit}{}{after,value,ancilla,in,out,inout}
\def\yquant@lang@@qubit#1{%
   \let\yquant@lang@create@type=\yquant@register@type@q%
   \def\yquant@lang@create@style{qubit}%
   \unless\ifdefined\yquant@lang@attr@value%
      \let\yquant@lang@attr@value=\yquant@config@register@default@name%
   \fi%
   \yquant@lang@create@parse@name#1[;%
}

\yquant@langhelper@declare@command@create{cbit}\yquant@lang@@cbit
\yquant@langhelper@setup@attrs{cbit}{}{after,value,ancilla,in,out,inout}
\def\yquant@lang@@cbit#1{%
   \let\yquant@lang@create@type=\yquant@register@type@c%
   \def\yquant@lang@create@style{cbit}%
   \unless\ifdefined\yquant@lang@attr@value%
      \let\yquant@lang@attr@value=\yquant@config@register@default@name%
   \fi%
   \yquant@lang@create@parse@name#1[;%
}

\yquant@langhelper@declare@command@create{qubits}\yquant@lang@@qubits
\yquant@langhelper@setup@attrs{qubits}{}{after,value,ancilla,in,out,inout}
\def\yquant@lang@@qubits#1{%
   \let\yquant@lang@create@type=\yquant@register@type@qs%
   \def\yquant@lang@create@style{qubits}%
   \unless\ifdefined\yquant@lang@attr@value%
      \let\yquant@lang@attr@value=\yquant@config@register@default@name%
   \fi%
   \yquant@lang@create@parse@name#1[;%
}

\def\yquant@lang@create@parse@name#1[#2;{%
   \ifstrempty{#2}{%
      \yquant@lang@create@do#1[1][;%
   }{%
      \yquant@lang@create@do#1[#2;%
   }%
}

\protected\def\yquant@lang@create@do#1[#2]#3[;{%
   % parse length
   \ifstrempty{#3}{%
      \yquant@langhelper@validate\len\count{#2}%
      \ifnum\len<1 %
         \PackageError{yquant.sty}{Invalid register length}%
                      {Valid register lengths are integers greater or equal to one.}%
      \fi%
   }{%
      \PackageError{yquant.sty}{Invalid register name}%
         {Register names must not contain `[' apart from register length indication.}%
   }%
   \edef\reg{\trim@spaces{#1}}%
   % we allow for scattering, so check whether the register already exists
   \ifcsname\yquant@prefix registerhigh@\reg\endcsname%
      \ifyquant@firsttoken+{#2}{%
         \numdef\idx{\csname\yquant@prefix registerhigh@\reg\endcsname+1}%
         \numdef\len{\len+\idx}%
      }{%
         \PackageError{yquant.sty}{Duplicate registers}%
            {Register `\reg' was already defined. Use `\reg[+#2]' with explicit plus symbol to indicate that you want to enlarge the register on purpose.}%
      }%
   \else%
      \def\idx{0}%
   \fi%
   % define text macros
   \ifnum\len=1 %
      \let\regidx=\reg%
   \else%
      \def\regidx{\reg[\idx]}%
   \fi%
   \numdef\yquant@circuit@operator@mintarget{\csname\yquant@prefix registers\endcsname+1}%
   % create the registers
   \begingroup%
      % if we have the after attribute, we start with a discarded wire
      \ifdefined\yquant@lang@attr@after%
         \ifdefined\yquant@lang@attr@input%
            \PackageError{yquant.sty}{An input register cannot be created with `after` attribute}{}%
         \fi%
         \let\yquant@lang@create@type=\yquant@register@type@none%
      \fi%
      \yquant@for \idx := \idx to \numexpr \len -1\relax {%
         \yquant@prepare@create\reg\idx\yquant@lang@create@type%
      }%
   \endgroup%
   % gather details about the created registers
   \letcs\yquant@circuit@operator@maxtarget{\yquant@prefix registers}%
   \numdef\yquant@circuit@operator@numtarget{\yquant@circuit@operator@maxtarget-\yquant@circuit@operator@mintarget+1}%
   \edef\yquant@circuit@operator@targets{%
      \yquant@list@range%
         \yquant@circuit@operator@mintarget%
         \yquant@circuit@operator@maxtarget%
   }%
   \let\yquant@circuit@operator@pctrls=\empty%
   \def\yquant@circuit@operator@minpctrl{2147483647}%
   \def\yquant@circuit@operator@maxpctrl{0}%
   \let\yquant@circuit@operator@numpctrl=\yquant@circuit@operator@maxpctrl%
   \let\yquant@circuit@operator@nctrls=\empty%
   \let\yquant@circuit@operator@minnctrl=\yquant@circuit@operator@minpctrl%
   \let\yquant@circuit@operator@maxnctrl=\yquant@circuit@operator@maxpctrl%
   \let\yquant@circuit@operator@numnctrl=\yquant@circuit@operator@numpctrl%
   \let\yquant@circuit@operator@minctrl=\yquant@circuit@operator@mintarget%
   \let\yquant@circuit@operator@maxctrl=\yquant@circuit@operator@maxtarget%
   % if we have the after attribute, we fake an align gate
   \ifdefined\yquant@lang@attr@after%
      \edef\jointindices{\yquant@circuit@operator@targets\yquant@lang@attr@after}%
      \yquant@circuit@align\jointindices%
      % and we also need to change the wire after the alignment
      \let\yquant@circuit@settype@to=\yquant@lang@create@type%
      \let\yquant@prepare@callback@prepare=\yquant@circuit@settype@prepare%
      \let\yquant@prepare@callback@draw=\yquant@circuit@settype%
      \expandafter\@thirdofthree%
   \else%
      \expandafter\@firstofone%
   \fi%
   % unless there is no name, no text and no after attribute, we now need an init gate
   {%
      \ifx\yquant@lang@attr@value\empty%
         \expandafter\@firstofone%
      \else%
         \expandafter\@secondoftwo%
      \fi%
   }%
   {%
      \ifx\yquant@lang@attr@name\empty%
         \expandafter\@gobble%
      \else%
         \expandafter\@firstofone%
      \fi%
   }%
   {%
      % there are no multi inits in this context
      \preto\yquant@attrs@remaining{internal/move label,}%
      \def\yquant@config@operator@minimum@width{0pt}%
      \unless\ifx\yquant@lang@attr@value\empty%
         % make sure to immediately remove the "clear" marker again if we have a text
         \yquant@for \i := \yquant@circuit@operator@mintarget to \yquant@circuit@operator@maxtarget {%
            \yquant@register@execclear@lastgate{\i}{init}%
         }%
      \fi%
      \expandafter\yquant@prepare%
         \expandafter{\yquant@lang@attr@value}%
         {/yquant/every label, /yquant/every initial label,%
          /yquant/every \yquant@lang@create@style\space label,%
          \ifnum\yquant@compat<2 \ifdefined\yquant@lang@attr@input /yquant/every input label\fi\fi}%
      \unless\ifx\yquant@lang@attr@name\empty%
         \ifnum\len=1 %
            \csxappto{\yquant@prefix draw}%
                     {\yquant@draw@alias{\yquant@lang@attr@name}}%
         \fi%
      \fi%
   }%
}
% END_FOLD

% BEGIN_FOLD Define own gates
\def\yquantdefinegate#1{%
   \ifcsname yquant@lang@#1\endcsname%
      \PackageError{yquant.sty}{Gate redefined}%
                   {The gate `#1' already exists. Use \string\yquantredefinegate\space if you really want to redefine it.}%
   \fi%
   \@ifnextchar[{\yquantdefinegate@i{#1}}%
                {\yquantdefinegate@i{#1}[/yquant/operators/every custom gate]}%
}

% while this command is provided to redefine gates, we do not clear the attributes that were once assigned to the previous one, so gate redefinition is discouraged!
\def\yquantredefinegate#1{%
   \unless\ifcsname yquant@lang@#1\endcsname%
      \PackageError{yquant.sty}{Unknown gate redefined}%
                   {The gate `#1' is unknown and cannot be redefined. Use \string\yquantdefinegate\space to define it.}%
   \fi%
   \@ifnextchar[{\yquantdefinegate@i{#1}}%
                {\yquantdefinegate@i{#1}[/yquant/operators/every custom gate]}%
}

\protected\long\def\yquantdefinegate@i#1[#2]#3{%
   \begingroup%
      \yquant@prepare@ifs@set%
      % usually, we will not be in a tikzpicture here, so all the commands that abbreviate some path operation are undefined!
      \tikz@installcommands%
      % While we want the content to be expanded, protect the most likely TikZ commands - the same ones that we usually substitute in \yquant@env@substikz.
      \protected\def\path{}%
      \let\scoped=\path%
      \let\scope=\path%
      \let\endscope=\path%
      \let\stopscope=\path%
      \protected@edef\yquantdefinegate@do{%
         \endgroup%
         \noexpand\pgfkeys{/yquant/operators/every #1/.code={%
            \yquant@config@operator@subcircuit@mangling@set{%
               \yquant@config@operator@subcircuit@mangling%
            }%
            \noexpand\pgfkeysalso{\unexpanded{#2}}%
         }}%
         \yquant@langhelper@declare@command%
            {#1}%
            \yquant@register@get@multiaslist%
            {%
               \let\noexpand\yquant@lang@attr@value=\expandafter\noexpand\csname yquant@lang@@#1\endcsname%
               \yquant@prepare@subcircuit{/yquant/operators/every #1}%
            }%
         % This does not clear the attributes for redefines, but makes at least sure nothing is marked as required that should not be.
         \yquant@langhelper@setup@attrs{#1}{}{}%
         % Now define the gate's content as a macro
         \def\expandafter\noexpand\csname yquant@lang@@#1\endcsname{%
            #3%
         }%
      }%
   \yquantdefinegate@do%
}

\def\yquantdefinebox#1{%
   \ifcsname yquant@lang@#1\endcsname%
      \PackageError{yquant.sty}{Gate redefined}%
                   {The gate `#1' already exists. Use \string\yquantredefinebox\space if you really want to redefine it.}%
   \fi%
   \yquantdefinebox@{#1}{}%
}

\def\yquantdefinemultibox#1{%
   \ifcsname yquant@lang@#1\endcsname%
      \PackageError{yquant.sty}{Gate redefined}%
                   {The gate `#1' already exists. Use \string\yquantredefinemultibox\space if you really want to redefine it.}%
   \fi%
   \yquantdefinebox@{#1}\yquant@register@get@allowmultitrue%
}

\def\yquantredefinebox#1{%
   \unless\ifcsname yquant@lang@#1\endcsname%
      \PackageError{yquant.sty}{Unknown gate redefined}%
                   {The gate `#1' is unknown and cannot be redefined. Use \string\yquantdefinebox\space to define it.}%
   \fi%
   \yquantdefinebox@{#1}{}%
}

\def\yquantredefinemultibox#1{%
   \unless\ifcsname yquant@lang@#1\endcsname%
      \PackageError{yquant.sty}{Unknown gate redefined}%
                   {The gate `#1' is unknown and cannot be redefined. Use \string\yquantdefinemultibox\space to define it.}%
   \fi%
   \yquantdefinebox@{#1}\yquant@register@get@allowmultitrue%
}

\def\yquantdefinebox@#1#2{%
   \@ifnextchar[{\yquantdefinebox@i{#1}{#2}}%
                {\yquantdefinebox@i{#1}{#2}[/yquant/operators/every box]}%
}

\protected\long\def\yquantdefinebox@i#1#2[#3]#4{%
   \pgfkeys{/yquant/operators/every #1/.style={#3}}%
   \begingroup%
      \yquant@prepare@ifs@set%
      \protected@edef\yquantdefinebox@do{%
         \endgroup%
         \yquant@langhelper@declare@command%
            {#1}%
            {\unexpanded{#2}}%
            {\yquant@prepare{#4}{/yquant/operators/every #1}}%
      }%
      \yquantdefinebox@do%
   \yquant@langhelper@setup@attrs{#1}{}{}%
}
% END_FOLD

% BEGIN_FOLD Box registers
% all-purpose box with arbitrary text
\yquant@langhelper@declare@command%
   {box}%
   \yquant@register@get@allowmultitrue%
   {%
      \expandafter\yquant@prepare%
         \expandafter{\yquant@lang@attr@value}%
         {/yquant/operators/every box}%
   }
\yquant@langhelper@setup@attrs{box}{value}{}

% Hadamard
\yquantdefinebox{h}{$H$}

% Pauli X (or NOT)
\yquantdefinebox{x}[/yquant/operators/every pauli]{$X$}

% Pauli Y
\yquantdefinebox{y}[/yquant/operators/every pauli]{$Y$}

% Pauli Z
\yquantdefinebox{z}[/yquant/operators/every pauli]{$Z$}

% sub-circuit: This is a nested circuit.
\yquant@langhelper@declare@command%
   {subcircuit}%
   \yquant@register@get@multiaslist%
   {%
      \yquant@prepare@subcircuit{/yquant/operators/every subcircuit}%
   }
\yquant@langhelper@setup@attrs{subcircuit}{value}{frameless,seamless,name mangling}
% END_FOLD

% BEGIN_FOLD other geometric shapes
% phase
\yquant@langhelper@declare@command%
   {phase}%
   {}%
   {%
      \edef\cmd{%
         \yquant@prepare%
            {}%
            {/yquant/operators/every phase, label={\unexpanded\expandafter{\yquant@lang@attr@value}}}%
      }%
      \cmd%
   }
\yquant@langhelper@setup@attrs{phase}{value}{}%

% two-qubit controlled x (symmetric notation)
\yquant@langhelper@declare@command%
   {xx}%
   \yquant@register@get@multiassingle%
   {%
      \yquant@prepare%
         {}%
         {/yquant/operators/every xx}%
   }
\yquant@langhelper@setup@attrs{xx}{}{}

% two-qubit controlled phase (symmetric notation)
\yquant@langhelper@declare@command@uncontrolled%
   {zz}%
   \yquant@register@get@multiassingle%
   {%
      \yquant@prepare%
         {}%
         {/yquant/operators/every zz}%
   }
\yquant@langhelper@setup@attrs{zz}{}{}

% slash (pseudo-operator, alternative indication for a bundle)
\yquant@langhelper@declare@command@uncontrolled%
   {slash}%
   {}%
   {%
      % temporarily squeeze most into the separation
      \pgfkeys{%
         /yquant/operator/minimum width=0pt,%
      }%
      \preto\yquant@attrs@remaining{internal/squeeze slash,}%
      \yquant@prepare%
         {}%
         {/yquant/operators/every slash}%
   }
\yquant@langhelper@setup@attrs{slash}{}{}

% swap
\yquant@langhelper@declare@command%
   {swap}%
   \yquant@register@get@multiassingle
   {%
      \yquant@prepare%
         {}%
         {/yquant/operators/every swap}%
   }
\yquant@langhelper@setup@attrs{swap}{}{}

% not
\yquant@langhelper@declare@command%
   {not}%
   {}%
   {%
      \yquant@prepare%
         {}%
         {/yquant/operators/every not}%
   }
\yquant@langhelper@setup@attrs{not}{}{}
% alias to cnot
\yquant@langhelper@declare@command@alias{cnot}{not}
\yquant@langhelper@setup@attrs{cnot}{}{}

% measure
\yquant@langhelper@declare@command@uncontrolled%
   {measure}%
   \yquant@register@get@allowmultitrue%
   {%
      \ifdefined\yquant@lang@attr@type%
         \yquant@register@type@fromstring\yquant@lang@attr@type\yquant@circuit@settype@to%
      \else%
         \let\yquant@circuit@settype@to=\yquant@register@type@c%
      \fi%
      \let\yquant@prepare@callback@prepare=\yquant@circuit@settype@prepare%
      \let\yquant@prepare@callback@draw=\yquant@circuit@settype%
      \unless\ifcsname yquant@lang@attr@value\endcsname%
         \let\yquant@lang@attr@value=\empty%
      \fi%
      \ifdefined\yquant@lang@attr@directcontrol%
         % direct control means that we must defer this operator until the next that has this/these targets as positive controls.
         \expandafter\yquant@prepare@injection%
            \expandafter{\yquant@lang@attr@value}%
            {/yquant/operators/every measure}%
      \else%
         \expandafter\yquant@prepare%
            \expandafter{\yquant@lang@attr@value}%
            {/yquant/operators/every measure}%
      \fi%
   }
\yquant@langhelper@setup@attrs{measure}{}{value,type,direct control,indirect control}

% measure (dmeter)
\yquant@langhelper@declare@command@uncontrolled%
   {dmeter}%
   \yquant@register@get@allowmultitrue%
   {%
      \ifdefined\yquant@lang@attr@type%
         \yquant@register@type@fromstring\yquant@lang@attr@type\yquant@circuit@settype@to%
      \else%
         \let\yquant@circuit@settype@to=\yquant@register@type@c%
      \fi%
      \let\yquant@prepare@callback@prepare=\yquant@circuit@settype@prepare%
      \let\yquant@prepare@callback@draw=\yquant@circuit@settype%
      \unless\ifcsname yquant@lang@attr@value\endcsname%
         \let\yquant@lang@attr@value=\empty%
      \fi%
      \expandafter\yquant@prepare%
         \expandafter{\yquant@lang@attr@value}%
         {/yquant/operators/every dmeter}%
   }
\yquant@langhelper@setup@attrs{dmeter}{}{value,type}
% END_FOLD

% BEGIN_FOLD miscellaneous
\yquant@langhelper@declare@command@uncontrolled%
   {barrier}%
   \yquant@register@get@allowmultitrue%
   {%
      \yquant@prepare%
         {}%
         {/yquant/operators/every barrier}%
   }%
\yquant@langhelper@setup@attrs{barrier}{}{}

\yquant@langhelper@declare@command@uncontrolled%
   {correlate}%
   {%
      % do not call \yquant@register@get@multiassingle, we do not want to install a different multi line style!
      \yquant@register@get@allowmultitrue%
      \let\yquant@register@multi@splitparts=\yquant@register@multi@splitparts@sepall%
   }{%
      \yquant@prepare%
         {}%
         {/yquant/operators/every wave}%
   }
\yquant@langhelper@setup@attrs{correlate}{}{}

\yquant@langhelper@declare@command@uncontrolled%
   {align}%
   {}%
   {%
      \yquant@circuit@align\yquant@circuit@operator@targets%
   }
\yquant@langhelper@setup@attrs{align}{}{}

\yquant@langhelper@declare@command@uncontrolled%
   {hspace}%
   {%
      \yquant@langhelper@validate\amount\dimen\yquant@lang@attr@value%
   }{%
      \yquant@circuit@hspace\yquant@circuit@operator@targets\amount%
   }
\yquant@langhelper@setup@attrs{hspace}{value}{}

\yquant@langhelper@declare@command@uncontrolled%
   {discard}%
   {}%
   {%
      \let\yquant@circuit@settype@to=\yquant@register@type@none%
      \yquant@circuit@actonwires%
         \yquant@circuit@settype@prepare%
         \yquant@circuit@settype%
         \yquant@circuit@operator@targets%
         {}%
   }
\yquant@langhelper@setup@attrs{discard}{}{}

\yquant@langhelper@declare@command@uncontrolled%
   {init}%
   {%
      \yquant@register@get@allowmultitrue%
      % we will count how many registers contain the "clean" flag, and only if this is equal to the number of targets, we apply the shift.
      \count8=0 %
   }%
   {%
      \ifdefined\yquant@lang@attr@type%
         \yquant@register@type@fromstring\yquant@lang@attr@type\yquant@circuit@settype@to%
      \else%
         % We don't know which type is desired. Scan all target registers and use the first wire that is available as a type.
         \let\yquant@circuit@settype@to=\yquant@register@type@none%
         \forlistloop\yquant@lang@@init@loop\yquant@circuit@operator@targets%
         \ifx\yquant@circuit@settype@to\yquant@register@type@none%
            % now we don't have a clue; assume it's a qubit
            \let\yquant@circuit@settype@to=\yquant@register@type@q%
         \fi%
         \edef\yquant@lang@attr@type{%
            \yquant@register@type@tostring\yquant@circuit@settype@to%
         }%
      \fi%
      \let\yquant@prepare@callback@prepare=\yquant@circuit@settype@prepare%
      \let\yquant@prepare@callback@draw=\yquant@circuit@settype%
      \let\yquant@prepare@multi=\yquant@prepare@multiinit%
      \ifnum\count8=\numexpr\yquant@circuit@operator@maxctrl-\yquant@circuit@operator@minctrl+1\relax%
         \def\yquant@config@operator@minimum@width{0pt}%
         \preto\yquant@attrs@remaining{internal/move label,}%
         \edef\cmd{%
            \yquant@prepare%
               {\unexpanded\expandafter{\yquant@lang@attr@value}}%
               {/yquant/every label, /yquant/every initial label,%
                /yquant/every \yquant@lang@attr@type\space label}%
         }%
      \else%
         \edef\cmd{%
            \yquant@prepare%
               {\unexpanded\expandafter{\yquant@lang@attr@value}}%
               {/yquant/every label, /yquant/every \yquant@lang@attr@type\space label}%
         }%
      \fi%
      \cmd%
   }
\yquant@langhelper@setup@attrs{init}{value}{type}

\protected\def\yquant@lang@@init@loop#1{%
   \ifyquant@firsttoken\yquant@register@multi{#1}{%
      \let\yquant@register@multi@contiguous=\yquant@lang@@init@multi@@extract%
      \@fifthoffive#1%
      % we should reset multi@contiguous to the original command; but this is really just a placeholder. As long as it is \protected, everything is fine.
   }{%
      \edef\yquant@circuit@settype@to{\yquant@register@get@type{#1}}%
   }%
   \unless\ifx\yquant@circuit@settype@to\yquant@register@type@none%
      \expandafter\listbreak%
   \fi%
}

\protected\def\yquant@lang@@init@multi@@extract#1#2#3{%
   \yquant@for \yquant@i := #1 to #2 {%
      \edef\yquant@circuit@settype@to{\yquant@register@get@type\yquant@i}%
      \unless\ifx\yquant@circuit@settype@to\yquant@register@type@none%
         \expandafter\yquant@for@break%
      \fi%
   }%
}

\yquant@langhelper@declare@command@uncontrolled%
   {output}%
   \yquant@register@get@allowmultitrue%
   \yquant@circuit@output%
\yquant@langhelper@setup@attrs{output}{value}{}

\yquant@langhelper@declare@command@uncontrolled%
   {inspect}%
   \yquant@register@get@allowmultitrue%
   {%
      \expandafter\yquant@prepare%
         \expandafter{\yquant@lang@attr@value}%
         {/yquant/operators/every inspect}%
   }
\yquant@langhelper@setup@attrs{inspect}{value}{}

\yquant@langhelper@declare@command@uncontrolled%
   {settype}%
   {}%
   {%
      \yquant@register@type@fromstring\yquant@lang@attr@value\yquant@circuit@settype@to%
      \yquant@circuit@actonwires%
         \yquant@circuit@settype@prepare%
         \yquant@circuit@settype%
         \yquant@circuit@operator@targets%
         {}%
   }
\yquant@langhelper@setup@attrs{settype}{value}{}

\ifnum\yquant@compat<2 %
   \def\yquant@lang@setwire{%
      \PackageWarning{yquant.sty}{`setwire' gate is deprecated as of yquant 0.1.2. Use `settype' instead.}%
      \yquant@lang@settype%
   }
   \yquant@langhelper@setup@attrs{setwire}{value}{}
\fi

\yquant@langhelper@declare@command@uncontrolled%
   {setstyle}%
   {}%
   {%
      \yquant@circuit@actonwires%
         \@gobbletwo%
         \yquant@circuit@setstyle%
         \yquant@circuit@operator@targets%
         {{\yquant@lang@attr@value}}%
   }
\yquant@langhelper@setup@attrs{setstyle}{value}{}

\yquant@langhelper@declare@command@uncontrolled%
   {addstyle}%
   {}%
   {%
      \yquant@circuit@actonwires%
         \@gobbletwo%
         \yquant@circuit@addstyle%
         \yquant@circuit@operator@targets%
         {{\yquant@lang@attr@value}}%
   }
\yquant@langhelper@setup@attrs{addstyle}{value}{}
% END_FOLD

==> yquant-langhelper.tex <==
% BEGIN_FOLD Parsing attributes
\let\yquant@langhelper@list@attrs=\empty
% gatecallback is called by every "standard" gate (which does not include the "create" type of gates)
\let\yquant@langhelper@gatecallback=\@gobble

\protected\long\def\yquant@langhelper@check@attrs[#1]{%
   \appto\yquant@langhelper@list@attrs{#1,}%
   \yquant@env@contscan%
}

% shorthands for declaring attributes
\protected\def\yquant@langhelper@declare@attr{%
   \pgfqkeys{/yquant/all attrs}%
}

\protected\def\yquant@langhelper@declare@attr@global{%
   \pgfqkeys{/yquant/global attrs}%
}

\pgfkeys{%
   /yquant/attr filter handler/.code={%
      \let\yquant@langhelper@filter@@name=\pgfkeyscurrentkeyRAW%
      \let\yquant@langhelper@filter@@value=\pgfkeyscurrentvalue%
      % the key was filtered out, i.e., it is neither a local nor a global attribute.
      \pgfkeysinterruptkeyfilter%
         % execute it in /yquant, if it exists there
         \pgfqkeys{/yquant}{\yquant@langhelper@filter@@name/.try/.expand once=\yquant@langhelper@filter@@value}%
         \ifpgfkeyssuccess%
            \eappto#1{%
               ,/yquant/\unexpanded\expandafter{\yquant@langhelper@filter@@name}%
                  \unless\ifx\yquant@langhelper@filter@@value\pgfkeysnovalue@text%
                     ={\unexpanded\expandafter{\yquant@langhelper@filter@@value}}%
                  \fi%
            }%
         \else%
            \pgfkeys{/yquant/operator style/.expanded=%
               {\unexpanded\expandafter{\yquant@langhelper@filter@@name}=%
                  {\unexpanded\expandafter{\yquant@langhelper@filter@@value}}%
               }%
            }%
            \eappto#1{%
               ,/yquant/operator style={\unexpanded\expandafter{\yquant@langhelper@filter@@name}%
                  \unless\ifx\yquant@langhelper@filter@@value\pgfkeysnovalue@text%
                     ={\unexpanded\expandafter{\yquant@langhelper@filter@@value}}%
                  \fi%
               }%
            }%
         \fi%
      \endpgfkeysinterruptkeyfilter%
   },%
   /pgf/key filters/attr filter/.code={%
      % we need to capture every non-attribute (which means filtering them out).
      \expandafter\ifyquant@beginswith\expandafter{\pgfkeyscurrentkey}{/yquant/attrs/}{%
         % the key is in /yquant/attrs. Does it actually exist (but not as a handler, which would define non-existing keys)?
         \if\pgfkeyscasenumber1%
            \pgfkeysfiltercontinuetrue%
         \else%
            \if\pgfkeyscasenumber2%
               \pgfkeysfiltercontinuetrue%
            \else%
               % 0 or 3 for our case means non-existing - now we need to check whether we can find it in the global attributes.
               \pgfkeysifassignable{/yquant/global attrs/\pgfkeyscurrentkeyRAW}{%
                  \pgfkeysfiltercontinuetrue%
               }{%
                  % it is not, so it is not a known attribute for this operator. Filter.
                  \pgfkeysfiltercontinuefalse%
               }%
            \fi%
         \fi%
      }{%
         % the key is not in /yquant/attrs. Is it a global attribute (usually, the user should not access this explicitly, but let's be tolerant here)?
         \expandafter\ifyquant@beginswith\expandafter{\pgfkeyscurrentkey}{/yquant/global attrs/}{%
            % the key is in /yquant/global attrs. Does it actually exist?
            \if\pgfkeyscasenumber1%
               \pgfkeysfiltercontinuetrue%
            \else%
               \if\pgfkeyscasenumber2%
                  \pgfkeysfiltercontinuetrue%
               \else%
                  % no - that's it.
                  \pgfkeysfiltercontinuefalse%
               \fi%
            \fi%
         }{%
            % the key is no known attribute
            \pgfkeysfiltercontinuefalse%
         }%
      }%
   },%
   /yquant/attr filter/.style={%
      /pgf/key filters/attr filter/.install key filter,%
      /yquant/attr filter handler/.install key filter handler=\yquant@attrs@remaining%
   }%
}

% specifies which attributes can be used for a given command
% #1: command name
% #2: comma-separated list of required attrs
% #3: comma-separated list of optional attrs
\protected\def\yquant@langhelper@setup@attrs#1#2#3{%
   \begingroup%
      \lowercase{\edef\cmd{#1}}%
      \edef\keyscmd{%
         \noexpand\pgfkeyslet{/yquant/attrs/\cmd/.unknown/.@cmd}%
                             \yquant@langhelper@setup@attrs@unknown%
      }%
      \let\keysset=\relax%
      \let\keyscheck=\relax%
      \def\do##1{%
         \eappto\keyscmd{%
            \noexpand\pgfkeysdef{/yquant/attrs/\cmd/##1}{%
               \unexpanded{%
                  \cslet{yquant@langhelper@attrs@req@##1}\relax%
                  \pgfkeysinterruptkeyfilter%
                     \pgfkeys{/yquant/all attrs/##1={####1}}%
                  \endpgfkeysinterruptkeyfilter%
               }%
            }%
         }%
         \eappto\keysset{%
            \def\expandafter\noexpand\csname yquant@langhelper@attrs@req@##1\endcsname{%
               \yquant@langhelper@setup@attrs@missing{##1}%
            }%
         }%
         \expandafter\appto\expandafter\keyscheck%
            \csname yquant@langhelper@attrs@req@##1\endcsname%
      }%
      \docsvlist{#2}%
      \global\cslet{yquant@langhelper@setup@attrs@set@\cmd}\keysset%
      \global\cslet{yquant@langhelper@setup@attrs@check@\cmd}\keyscheck%
      \def\do##1{%
         \eappto\keyscmd{%
            \noexpand\pgfkeysdef{/yquant/attrs/\cmd/##1}{%
               \unexpanded{%
                  \pgfkeysinterruptkeyfilter%
                     \pgfkeys{/yquant/all attrs/##1={####1}}%
                  \endpgfkeysinterruptkeyfilter%
               }%
            }%
         }%
      }%
      \docsvlist{#3}%
      \expandafter%
   \endgroup%
   \keyscmd%
}

\protected\def\yquant@langhelper@setup@attrs@unknown#1\pgfeov{%
   % This is in its essence /.search also={/yquant/global attrs}, but with filtering interrupted
   \pgfkeysinterruptkeyfilter%
      \ifpgfkeysaddeddefaultpath%
         % only process keys for which no full path has been provided:
         \pgfkeyssuccessfalse%
         \let\pgfkeys@searchalso@name=\pgfkeyscurrentkeyRAW%
         % We interrupt the filtering process because we only want to append the very top-level command to the remaining-macro.
         \unless\ifpgfkeyssuccess%
            \pgfqkeys{/yquant/global attrs}%
                     {\pgfkeys@searchalso@name={#1}}%
         \fi%
      \else%
         % the /.search also implementation defines this in an unexpanded macro, which is then executed. Any reason?
         \pgfkeysvalueof{/handlers/.unknown/.@cmd}#1\pgfeov%
      \fi%
   \endpgfkeysinterruptkeyfilter%
}

\protected\def\yquant@langhelper@setup@attrs@missing#1{%
   \PackageError{yquant.sty}{Required attribute `#1' missing}%
      {You used a command that requires specifying the attribute `#1'.}%
}%
% END_FOLD

% BEGIN_FOLD Parsing command itself
\protected\def\yquant@langhelper@check@name#1 {%
   \lowercase{\edef\cmd{#1}}%
   \unless\ifcsname yquant@lang@\cmd\endcsname%
      \PackageError{yquant.sty}{Unsupported yquant command: `#1'}%
         {You used a command that is unknown to yquant.}%
   \fi%
   \edef\yquant@langhelper@cmd@original{#1}%
   % Provide the association with the correct attributes
   \csname yquant@langhelper@setup@attrs@set@\cmd\endcsname%
   % For "ordinary" uses of the quotes library (without additional options), it would be better not to load the library now, since then the original text (everything in quotes) is just appended to /yquant/operator style. However, then uses with options will break the pgfkeys parser, as they are invalid. For this reason, we must enable the quotes library already at this state, with the consequence that we store the longer version, i.e., the output of the quotes-parsed expression instead.
   \tikz@enable@node@quotes%
   % execute them
   \let\yquant@attrs@remaining=\empty%
   \unless\ifx\yquant@langhelper@list@attrs\empty%
      \edef\yquant@langhelper@list@attrs{%
         \noexpand\pgfqkeysfiltered%
            {/yquant/attrs/\cmd}%
            {\unexpanded\expandafter{\yquant@langhelper@list@attrs}}%
      }%
      \pgfkeys{/yquant/attr filter}%
      \yquant@langhelper@list@attrs%
      \let\yquant@langhelper@list@attrs=\empty% required for nested environments
   \fi%
   % If there was an argument, set it
   \@ifnextchar\bgroup%
      \yquant@langhelper@check@name@i%
      \yquant@langhelper@check@name@ii%
}

\protected\long\def\yquant@langhelper@check@name@i#1{%
   \ifdefined\yquant@lang@attr@value%
      \PackageWarning{yquant.sty}{Node content given explicitly and as an attribute. Using the explicit value.}%
   \fi%
   \def\yquant@lang@attr@value{#1}%
   \let\yquant@langhelper@attrs@req@value=\relax%
   \yquant@langhelper@check@name@ii%
}

\protected\def\yquant@langhelper@check@name@ii{%
   % Check all necessary attributes were given.
   \csname yquant@langhelper@setup@attrs@check@\cmd\endcsname%
   % Finally execute the command
   \letcs\cmd{yquant@lang@\cmd}%
   \yquant@langhelper@declare@command@@parse%
}
% END_FOLD

% BEGIN_FOLD Declarations
\newif\ifyquant@langhelper@execclear@lastgate
% Defining commands that accept registers and take an optional value
% #1: name of the argument
% #2: command (sequence) that is to be called before the target macros are filled
% #3: command (sequence) that is to be called after the target macros are filled
\protected\def\yquant@langhelper@declare@command#1#2#3{%
   \begingroup%
      \lowercase{\edef\cmd{#1}}%
      \long\protected\csxdef{yquant@lang@\cmd}##1##2##3{%
         \noexpand\yquant@langhelper@gatecallback{\cmd}%
         \noexpand\yquant@langhelper@execclear@lastgatetrue%
         \unexpanded{#2}%
         \yquant@circuit@operator{##1}{##2}{##3}%
         \noexpand\ifyquant@langhelper@execclear@lastgate%
            \yquant@for \noexpand\i := \noexpand\yquant@circuit@operator@minctrl to \noexpand\yquant@circuit@operator@maxctrl {%
               \yquant@register@execclear@lastgate{\noexpand\i}{\cmd}%
            }%
         \noexpand\fi%
         \unexpanded{#3}%
      }%
   \endgroup%
}

% Defining commands that accept registers and take an optional value, but don't allow for controls
% #1: name of the argument
% #2: command (sequence) that is to be called before the target macros are filled
% #3: command (sequence) that is to be called after the target macros are filled
\protected\def\yquant@langhelper@declare@command@uncontrolled#1#2#3{%
   \begingroup%
      \lowercase{\edef\cmd{#1}}%
      \long\protected\csxdef{yquant@lang@\cmd}##1##2##3{%
         \noexpand\ifstrempty{##1}\relax{%
            \noexpand\PackageError{yquant.sty}{Positive controls are not allowed for the command `\cmd`}{}%
         }%
         \noexpand\ifstrempty{##2}\relax{%
            \noexpand\PackageError{yquant.sty}{Negative controls are not allowed for the command `\cmd`}{}%
         }%
         \noexpand\yquant@langhelper@gatecallback{\cmd}%
         \noexpand\yquant@langhelper@execclear@lastgatetrue%
         \unexpanded{#2}%
         \yquant@circuit@operator{}{}{##3}%
         \noexpand\ifyquant@langhelper@execclear@lastgate%
            \yquant@for \noexpand\i := \noexpand\yquant@circuit@operator@minctrl to \noexpand\yquant@circuit@operator@maxctrl {%
               \yquant@register@execclear@lastgate{\noexpand\i}{\cmd}%
            }%
         \noexpand\fi%
         \unexpanded{#3}%
      }%
   \endgroup%
}

% Defining commands that accept an undefined register and take an optional value, but don't allow for controls
% #1: name of the argument
% #2: macro that is to be called with parameter #1 being the name of the register
\protected\def\yquant@langhelper@declare@command@create#1#2{%
   \begingroup%
      \lowercase{\edef\cmd{#1}}%
      \long\protected\csxdef{yquant@lang@\cmd}##1##2{%
         \noexpand\ifstrempty{##1}\relax{%
            \noexpand\PackageError{yquant.sty}{Positive controls are not allowed for the command `\cmd`}{}%
         }%
         \noexpand\ifstrempty{##2}\relax{%
            \noexpand\PackageError{yquant.sty}{Negative controls are not allowed for the command `\cmd`}{}%
         }%
         \noexpand#2%
      }%
   \endgroup%
}

% make #1 an identical command to #2 (does not copy attributes)
\protected\def\yquant@langhelper@declare@command@alias#1#2{%
   \global\csletcs{yquant@lang@#1}{yquant@lang@#2}%
}

\long\def\yquant@langhelper@declare@command@@parse#1;{%
   \yquant@langhelper@declare@command@@extract@nctrl#1~;%
   \yquant@env@rescan%
}

\def\yquant@langhelper@declare@command@@extract@nctrl#1~#2;{%
   \ifstrempty{#2}{%
      \yquant@langhelper@declare@command@@extract@pctrl#1|~~;%
   }{%
      \yquant@langhelper@declare@command@@extract@pctrl#1|~#2;%
   }%
}

\def\yquant@langhelper@declare@command@@extract@pctrl#1|#2~#3~;{%
   \ifstrempty{#2}{%
      \yquant@langhelper@declare@command@@exec#1||~#3;%
   }{%
      \yquant@langhelper@declare@command@@exec#1|#2~#3;%
   }%
}

\protected\def\yquant@langhelper@declare@command@@exec#1|#2|~#3;{%
   \edef\params{%
      {\trim@spaces{#2}}%
      {\trim@spaces{#3}}%
      {\trim@spaces{#1}}%
   }%
   \expandafter\cmd\params%
}
% END_FOLD

% shorthands for validation of property values
% #1: a macro that will contain the sanitized value
% #2: a TeX register type: most likely \count, \dimen
% #3: a string to be checked
% This macro is not expandable.
\protected\def\yquant@langhelper@validate#1#2#3{%
   \begingroup%
      \afterassignment\yquant@langhelper@validate@i%
      #2 255=#3\relax\yquant@end%
      \unless\ifvalid%
         \PackageError{yquant.sty}{Invalid property value: `#3'}%
            {The value must be assignable to a \protect#2 register.}%
      \fi%
      \expandafter%
   \endgroup%
   \expandafter\def\expandafter#1\expandafter{\the#2 255}%
}

\def\yquant@langhelper@validate@relax{\relax}
\protected\def\yquant@langhelper@validate@i#1\relax#2\yquant@end{%
   % if the valid value was not user-delimited by \relax, #1 and #2 are empty
   % if the valid value was user-delimited by \relax, #1 is empty and #2 is \relax
   \let\ifvalid=\iffalse%
   \ifstrempty{#1}{%
      \def\tmp{#2}%
      \ifx\empty\tmp%
         \csletcs{ifvalid}{iftrue}%
      \else%
         \ifx\yquant@langhelper@validate@relax\tmp%
            \csletcs{ifvalid}{iftrue}%
         \fi%
      \fi%
   }\relax%
   % eat the rest (which should be empty anyway)
}

==> yquant-prepare.tex <==
% Most drawing operations will be realized through nodes
\let\yquant@prepare@callback@prepare=\@gobble
\let\yquant@prepare@callback@draw=\@gobble%

% #1: register name
% #2: register index
% #3: register type
\protected\def\yquant@prepare@create#1#2#3{%
   \ifdefined\yquant@lang@attr@input%
      \expandafter\yquant@list@gdequeue\csname\yquant@prefix parameters\endcsname\outermap%
      \ifx\outermap\empty%
         \PackageError{yquant.sty}{Invalid subcircuit parameter count}%
                      {No outer register available for input register `#1[#2]`.}%
      \fi%
      \begingroup%
         \let\yquant@prefix=\yquant@parent %
         \unless\if#3\yquant@register@get@type\outermap%
            \PackageError{yquant.sty}%
                         {Subcircuit expects wire of type `\yquant@register@type@tostring#3', but got `\yquant@register@type@tostring{\yquant@register@get@type\outermap}'}%
                         {Outer and inner wire types must match for input wire `#1[#2]`.}%
         \fi%
      \endgroup%
      \unless\ifdefined\yquant@lang@attr@output%
         \listcsxadd{\yquant@prefix inonly}%
                    {\the\numexpr\csname\yquant@prefix registers\endcsname+1\relax}%
      \fi%
      \yquant@register@alias{#3}{#1}{#2}\outermap%
   \else%
      \ifdefined\yquant@lang@attr@output%
         \expandafter\yquant@list@gdequeue\csname\yquant@prefix parameters\endcsname\outermap%
         \ifx\outermap\empty%
            \PackageError{yquant.sty}{Invalid subcircuit parameter count}%
                         {No outer register available for output register `#1[#2]`.}%
         \fi%
         \begingroup%
            \let\yquant@prefix=\yquant@parent%
            \unless\if\yquant@register@type@none\yquant@register@get@type\outermap%
               \PackageError{yquant.sty}%
                            {Subcircuit expects discarded wire, got `\yquant@register@type@tostring{\yquant@register@get@type\outermap}'}%
                            {Outer wire must be discarded before being acceptable for output-only register `#1[#2]`.}%
            \fi%
         \endgroup%
         \yquant@register@alias{#3}{#1}{#2}\outermap%
      \else%
         \yquant@register@define{#3}{#1}{#2}%
      \fi%
   \fi%
   % we must be allowed to change the wire types during preparation for various reasons, so we need to reset it here (TODO: can we eliminate all those reasons?)
   \csxappto{\yquant@prefix draw}{%
      \yquant@draw@init{\csname\yquant@prefix registers\endcsname}{#3}%
   }%
}

% generic shape of an operator
% #1: value
% #2: tikz options that select the correct shape
\protected\long\def\yquant@prepare#1#2{%
   \yquant@sort@clear%
   \def\yquant@prepare@injectcontrols@count{0}%
   \def\idx{0}%
   \yquant@prepare@ifs@direct%
   \dimen2=\yquant@config@operator@minimum@width%
   \ifyquant@circuit@operator@hasControls%
      \edef\yquant@prepare@list{%
         \yquant@list@range%
            \yquant@circuit@operator@minctrl%
            \yquant@circuit@operator@maxctrl%
      }%
   \else%
      \let\yquant@prepare@list=\empty%
   \fi%
   % BEGIN_FOLD register
   \def\do##1{%
      \ifx\yquant@lang@attr@name\empty%
         \let\nodename=\empty%
      \else%
         \edef\nodename{\yquant@lang@attr@name-\idx}%
      \fi%
      \ifyquant@firsttoken\yquant@register@multi{##1}{%
         \yquant@prepare@multi{#1}{#2}{##1}%
      }{%
         \yquant@prepare@single{#1}{#2}{##1}%
      }%
         \expandafter%
      \endpgfinterruptboundingbox%
      \expandafter\dimen\expandafter0\expandafter=%
         \the\dimexpr\pgf@picmaxx-\pgf@picminx\relax\relax%
      \ifdim\dimen0>\dimen2 %
         \dimen2=\dimen0 %
      \fi%
      \numdef\idx{\idx+1}%
   }%
   \dolistloop\yquant@circuit@operator@targets%
   % END_FOLD
   \yquant@prepare@controls%
   \yquant@prepare@finalize{#1}{#2}%
}

\newcount\yquant@prepare@injections
% generic shape of an operator - but delayed to some later point
% #1: value
% #2: tikz options that select the correct shape
\protected\long\def\yquant@prepare@injection#1#2{%
   \global\advance\yquant@prepare@injections by 1 % we just keep increasing, doesn't really matter
   \edef\yquant@draw@group{\yquant@draw@injectiongroup{\the\yquant@prepare@injections}}%
   \def\yquant@draw@endgroup{\noexpand\yquant@draw@endinjectiongroup}%
   \yquant@prepare{#1}{#2}%
   \csxdef{yquant@prepare@@injection@\the\yquant@prepare@injections}{%
      {\the\dimen2}{\unexpanded\expandafter{\yquant@circuit@operator@targets}}%
   }%
   \forlistloop\yquant@prepare@injection@loop\yquant@circuit@operator@targets%
}

\protected\def\yquant@prepare@injection@loop#1{%
   \ifyquant@firsttoken\yquant@register@multi{#1}{%
      \edef\first{\@secondoffive#1}%
      \edef\last{\@thirdoffive#1}%
      \yquant@for \i := \first to \last {%
         \yquant@register@set@lastgate\i{%
            % we only need this once, but it may be called multiple times if acting on multiple registers
            \noexpand\ifcsname yquant@prepare@@injection@\the\yquant@prepare@injections\noexpand\endcsname%
               % first check whether this is valid - i.e., the list of targets for this measurement is in fact a subset of the list of positive controls for the next operation
               \ifyquant@registersubset%
                  {\unexpanded\expandafter{\yquant@circuit@operator@targets}}%
                  {\noexpand\yquant@circuit@operator@pctrls}{%
                  \yquant@prepare@inject{\the\yquant@prepare@injections}%
               }{%
                  \yquant@prepare@inject@discard{\the\yquant@prepare@injections}%
               }%
               \yquant@prepare@injection@clean{\first}{\last}%
            \noexpand\fi
            \noexpand\@gobble%
         }%
      }%
   }{%
      \yquant@register@set@lastgate{#1}{%
         \noexpand\ifcsname yquant@prepare@@injection@\the\yquant@prepare@injections\noexpand\endcsname%
            % first check whether this is valid - i.e., the list of targets for this measurement is in fact a subset of the list of positive controls for the next operation
            \ifyquant@registersubset%
               {\unexpanded\expandafter{\yquant@circuit@operator@targets}}%
               {\noexpand\yquant@circuit@operator@pctrls}{%
               \yquant@prepare@inject{\the\yquant@prepare@injections}%
            }{%
               \yquant@prepare@inject@discard{\the\yquant@prepare@injections}
            }%
         \noexpand\fi%
         \noexpand\@gobble%
      }%
   }%
}

\protected\def\yquant@prepare@injection@clean#1#2{%
   \yquant@for \i := #1 to #2 {%
      \yquant@register@set@lastgate\i{}%
   }%
}

\protected\def\yquant@prepare@inject#1{%
   \letcs\yquant@prepare@inject@@data{yquant@prepare@@injection@#1}%
   \csgundef{yquant@prepare@@injection@#1}%
   \dimen0=\expandafter\@firstoftwo\yquant@prepare@inject@@data\relax%
   \let\@tmpconti=\yquant@register@multi@contiguous%
   \protected\def\yquant@register@multi@contiguous##1##2{%
      \yquant@for \i := ##1 to ##2 {%
         \cslet{yquant@prepare@replacecontrol@\i}\empty%
      }%
   }%
   \expandafter\expandafter\expandafter\etb@forlistloop%
      \expandafter\expandafter\expandafter{%
      \expandafter\@secondoftwo%
      \yquant@prepare@inject@@data%
   }{\yquant@prepare@inject@loop{#1}}%
   \let\yquant@register@multi@contiguous=\@tmpconti%
}

\protected\def\yquant@prepare@inject@loop#1#2{%
   \ifyquant@firsttoken\yquant@register@multi{#2}{%
      \@fifthoffive#2% this clears all the actions for the individual contiguous slices
      % but we need to do something for the first register
      \csedef{yquant@prepare@replacecontrol@\@secondoffive#2}{%
         \noexpand\ifdim\the\dimen0>\dimen2 %
            \dimen2=\the\dimen0 \relax%
         \noexpand\fi%
         \yquant@sort@eadd{%
            \yquant@draw@inject{#1}%
         }
      }%
   }{%
      \csedef{yquant@prepare@replacecontrol@#2}{%
         \noexpand\ifdim\the\dimen0>\dimen2 %
            \dimen2=\the\dimen0 \relax%
         \noexpand\fi%
         \yquant@sort@eadd{%
            \yquant@draw@inject{#1}%
         }%
      }%
   }%
}

\protected\def\yquant@prepare@inject@discard#1{%
   \csgappto{\yquant@prefix draw}{%
      \yquant@draw@inject@outer{#1}%
   }%
   \csgundef{yquant@prepare@@injection@#1}%
}

\def\yquant@prepare@sort#1#2{%
   \yquant@prepare@sort@aux#1\relax#2\relax%
      \expandafter\@firstoftwo%
   \else%
      \expandafter\@secondoftwo%
   \fi%
}

\def\yquant@prepare@sort@aux#1#2#3\relax#4#5#6\relax{%
   \unless\ifnum#2>#5\relax%
}

\protected\def\yquant@prepare@controls@loop#1#2{%
   \ifx\yquant@lang@attr@name\empty%
      \let\nodename=\empty%
   \else%
      \edef\nodename{\yquant@lang@attr@name-#1\idx}%
   \fi%
   \ifcsname yquant@prepare@replacecontrol@#2\endcsname%
      \ifcsempty{yquant@prepare@replacecontrol@#2}\relax{%
         % do something unorthodox
         \csname yquant@prepare@replacecontrol@#2\endcsname%
         \numdef\idx{\idx+1}%
         \unless\ifdefined\yquant@prepare@controltype%
            \edef\yquant@prepare@controltype{#2}%
         \fi%
      }%
   \else%
      \yquant@sort@eadd{%
         \expandafter\noexpand\csname yquant@draw@#1control\endcsname%
            {#2}% register index
            {\nodename}%
      }%
      \numdef\idx{\idx+1}%
      \unless\ifdefined\yquant@prepare@controltype%
         \edef\yquant@prepare@controltype{#2}%
      \fi%
   \fi%
}

\protected\def\yquant@prepare@controls{%
   \ifyquant@circuit@operator@hasControls%
      \def\idx{0}%
      \forlistloop{\yquant@prepare@controls@loop p}\yquant@circuit@operator@pctrls%
      \def\idx{0}%
      \forlistloop{\yquant@prepare@controls@loop n}\yquant@circuit@operator@nctrls%
      \unless\ifdefined\yquant@prepare@controltype%
         \PackageError{yquant.sty}{Internal inconsistency detected}%
                      {Controlled action without controls found.}%
      \fi%
   \fi%
}

\ifnum\yquant@compat>1 %
   \expandafter\@firstoftwo
\else
   \expandafter\@secondoftwo
\fi{
   \def\yquant@prepare@ifs@Ifnum{\noexpand\ifnum}
   \def\yquant@prepare@ifs@Ifcase{\noexpand\ifcase}
   \def\yquant@prepare@ifs@Or{\noexpand\or}
   \def\yquant@prepare@ifs@Else{\noexpand\else}
   \def\yquant@prepare@ifs@Fi{\noexpand\fi}
   \def\yquant@prepare@ifs@Unless{\noexpand\unless}
   \def\yquant@prepare@ifs@The{\noexpand\the}
   \protected\def\yquant@prepare@ifs@set{%
      \let\Ifnum=\yquant@prepare@ifs@Ifnum%
      \let\Ifcase=\yquant@prepare@ifs@Ifcase%
      \let\Or=\yquant@prepare@ifs@Or%
      \let\Else=\yquant@prepare@ifs@Else%
      \let\Fi=\yquant@prepare@ifs@Fi%
      \let\Unless=\yquant@prepare@ifs@Unless%
      \let\The=\yquant@prepare@ifs@The%
   }
   \protected\def\yquant@prepare@ifs@direct{%
      \let\Ifnum=\ifnum%
      \let\Ifcase=\ifcase%
      \let\Or=\or%
      \let\Else=\else%
      \let\Fi=\fi%
      \let\Unless=\unless%
      \let\The=\the%
   }
}{
   \let\yquant@prepare@ifs@set=\relax%
   \let\yquant@prepare@ifs@direct=\relax%
}
\protected\long\def\yquant@prepare@finalize#1#2{%
   % We now know the dimensions of all the registers (though we didn't bother with the height of the control knobs [if present], we just assume they are too small to change this).
   \protected\def\idx{}%#
   \yquant@prepare@ifs@set%
   \let\yquant@prepare@append=\empty%
   \yquant@sort\yquant@prepare@sort%
   \def\do##1{%
      \appto\yquant@prepare@append{##1}%
      \yquant@prepare@finalize@ctrl##1%
   }%
   \yquant@sort@dolistloop%
   \protected@csxappto{\yquant@prefix draw}{%
      \yquant@draw@group%
         {\the\dimen2}%
         \ifyquant@circuit@operator@hasControls%
           \yquant@register@get@type\yquant@prepare@controltype%
         \else%
           F%
         \fi% if-switch whether controls are present
         {\yquant@attrs@remaining}% custom style
         {#2}% operator style
         {#1}%
         {\yquant@prepare@list}%
      \unexpanded\expandafter{\yquant@prepare@append}%
      \yquant@draw@endgroup%
         \ifyquant@circuit@operator@hasControls%
            T%
         \else%
            F%
         \fi%
         \ifx\yquant@lang@attr@name\empty%
            {}0%
         \else%
            {\yquant@lang@attr@name}%
            \ifnum\yquant@circuit@operator@numtarget=1 %
               \ifnum\yquant@circuit@operator@numpctrl=1 %
                  \ifnum\yquant@circuit@operator@numnctrl=1 %
                     7%
                  \else%
                     6%
                  \fi%
               \else%
                  \ifnum\yquant@circuit@operator@numnctrl=1 %
                     5%
                  \else%
                     4%
                  \fi%
               \fi%
            \else%
               \ifnum\yquant@circuit@operator@numpctrl=1 %
                  \ifnum\yquant@circuit@operator@numnctrl=1 %
                     3%
                  \else%
                     2%
                  \fi%
               \else%
                  \ifnum\yquant@circuit@operator@numnctrl=1 %
                     1%
                  \else%
                     0%
                  \fi%
               \fi%
            \fi%
         \fi%
   }%
}

\protected\def\yquant@prepare@single#1#2#3{%
   \yquant@sort@eadd{%
      \yquant@draw@single%
         {#3}% register index
         {\nodename}%
   }%
   \unless\ifyquant@circuit@operator@hasControls%
      \listadd\yquant@prepare@list{#3}%
   \fi%
   % determine the actual dimensions by a virtual draw command
   \pgfinterruptboundingbox%
      \yquant@config@operator@multifalse%
      \yquant@env@virtualize@path%
      \path%
         (0pt, 0pt)%
         node[/yquant/every operator, #2, /yquant/this operator,%
              name prefix=, name suffix=, name=] {#1};%
      \yquant@register@update@height{#3}{\the\pgf@picmaxy}%
      \yquant@register@update@depth{#3}{\the\dimexpr-\pgf@picminy\relax}%
}

\protected\def\yquant@prepare@multi#1#2#3{%
   \yquant@sort@eadd{%
      \yquant@draw@multi%
         #3%
         {\nodename}%
   }%
   \unless\ifyquant@circuit@operator@hasControls%
      \eappto\yquant@prepare@list{%
         \expandafter\yquant@list@range\@secondandthirdoffive#3%
      }%
   \fi%
   \pgfinterruptboundingbox%
      \yquant@config@operator@multitrue%
      \yquant@env@virtualize@path%
      \def\yquant@prepare@content{#1}%
      \def\yquant@prepare@style{#2}%
      \let\yquant@register@multi@contiguous=\yquant@prepare@multi@contiguous%
      \@fifthoffive#3%
      \ifdim\pgf@picmaxy=-16000pt %
         % if there was no single contiguous part before, determine the width now
         \path%
            (0pt, 0pt)%
            node[/yquant/every operator, #2, /yquant/this operator,%
                 name prefix=, name suffix=, name=] {#1};%
      \fi%
}

\protected\def\yquant@prepare@multi@contiguous#1#2#3{%
   \global\pgf@picmaxy=-16000pt %
   \global\pgf@picminy=16000pt %
   \edef\cmd{%
      \noexpand\path (0pt, 0pt)%
         node[/yquant/every operator, \yquant@prepare@style, /yquant/this operator,%
              /yquant/internal/multi main=\ifnum#3=1 true\else false\fi,%
              name prefix=, name suffix=, name=]%
            {\unexpanded\expandafter{\yquant@prepare@content}};%
   }%
   \cmd%
   \ifnum#1=#2 %
      % this is a single register in disguise
      \yquant@register@update@height{#1}{\the\pgf@picmaxy}%
      \yquant@register@update@depth{#1}{\the\dimexpr-\pgf@picminy\relax}%
   \else%
      \yquant@register@update@multispace{#1}{#2}{\the\dimexpr\pgf@picmaxy-\pgf@picminy\relax}%
   \fi%
}

\protected\def\yquant@prepare@multiinit#1#2#3{%
   \yquant@sort@eadd{%
      \yquant@draw@multiinit%
         #3%
         {\nodename}%
   }%
   \unless\ifyquant@circuit@operator@hasControls%
      \eappto\yquant@prepare@list{%
         \expandafter\yquant@list@range\@secondandthirdoffive#3%
      }%
   \fi%
   \pgfinterruptboundingbox%
      \yquant@config@operator@multitrue%
      \yquant@env@virtualize@path%
      \edef\first{\@secondoffive#3}%
      \def\pgfdecorationsegmentaspect{0.5}%
      \def\pgfdecorationsegmentfromto{0-1}%
      \ifnum\yquant@compat<2 %
         \path (0pt, 0pt)%
            node[/yquant/every operator, #2, /yquant/every multi label,%
                 /yquant/this operator, name prefix=, name suffix=, name=] {#1};%
      \else%
         \path (0pt, 0pt)%
            node[/yquant/every operator, #2,%
                 /yquant/this operator, name prefix=, name suffix=, name=] {#1};%
      \fi%
      \ifnum\@secondoffive#3=\@thirdoffive#3 %
         % this is a single register in disguise
         \yquant@register@update@height{\first}{\the\pgf@picmaxy}%
         \yquant@register@update@depth{\first}{\the\dimexpr-\pgf@picminy\relax}%
      \else%
         % this may not be sufficient. Since the text position need not necessarily be at the center (if the register corresponding to the visual center is excluded), we may require some space here which we will later only use in parts, but then extend where we should not. However, resolving this would require a special handling when calculating the y positions at the end, meaning we could not use the multispace facility. Let's assume discontiguous init registers are so scarce that this does not matter (disable the acquiration by using the operator/overlay key).
         \edef\upd{%
            \yquant@register@update@multispace%
               {\first}{\@thirdoffive#3}%
               {\the\dimexpr\pgf@picmaxy-\pgf@picminy\relax}%
         }%
         \upd%
      \fi%
}

\protected\gdef\yquant@prepare@output@discard#1#2#3{%
   \ifstrequal{#3}{discard}{%
      % This notification is triggered in the main circuit if there was an output gate on a wire with [out] or [inout] modifier, but the wire was discarded directly after the subcircuit. Then, it would look weird to extend the wire from the output gate until the end of the subcircuit, so we change the modifier to [ancilla] (not really, this is an artificial state) or [out].
      \listcsxadd{#2inonly}{#1}%
   }\relax%
}

\protected\long\def\yquant@prepare@output@single#1#2#3{%
   \yquant@sort@eadd{%
      \yquant@draw@output@single%
         {#3}% register index
         {\nodename}%
   }%
   \listadd\yquant@prepare@list{#3}%
   % we must be extra careful with outputs in subcircuits: Assume the wire is discarded after the subcircuit, then we don't want to extend it after our output label
   \ifdefined\yquant@parent%
      \ifinlistcs{#3}{\yquant@prefix inonly}\relax{%
         \yquant@register@set@lastgate{#3}{%
            \yquant@prepare@output@discard{#3}{\yquant@prefix}%
         }%
      }%
   \fi%
   % determine the actual dimensions by a virtual draw command
   \pgfinterruptboundingbox%
      \yquant@config@operator@multifalse%
      \yquant@env@virtualize@path%
      % #2 is empty anyway
      \edef\cmd{%
         \noexpand\path (0pt, 0pt)%
            node[\ifnum\yquant@compat>1 /yquant/every operator, \fi /yquant/every output,%
                 /yquant/every \yquant@register@type@tostring{\yquant@register@get@type{#3}} output,%
                 \ifnum\yquant@compat>1 /yquant/this operator, \fi%
                 name prefix=, name suffix=, name=] {\unexpanded{#1}};%
      }%
      \cmd%
      \yquant@register@update@height{#3}{\the\pgf@picmaxy}%
      \yquant@register@update@depth{#3}{\the\dimexpr-\pgf@picminy\relax}%
}

\protected\long\def\yquant@prepare@output@multi#1#2#3{%
   \yquant@sort@eadd{%
      \yquant@draw@output@multi%
         #3%
         {\nodename}%
   }%
   \eappto\yquant@prepare@list{%
      \expandafter\yquant@list@range\@secondandthirdoffive#3%
   }%
   % we must be extra careful with outputs in subcircuits: Assume the wire is discarded after the subcircuit, then we don't want to extend it after our output label
   \ifdefined\yquant@parent%
      \edef\first{\@secondoffive#3}%
      \edef\last{\@thirdoffive#3}%
      \yquant@for \i := \first to \last {%
         \xifinlistcs\i{\yquant@prefix inonly}\relax{%
            \yquant@register@set@lastgate\i{%
               \yquant@prepare@output@discard{\i}{\yquant@prefix}%
            }%
         }%
      }%
   \fi%
   \pgfinterruptboundingbox%
      \yquant@config@operator@multitrue%
      \yquant@env@virtualize@path%
      % We need to draw a line with some vertical extent, so just take the current height, whether it makes sense or not. We only need an estimate
      \edef\first{\@secondoffive#3}%
      \def\pgfdecorationsgmentaspect{0.5}%
      \def\pgfdecorationsegmentfromto{0-1}%
      % #2 is empty anyway
      \edef\cmd{%
         \noexpand\path (0pt, 0pt)
            node[\ifnum\yquant@compat>1 /yquant/every operator, /yquant/every output, \fi%
                 \ifnum\yquant@compat<2 /yquant/every multi output,\fi%
                 \ifnum\yquant@compat>1  /yquant/this operator,\fi%
                 name prefix=, name suffix=, name=] {\unexpanded{#1}};%
      }%
      \cmd%
      \ifnum\@secondoffive#3=\@thirdoffive#3 %
         % this is a single register in disguise
         \yquant@register@update@height{\first}{\the\pgf@picmaxy}%
         \yquant@register@update@depth{\first}{\the\dimexpr-\pgf@picminy\relax}%
      \else%
         % this may not be sufficient. Since the text position need not necessarily be at the center (if the register corresponding to the visual center is excluded), we may require some space here which we will later only use in parts, but then extend where we should not. However, resolving this would require a special handling when calculating the y positions at the end, meaning we could not use the multispace facility. Let's assume discontiguous output registers are so scarce that this does not matter (disable the acquiration by using the operator/overlay key).
         \edef\upd{%
            \yquant@register@update@multispace%
               {\first}{\@thirdoffive#3}%
               {\the\dimexpr\pgf@picmaxy-\pgf@picminy\relax}%
         }%
         \upd%
      \fi%
}

% BEGIN_FOLD replacement commands for draw actions that just keep track of the width
\protected\long\def\yquant@prepare@subcircuit@init#1#2{%
   \csdef{\yquant@prefix xpos@#1}{0pt}%
   \yquant@register@set@type{#1}{#2}%
}

\protected\def\yquant@prepare@subcircuit@getmaxx#1{%
   \begingroup%
      \dimen0=-16383.99999pt %
      \def\do##1{%
         \ifcsname\yquant@prefix xpos@##1\endcsname%
            \dimen2=\csname\yquant@prefix xpos@##1\endcsname\relax%
            \ifdim\dimen0<\dimen2 %
               \dimen0=\dimen2 %
            \fi%
         \else%
            \PackageError{yquant.sty}{Internal inconsistency detected}%
                         {Undefined internal wire x position.}%
         \fi%
      }%
      \dolistloop{#1}%
      \expandafter%
   \endgroup%
   \expandafter\def\expandafter\newx\expandafter{\the\dimen0}%
}

\protected\def\yquant@prepare@subcircuit@move@loop#1{%
   \cslet{\yquant@prefix xpos@#1}\newx%
}

\protected\long\def\yquant@prepare@subcircuit@group#1#2#3#4#5#6#7\yquant@draw@endgroup{%
   \begingroup%
      \yquant@prepare@subcircuit@getmaxx{#6}%
      % If the quotes library is loaded, activate it. (else, this is by default \relax)
      \tikz@enable@node@quotes%
      \yquant@config@operator@position@rightalignfalse%
      \yquant@config@operator@position@advancetrue%
      \yquant@set{#3}%
      \let\next=\endgroup%
      \ifyquant@config@operator@position@rightalign%
         \ifdim#1>-\pgf@picminx%
            \global\pgf@picminx=-\dimexpr#1\relax%
         \fi%
      \else%
         \ifyquant@env@seamless{%
            \ifdim\newx=0pt %
               \dimdef\newx{%
                  \newx+#1%
               }%
            \else%
               \dimdef\newx{%
                  \newx+\yquant@config@operator@sep+#1%
               }%
            \fi%
         }{%
            \dimdef\newx{%
               \newx+\yquant@config@operator@sep+#1%
            }%
         }%
         \ifdim\newx>\pgf@picmaxx%
            \global\pgf@picmaxx=\newx%
         \fi%
         \ifyquant@config@operator@position@advance%
            \edef\next{%
               \endgroup%
               \def\noexpand\newx{\newx}%
               \noexpand\forlistloop\yquant@prepare@subcircuit@move@loop{#6}%
            }%
         \fi%
      \fi%
   \next%
   \@gobblethree% three arguments for the endgroup
}

\let\yquant@prepare@subcircuit@pgfpointanchor=\pgfpointanchor
\patchcmd\yquant@prepare@subcircuit@pgfpointanchor{%
   \pgferror{No shape named `#1' is known}%
}{}\relax{%
   \PackageWarning{yquant.sty}{Patching \string\pgfpointanchor\space for the purpose of subcircuits failed; using and referencing named nodes in subcircuits may lead to irrelevant errors.}%
}
\let\yquant@prepare@subcircuit@pgfpointshapeborder=\pgfpointshapeborder
\patchcmd\yquant@prepare@subcircuit@pgfpointshapeborder{%
   \pgferror{No shape named `#1' is known}%
}{}\relax{%
   \PackageWarning{yquant.sty}{Patching \string\pgfpointshapeborder\space for the purpose of subcircuits failed; using and referencing named nodes in subcircuits may lead to irrelevant errors.}%
}

\protected\def\yquant@prepare@subcircuit@hspace#1#2{%
   \yquant@prepare@subcircuit@getmaxx{#1}%
   \dimdef\newx{\newx+#2}%
   \forlistloop\yquant@prepare@subcircuit@move@loop{#1}%
   \ifdim\newx>\pgf@picmaxx %
      \global\pgf@picmaxx=\newx %
   \fi%
}

\protected\def\yquant@prepare@subcircuit@endwires{%
   \expandafter\ifx\csname\yquant@prefix outputs\endcsname\relax%
      % to have a symmetric situation, we extend again one separation at the end, unless this is supposed to be seamless and we don't have outputs (for seamless circuits with outputs, extend - since this extension will be between last register and output)
      \ifyquant@env@seamless\relax{%
         \global\advance\pgf@picmaxx by \yquant@config@operator@sep\relax%
      }%
   \else%
      % if we have outputs, those will be realized as additional drawing groups following this macro, so increasing the picture at this point is rather pointless. Instead, we adjust the wire positions appropriately. The additional separation will be inserted by the outputs.
      \begingroup%
         \dimen0=-16383.99999pt %
         \yquant@fordown \i := \csname\yquant@prefix registers\endcsname downto 1 {%
            \ifcsname\yquant@prefix xpos@\i\endcsname%
               \dimen2=\csname\yquant@prefix xpos@\i\endcsname\relax%
               \ifdim\dimen0<\dimen2 %
                  \dimen0=\dimen2 %
               \fi%
            \else%
               \PackageError{yquant.sty}{Internal inconsistency detected}%
                            {Undefined internal wire x position.}%
            \fi%
         }%
         \expandafter%
      \endgroup%
      \expandafter\def\expandafter\newx\expandafter{\the\dimen0}%
      \yquant@fordown \i := \csname\yquant@prefix registers\endcsname downto 1 {%
         \cslet{\yquant@prefix xpos@\i}\newx%
      }%
   \fi%
   \let\yquant@circuit@endwires@finalize=\relax%
   \forlistcsloop\yquant@prepare@subcircuit@endwires@loop{\yquant@prefix inonly}%
}

\protected\def\yquant@prepare@subcircuit@endwires@loop#1{%
   \eappto\yquant@circuit@endwires@finalize{%
      \yquant@register@set@type{#1}\noexpand\yquant@register@type@none%
   }%
}
% END_FOLD

\newbox\yquant@prepare@subcircuit@box

\protected\long\def\yquant@prepare@subcircuit#1{%
   \yquant@sort@clear%
   \def\idx{0}%
   \dimen2=\yquant@config@operator@minimum@width%
   \ifyquant@circuit@operator@hasControls%
      \edef\yquant@prepare@list{%
         \yquant@list@range%
            \yquant@circuit@operator@minctrl%
            \yquant@circuit@operator@maxctrl%
      }%
   \else%
      \let\yquant@prepare@list=\empty%
   \fi%
   % BEGIN_FOLD register
   \def\do##1{%
      \ifx\yquant@lang@attr@name\empty%
         \let\nodename=\empty%
      \else%
         \edef\nodename{\yquant@lang@attr@name-\idx}%
      \fi%
      \ifyquant@firsttoken\yquant@register@multi{##1}{%
         \yquant@prepare@subcircuit@multi{#1}{##1}%
      }{%
         \yquant@prepare@subcircuit@single{#1}{##1}%
      }%
      \pgfinterruptboundingbox%
         % In order to determine the width of the subcircuit, we must execute the draw command at preparation time, where we will remap all relevant commands to virtual ones so that this has no effect and is not very costly. Although nothing should be drawn, as a precaution, we "draw" everything in a box that is dropped afterwards.
         % There will still be some extra width and height taken by separations or other things related to the box itself.
         \yquant@env@virtualize@path%
         \begingroup%
            \let\yquant@parent=\yquant@prefix%
            \edef\yquant@prefix{yquant@env\yquant@circuit@subcircuit@id @}%
            \let\yquant@draw@init=\yquant@prepare@subcircuit@init%
            \let\yquant@draw@group=\yquant@prepare@subcircuit@group%
            % We may have draw actions within the subcircuit which reference nodes that have been created within the same subcircuit - but they are not known at the stage of preparation! So we here hack into the node querying macros of pgf and just let every unknown node be equal to the origin. If the node is truely unknown, we will find out about this in the draw stage.
            \let\pgfpointanchor=\yquant@prepare@subcircuit@pgfpointanchor%
            \let\pgfpointshapeborder=\yquant@prepare@subcircuit@pgfpointshapeborder%
            \let\yquant@draw@alias=\@gobble%
            \let\yquant@draw@hspace=\yquant@prepare@subcircuit@hspace%
            \let\yquant@circuit@endwires=\yquant@prepare@subcircuit@endwires%
            \let\yquant@circuit@flushwire=\@gobble%
            \let\yquant@circuit@setstyle=\@gobbletwo%
            \let\yquant@circuit@addstyle=\@gobbletwo%
            % do not overwrite \yquant@register@set@type, which may also occur - we want to change the register type!
            % restore tikz commands... as in env@end
            \let\path=\tikz@command@path%
            \let\tikz@lib@scope@check=\yquant@env@substikz@scopecheck%
            \let\tikz@scope@opt=\yquant@env@substikz@scope%
            \let\endtikz@scope@env=\yquant@env@substikz@endscope%
            \let\endscope=\endtikz@scope@env%
            \let\stopscope=\endscope%
            \global\pgf@picmaxx=0pt %
            \global\pgf@picminx=0pt %
            \global\setbox\yquant@prepare@subcircuit@box=\vbox to 1sp{%
               \csname\yquant@prefix draw\endcsname%
            }%
            \ifdim\pgf@picmaxy=-16000pt %
               \global\pgf@picmaxy=0pt %
               \global\pgf@picminy=0pt %
            \fi%
            \ifyquant@env@seamless{%
               % for seamless circuits, we do not have an initial separation. However, if there is a label to registers (which you should not do for seamless subcircuits), the "initial" separation is in fact an inner one, so we need it.
               \ifdim\pgf@picminx<0pt %
                  \global\advance\pgf@picmaxx by \yquant@config@operator@sep\relax%
               \fi%
            }\relax%
            \global\wd\yquant@prepare@subcircuit@box=\dimexpr\pgf@picmaxx-\pgf@picminx\relax%
         \endgroup%
         \edef\yquant@prepare@subcircuit@width{%
            {\the\wd\yquant@prepare@subcircuit@box}% inner width
            {\noexpand\the\dimexpr\pgf@picmaxx-\pgf@picminx\relax}% outer width
            {\the\pgf@picminx}% left margin
         }%
         \pgfresetboundingbox%
         \path%
            (0pt, 0pt)%
            node[/yquant/every operator, #1,%
                 /yquant/operators/every subcircuit box, /yquant/this operator,%
                 /yquant/operators/this subcircuit box,%
                 name prefix=, name suffix=, name=, y radius=0pt]%
            {\box\yquant@prepare@subcircuit@box};%
         % the extra height is taken care for by manually inserting it to the height of the first and last register in the subcircuit
         \yquant@register@inject@extents{\pgf@picmaxy}{-\pgf@picminy}%
         \edef\cmd{%
            \dimen0=\the\dimexpr\pgf@picmaxx-\pgf@picminx\relax\relax%
            \yquant@prepare@subcircuit@add%
         }%
         \expandafter%
      \endpgfinterruptboundingbox%
      \cmd%
      \ifdim\dimen0>\dimen2 %
         \dimen2=\dimen0 %
      \fi%
      \numdef\idx{\idx+1}%
   }%
   \dolistloop\yquant@circuit@operator@targets%
   % END_FOLD
   \yquant@prepare@controls%
   \preto\yquant@attrs@remaining{internal/no advance,}%
   \yquant@prepare@finalize{}{#1}%
}

\protected\def\yquant@prepare@subcircuit@single#1#2{%
   \yquant@config@operator@multifalse%
   \edef\yquant@circuit@subcircuit@param{#2\yquant@list@delim}%
   \yquant@circuit@subcircuit{#1}%
   \unless\ifyquant@circuit@operator@hasControls%
      \listadd\yquant@prepare@list{#2}%
   \fi%
   \edef\yquant@prepare@subcircuit@add{%
      \yquant@sort@eadd{%
         \yquant@draw@subcircuit@single%
            {#2}% register index
            {\yquant@circuit@subcircuit@id}%
            {\nodename}\ifnum\yquant@circuit@operator@numtarget=1 1\else0\fi%
            {\noexpand\yquant@prepare@subcircuit@width}%
      }%
   }%
}

\protected\def\yquant@prepare@subcircuit@multi#1#2{%
   \yquant@config@operator@multitrue%
   \edef\yquant@circuit@subcircuit@param{\@fifthoffive#2}%
   \yquant@sort@list\yquant@circuit@subcircuit@param\yquant@sort@ascending%
   \yquant@circuit@subcircuit{#1}%
   \unless\ifyquant@circuit@operator@hasControls%
      \eappto\yquant@prepare@list{%
         \expandafter\yquant@list@range\@secondandthirdoffive#2%
      }%
   \fi%
   \edef\yquant@prepare@subcircuit@add{%
      \yquant@sort@eadd{%
         \yquant@draw@subcircuit@multi%
            #2%
            {\yquant@circuit@subcircuit@id}%
            {\nodename}\ifnum\yquant@circuit@operator@numtarget=1 1\else0\fi%
            {\noexpand\yquant@prepare@subcircuit@width}%
      }%
   }%
}

\protected\def\yquant@prepare@finalize@ctrl#1{%
   \let\next=\yquant@prepare@finalize@ctrl@single%
   \ifx\yquant@draw@multi#1%
      \let\next=\yquant@prepare@finalize@ctrl@multi%
   \else%
      \ifx\yquant@draw@multiinit#1%
         \let\next=\yquant@prepare@finalize@ctrl@multi%
      \else%
         \ifx\yquant@draw@output@multi#1%
            \let\next=\yquant@prepare@finalize@ctrl@multi%
         \else%
            \ifx\yquant@draw@subcircuit@multi#1%
               \let\next=\yquant@prepare@finalize@ctrl@subcircuit@multi%
            \else%
               \ifx\yquant@draw@subcircuit@single#1%
                  \let\next=\yquant@prepare@finalize@ctrl@subcircuit@single%
               \else%
                  \ifx\yquant@draw@inject#1%
                     \let\next=\@gobble%
                  \fi%
               \fi%
            \fi%
         \fi%
      \fi%
   \fi%
   \next%
}

\protected\def\yquant@prepare@finalize@ctrl@single#1#2{%
   \eappto\yquant@prepare@append{%
      \yquant@prepare@callback@draw{#1}%
   }%
   \yquant@prepare@callback@prepare{#1}%
}

\protected\def\yquant@prepare@finalize@ctrl@multi#1#2#3#4#5{%
   \let\yquant@register@multi@contiguous=\yquant@prepare@finalize@ctrl@multi@contiguous%
   \ifyquant@circuit@operator@hasControls%
      \ifyquant@config@operator@multi@warn%
         \def\yquant@prepare@finalize@ctrl@multi@contiguous@warn{0}%
      \else%
         \def\yquant@prepare@finalize@ctrl@multi@contiguous@warn{2}%
      \fi%
   \else%
      \def\yquant@prepare@finalize@ctrl@multi@contiguous@warn{2}%
   \fi%
   \cslet{\yquant@prefix finalize@ctrl@prepare@appto}\empty%
   #4%
   \eappto\yquant@prepare@append{\csname\yquant@prefix finalize@ctrl@prepare@appto\endcsname}%
   \csgundef{\yquant@prefix finalize@ctrl@prepare@appto}%
}

\protected\def\yquant@prepare@finalize@ctrl@multi@contiguous#1#2#3{%
   \ifnum\yquant@prepare@finalize@ctrl@multi@contiguous@warn=1 %
      \PackageWarning{yquant.sty}{Ambiguous operation: multiple discontiguous multi-register operations in combination with controls make it hard to visually determine on which registers the gates act on.}%
      % switch the warning off for this group (which is a single operation)
      \yquant@config@operator@multi@warnfalse%
      \def\yquant@prepare@finalize@ctrl@multi@contiguous@warn{2}%
   \else%
      \numdef\yquant@prepare@finalize@ctrl@multi@contiguous@warn{%
         \yquant@prepare@finalize@ctrl@multi@contiguous@warn+1%
      }%
   \fi%
   {% save \body
      \yquant@for \yquant@i := #1 to #2 {{% let inner loop mess up with macros
         \csxappto{\yquant@prefix finalize@ctrl@prepare@appto}{%
            \expandafter\yquant@prepare@callback@draw\expandafter{\yquant@i}%
         }%
         \expandafter\yquant@prepare@callback@prepare\expandafter{\yquant@i}%
      }}%
   }%
}

\def\yquant@prepare@finalize@ctrl@subcircuit@single#1#2#3#4#5{%
   \yquant@prepare@finalize@ctrl@single{#1}{#3}%
}

\protected\def\yquant@prepare@finalize@ctrl@subcircuit@multi@loop#1{%
   \eappto\yquant@prepare@append{%
      \yquant@prepare@callback@draw{#1}%
   }%
   \yquant@prepare@callback@prepare{#1}%
}

\protected\def\yquant@prepare@finalize@ctrl@subcircuit@multi#1#2#3#4#5#6#7#8{%
   % there are no contiguous parts here, don't call the normal @multi
   \forlistloop\yquant@prepare@finalize@ctrl@subcircuit@multi@loop{#4}%
}

==> yquant-registers.tex <==
\def\yquant@register@type@none{0}
\def\yquant@register@type@q{1}
\def\yquant@register@type@c{2}
\def\yquant@register@type@qs{3}

\def\yquant@register@type@tostring#1{%
   \ifcase#1 %
      nobit%
   \or%
      qubit%
   \or%
      cbit%
   \or%
      qubits%
   \else%
      \PackageError{yquant.sty}{Internal inconsistency detected}%
                   {Unknown wire type: `#1'.}%
   \fi%
}

\protected\def\yquant@register@type@fromstring#1#2{%
   \expandafter\ifstrequal\expandafter{#1}{qubit}%
      {\let#2=\yquant@register@type@q}%
      {%
         \expandafter\ifstrequal\expandafter{#1}{cbit}%
         {\let#2=\yquant@register@type@c}%
         {%
            \expandafter\ifstrequal\expandafter{#1}{qubits}%
            {\let#2=\yquant@register@type@qs}%
            {%
               \PackageError{yquant.sty}{Invalid bit type: `#1'}%
                  {Use one of `qubit', `cbit', or `qubits'.}%
            }%
         }%
      }%
}

% Internally, we store the register information in a single macro. Indeed, this is almost always faster than using multiple macros (at least in the way implemented here), apart from changing a single type of information, which is almost as fast.
% BEGIN_FOLD Constructor: create single register and cleanup environment

% #1: type
% #2: name
% #3: index
\protected\def\yquant@register@define#1#2#3{%
   \csnumgdef{\yquant@prefix registers}%
             {\csname\yquant@prefix registers\endcsname+1}%
   % sync with yquantlanguage-groups/\yquantgroup@startenvironment
   \csxdef{\yquant@prefix register@\csname\yquant@prefix registers\endcsname}{%
      {#1}% type
      {0pt}% x pos
      {{\yquant@config@register@minimum@height}%
       {\yquant@config@register@minimum@depth}%
       {}}% height, depth, and multi-space parts; at the end, the y position
      {{0pt}{0pt}{}{}}% wire start positions and clipping
      {}% wire style
      {\yquant@register@flag@clean}% information about the last gate
   }%
   \global\csletcs{\yquant@prefix registername@#2[#3]}{\yquant@prefix registers}%
   \csxdef{\yquant@prefix registerhigh@#2}{#3}%
   \yquant@cleanup@csadd{\yquant@prefix register@\csname\yquant@prefix registers\endcsname}%
   \yquant@cleanup@csadd{\yquant@prefix registername@#2[#3]}%
   \ifnum0=#3\relax%
      \yquant@cleanup@csadd{\yquant@prefix registerhigh@#2}%
   \fi%
}

% in a subcircuit, create a new register that is only an alias for an existing register in the outer circuit.
% #4: id in the outer circuit
\protected\def\yquant@register@alias#1#2#3#4{%
   \csnumgdef{\yquant@prefix registers}%
             {\csname\yquant@prefix registers\endcsname+1}%
   \ifcsname\yquant@parent registermap@#4\endcsname%
      % the parent is already an alias itself, pass this on transparently
      \global\csletcs%
         {\yquant@prefix registermap@\csname\yquant@prefix registers\endcsname}%
         {\yquant@parent registermap@#4}%
   \else%
      \csxdef{\yquant@prefix registermap@\csname\yquant@prefix registers\endcsname}%
             {\yquant@parent register@#4}%
   \fi%
   % we still store height, depth, and multi-space parts. To keep the same macros, we create a full register structure, but "abuse" the type component to contain the direct parent
   \csxdef{\yquant@prefix register@\csname\yquant@prefix registers\endcsname}{%
      {{\expandafter\yquant@register@alias@extract\yquant@parent}{#4}}% direct parent (circuit id, register id)
      {}% unused
      {{\yquant@config@register@minimum@height}%
       {\yquant@config@register@minimum@depth}%
       {}}% height, depth, and multi-space parts
      {}% unused
      {}% unused
      {}% unused
   }%
   \global\csletcs{\yquant@prefix registername@#2[#3]}{\yquant@prefix registers}%
   \csxdef{\yquant@prefix registerhigh@#2}{#3}%
   \yquant@cleanup@csadd{\yquant@prefix register@\csname\yquant@prefix registers\endcsname}%
   \yquant@cleanup@csadd{\yquant@prefix registermap@\csname\yquant@prefix registers\endcsname}%
   \yquant@cleanup@csadd{\yquant@prefix registername@#2[#3]}%
   \ifnum0=#3\relax%
      \yquant@cleanup@csadd{\yquant@prefix registerhigh@#2}%
   \fi%
   \expandafter\yquant@register@set@@aux%
      \csname\csname\yquant@prefix registermap@\csname\yquant@prefix registers\endcsname\endcsname\endcsname%
      \yquant@register@set@typelastgate@aux%
      {{#1}{\yquant@register@flag@clean}}%
}

\def\yquant@register@alias@extract yquant@env#1@{#1}%
% END_FOLD

% BEGIN_FOLD Converter: convert a register name to its id
% store the number corresponding to register #2 into #1
\protected\def\yquant@register@get@id#1#2{%
   \ifcsname\yquant@prefix registername@#2\endcsname%
      \letcs#1{\yquant@prefix registername@#2}%
   \else%
      \yquant@register@get@id@lazycreate{#2}%
      \letcs#1{\yquant@prefix registers}%
   \fi%
}

% same as before, but resolves to the _index_ of the last register
\protected\def\yquant@register@get@id@high#1#2{%
   \unless\ifcsname\yquant@prefix registerhigh@#2\endcsname%
      \yquant@register@get@id@lazycreate{#2}%
   \fi%
   \letcs#1{\yquant@prefix registerhigh@#2}%
}

% In the lazy mode, we create all unknown registers on-the-fly.
\def\yquant@register@get@id@lazycreate#1{%
   \ifyquant@env@lazy%
      % In principle, we could just call \yquant@lang@@qubit. However, if access to a vector register is desired and a _part_ of this does already exist (though not the requested index), we only create the missing registers.
      \yquant@register@get@id@lazycreate@parse#1[;%
   \else%
      \PackageError{yquant.sty}{Register `#1' unknown}%
         {You referred to an unknown register.
          Declare registers first using `qubit' and friends.}%
   \fi%
}

\def\yquant@register@get@id@lazycreate@parse#1[#2;{%
   \ifstrempty{#2}{%
      \yquant@register@get@id@lazycreate@do#1[0][;%
   }{%
      \yquant@register@get@id@lazycreate@do#1[#2;%
   }%
}

\protected\def\yquant@register@get@id@lazycreate@do#1[#2]#3[;{%
   \begingroup%
      % parse length
      \ifstrempty{#3}{%
         \yquant@langhelper@validate\len\count{#2}%
         \numdef\len{\len+1}%
      }{%
         \PackageError{yquant.sty}{Invalid register name}%
            {Register names must not contain `[' apart from register length indication.}%
      }%
      \edef\reg{\trim@spaces{#1}}%
      % Was this register already defined?
      \ifcsname\yquant@prefix registerhigh@\reg\endcsname%
         \numdef\idx{\csname\yquant@prefix registerhigh@\reg\endcsname+1}%
         \unless\ifnum\idx<\len\relax%
            \PackageError{yquant.sty}{Internal inconsistency detected}%
               {Tried to create a register on-the-fly that already existed.}%
         \fi%
      \else%
         \def\idx{0}%
      \fi%
      % pre-set y position
      \yquant@for \idx := \idx to \numexpr \len -1\relax {%
         \yquant@prepare@create\reg\idx\yquant@register@type@q%
      }%
   \endgroup%
}

\newif\ifyquant@register@get@allowmulti
% converts names to indices
% #1: comma-separated string of names or ranges
%     range format: startname-endname
%     Both startname and endname may be omitted, denoting the very first and last
%     register, respectively
%     If \ifyquant@register@get@allowmulti is set to true, multi-qubit registers are
%     allowed, which are surrounded by parentheses. They may not appear in ranges.
% \yquant@register@get@ids@list, \yquant@register@get@ids@min, \yquant@register@get@ids@max and \yquant@register@get@ids@count will be set appropriately
\begingroup%
\catcode`[=\active%
\catcode`(=\active%
\protected\gdef\yquant@register@get@ids#1{%
   \begingroup%
      \let\yquant@register@get@ids@list=\empty%
      \count0=2147483647 % minimal id
      \count2=0 % maximal id
      \count4=0 % number of total registers
      \ifblank{#1}{}{%
         \let\ifinmulti=\iffalse%
         \let\ifallowmain=\iffalse%
         \let\do=\yquant@register@get@ids@outerlist%
         \begingroup%
            \catcode`[=\active%
            \catcode`(=\active%
            \def[##1]{\yquant@register@get@ids@@index{##1}}%
            \def(##1){\yquant@register@get@ids@@multi{##1}}%
            % this is also invoked by other languages which might have completely redefined all catcodes (qasm redefines the backslash), so don't just add \noexpand at the end of the \scantokens...
            \everyeof{\noexpand}%
            \endlinechar=-1 %
            \edef\yquant@register@get@ids@retokenized{\scantokens{#1}}%
            \expandafter%
         \endgroup%
         \expandafter\docsvlist\expandafter{\yquant@register@get@ids@retokenized}%
      }%
      \global\let\yquant@register@get@ids@list=\yquant@register@get@ids@list%
      \xdef\yquant@register@get@ids@min{\the\count0}%
      \xdef\yquant@register@get@ids@max{\the\count2}%
      \xdef\yquant@register@get@ids@count{\the\count4}%
   \endgroup%
}
\endgroup

\protected\def\yquant@register@get@ids@@index{}
\protected\def\yquant@register@get@ids@@multi{}

\def\yquant@register@get@ids@outerlist#1{%
   \ifyquant@firsttoken\yquant@register@get@ids@@multi{#1}{%
      \unless\ifyquant@register@get@allowmulti%
         \PackageError{yquant.sty}{Multi-register gate not allowed}%
                      {The selected gate can only be used in a single-register context.}%
      \fi%
      \yquant@register@get@ids@multi#1\yquant@sep%
   }{%
      \yquant@register@get@ids@checkrange#1-\yquant@sep%
   }%
}

\protected\def\yquant@register@get@ids@multi\yquant@register@get@ids@@multi#1\yquant@sep{%
   \begingroup%
      \let\yquant@register@get@ids@list=\empty%
      \count0=2147483647 % minimal id
      \count2=0 % maximal id
      \count4=0 % number of total registers
      \count6=-1 % index of main register
      \let\ifinmulti=\iftrue%
      \let\ifallowmain=\iftrue%
      \let\do=\yquant@register@get@ids@multilist%
      \docsvlist{#1}%
      \ifnum\count6=-1 %
         \count6=\count0 %
      \fi%
      \yquant@register@multi@splitparts%
      \edef\process{%
            \endgroup%
         \noexpand\listadd\noexpand\yquant@register@get@ids@list{%
            \noexpand\yquant@register@multi%
               {\the\count0}{\the\count2}{\the\count4}%
               {\yquant@register@get@ids@list}%
         }%
         \noexpand\ifnum\count0>\the\count0\space%
            \count0=\the\count0\space%
         \noexpand\fi%
         \noexpand\ifnum\count2<\the\count2\space%
            \count2=\the\count2\space%
         \noexpand\fi%
         \advance\count4 by 1 %
      }%
      \process%
}

\def\yquant@register@get@ids@multilist#1{%
   \yquant@register@get@ids@checkrange#1-\yquant@sep%
}

\def\yquant@register@get@ids@checkrange#1-#2\yquant@sep{%
   \ifstrempty{#2}{%
      % the string does not contain a dash
      \yquant@register@get@ids@norange{#1}%
   }{%
      % this is a range argument
      \yquant@register@get@ids@range#1-#2\yquant@sep%
   }%
}

\def\yquant@register@get@ids@norange#1{%
   % the register is not used within a range, which gives us full freedom with respect to sub-index selections
   \yquant@register@get@ids@norange@checkindex%
      #1%
      \yquant@register@get@ids@@index%
      \yquant@sep%
}

\protected\def\yquant@register@get@ids@norange@checkindex#1\yquant@register@get@ids@@index#2\yquant@sep{%
   \edef\current{\trim@spaces{#1}}%
   \ifallowmain%
      \expandafter\ifyquant@firsttoken\expandafter*\expandafter{\current}{%
         \edef\current{%
            \expandafter\expandafter\expandafter\trim@spaces%
            \expandafter\expandafter\expandafter{%
               \expandafter\@gobble\current%
            }%
         }%
         % catch the minimal index
         \edef\yquant@register@get@ids@norange@checkindex@setmain{%
            \count6=\count2%
            \ifnum\count0<\the\count0 %
               \count0=\the\count0 %
            \fi%
         }%
         \count0=2147483647 %
         \csletcs{ifallowmain}{iffalse}%
      }{%
         \let\yquant@register@get@ids@norange@checkindex@setmain=\relax%
      }%
   \else%
      \let\yquant@register@get@ids@norange@checkindex@setmain=\relax%
   \fi%
   \ifstrempty{#2}{%
      % the string does not contain a sub-index; we add the full register
      \yquant@register@get@id\first{\current[0]}%
      \letcs\high{\yquant@prefix registerhigh@\current}%
      \yquant@register@get@id\last{\current[\high]}%
      \ifnum\first<\count0 %
         \count0=\first\relax%
      \fi%
      \ifnum\last>\count2 %
         \count2=\last\relax%
      \fi%
      \advance\count4 by \numexpr\high+1\relax%
      \yquant@for \i := 0 to \high {%
         \yquant@register@get@id\idx{\current[\i]}%
         \listeadd\yquant@register@get@ids@list{\idx}%
      }%
   }{%
      \yquant@register@get@ids@norange@index#2%
   }%
   \yquant@register@get@ids@norange@checkindex@setmain%
}

\protected\def\yquant@register@get@ids@norange@index#1\yquant@register@get@ids@@index{%
   \let\olddo=\do%
   % the string contains sub-indices; since we are not in a range, multi-indices may still be allowed
   \ifinmulti%
      \let\do=\yquant@register@get@ids@subindex@nomulti%
   \else%
      \let\do=\yquant@register@get@ids@subindex@allowmulti%
   \fi%
   \docsvlist{#1}%
   \let\do=\olddo%
}

\def\yquant@register@get@ids@subindex@nomulti#1{%
   \yquant@register@get@ids@subindex@checkrange#1-\yquant@sep%
}

\def\yquant@register@get@ids@subindex@allowmulti#1{%
   \ifyquant@firsttoken\yquant@register@get@ids@@multi{#1}{%
      \unless\ifyquant@register@get@allowmulti%
         \PackageError{yquant.sty}{Multi-register gate not allowed}%
                      {The selected gate can only be used in a single-register context.}%
      \fi%
      \yquant@register@get@ids@subindex@multi#1\yquant@sep%
   }{%
      \yquant@register@get@ids@subindex@checkrange#1-\yquant@sep%
   }%
}

\protected\def\yquant@register@get@ids@subindex@multi\yquant@register@get@ids@@multi#1\yquant@sep{%
   \begingroup%
      \let\yquant@register@get@ids@list=\empty%
      \count0=2147483647 % minimal id
      \count2=0 % maximal id
      \count4=0 % number of total registers
      \count6=-1 % index of main register
      \let\ifinmulti=\iftrue%
      \let\ifallowmain=\iftrue%
      \let\do=\yquant@register@get@ids@subindex@nomulti%
      \docsvlist{#1}%
      \ifnum\count6=-1 %
         \count6=\count0 %
      \fi%
      \yquant@register@multi@splitparts%
      \edef\process{%
            \endgroup%
         \noexpand\listadd\noexpand\yquant@register@get@ids@list{%
            \noexpand\yquant@register@multi%
               {\the\count0}{\the\count2}{\the\count4}%
               {\yquant@register@get@ids@list}%
         }%
         \noexpand\ifnum\count0>\the\count0\space%
            \count0=\the\count0\space%
         \noexpand\fi%
         \noexpand\ifnum\count2<\the\count2\space%
            \count2=\the\count2\space%
         \noexpand\fi%
         \advance\count4 by 1 %
      }%
      \process%
}

\def\yquant@register@get@ids@subindex@checkrange#1-#2\yquant@sep{%
   \ifstrempty{#2}{%
      % the string does not contain a dash, this is a single sub-item
      \edef\idx{\trim@spaces{#1}}%
      \expandafter\yquant@register@get@ids@subindex@norange\expandafter{\idx}%
   }{%
      % this is a range argument
      \yquant@register@get@ids@subindex@range#1-#2\yquant@sep%
   }%
}

\protected\def\yquant@register@get@ids@subindex@norange#1{%
   \ifallowmain%%
      \ifyquant@firsttoken*{#1}{%
         \edef\idx{\current[\expandafter\trim@spaces\expandafter{\@gobble#1}]}%
         \expandafter\yquant@register@get@id\expandafter\idx\expandafter{\idx}%
         \count6=\idx%
         \csletcs{ifallowmain}{iffalse}%
      }{%
         \yquant@register@get@id\idx{\current[#1]}%
      }%
   \else%
      \yquant@register@get@id\idx{\current[#1]}%
   \fi%
   \ifnum\idx<\count0 %
      \count0=\idx\relax%
   \fi%
   \ifnum\idx>\count2 %
      \count2=\idx\relax%
   \fi%
   \advance\count4 by 1\relax%
   \listeadd\yquant@register@get@ids@list{\idx}%
}

\protected\def\yquant@register@get@ids@subindex@range#1-#2-\yquant@sep{%
   \ifallowmain%
      \ifyquant@firsttoken*{#1}{%
         \expandafter\ifblank\expandafter{\@gobble#1}{%
            \def\first{0}%
         }{%
            \expandafter\yquant@langhelper@validate\expandafter\first\expandafter\count\expandafter{\@gobble#1}%
         }%
         \yquant@register@get@id\idx{\current[\first]}%
         \count6=\idx%
         \csletcs{ifallowmain}{iffalse}%
      }{%
         \ifblank{#1}{%
            \def\first{0}%
         }{%
            \yquant@langhelper@validate\first\count{#1}%
         }%
      }%
   \else%
      \ifblank{#1}{%
         \def\first{0}%
      }{%
         \yquant@langhelper@validate\first\count{#1}%
      }%
   \fi%
   \ifallowmain%
      % in #1, all initial spaces are gobbled automatically, but not in #2
      \expandafter\ifyquant@firsttoken\expandafter*\expandafter{\empty#2}{%
         \expandafter\ifblank\expandafter{\@gobble#2}{%
            \yquant@register@get@id@high\last\current%
         }{%
            \expandafter\yquant@langhelper@validate\expandafter\last\expandafter\count\expandafter{\@gobble#2}%
         }%
         \yquant@register@get@id\idx{\current[\last]}%
         \count6=\idx%
         \csletcs{ifallowmain}{iffalse}%
      }{%
         \ifblank{#2}{%
            \yquant@register@get@id@high\last\current%
         }{%
            \yquant@langhelper@validate\last\count{#2}%
         }%
      }%
   \else%
      \ifblank{#2}{%
         \yquant@register@get@id@high\last\current%
      }{%
         \yquant@langhelper@validate\last\count{#2}%
      }%
   \fi%
   \yquant@for \i := \first to \last {%
      \yquant@register@get@ids@subindex@norange\i%
   }%
}

\protected\def\yquant@register@get@ids@range#1-#2-\yquant@sep{%
   % being a range between two registers, those must be uniquely identifiable, i.e. either a single sub-indexed part of a vector register, or no vector specification at all.
   \ifallowmain%
      \ifyquant@firsttoken*{#1}{%
         \expandafter\ifblank\expandafter{\@gobble#1}{%
            \def\first{1}%
         }{%
            \expandafter\yquant@register@get@ids@range@getfirst\@gobble#1\yquant@register@get@ids@@index\yquant@sep%
         }%
         \count6=\first%
         \csletcs{ifallowmain}{iffalse}%
      }{%
         \ifblank{#1}{%
            \def\first{1}%
         }{%
            \yquant@register@get@ids@range@getfirst#1\yquant@register@get@ids@@index\yquant@sep%
         }%
      }%
   \else%
      \ifblank{#1}{%
         \def\first{1}%
      }{%
         \yquant@register@get@ids@range@getfirst#1\yquant@register@get@ids@@index\yquant@sep%
      }%
   \fi%
   % it does not make sense to allow to set the main part on the second half of the range, since a range over registers (not indices) is automatically visual, so this range will be contiguous.
   \ifblank{#2}{%
      \letcs\last{\yquant@prefix registers}%
   }{%
      \yquant@register@get@ids@range@getlast#2\yquant@register@get@ids@@index\yquant@sep%
   }%
   \ifnum\first<\last\relax%
      \ifnum\first<\count0 %
         \count0=\first\relax%
      \fi%
      \ifnum\last>\count2 %
         \count2=\last\relax%
      \fi%
      \advance\count4 by \numexpr\last-\first+1\relax%
   \else%
      \ifnum\last<\count0 %
         \count0=\last\relax%
      \fi%
      \ifnum\first>\count2 %
         \count2=\first\relax%
      \fi%
      \advance\count4 by \numexpr\first-\last+1\relax%
   \fi%
   \yquant@for \i := \first to \last {%
      \listeadd\yquant@register@get@ids@list{\i}%
   }%
}

\def\yquant@register@get@ids@range@getfirst#1\yquant@register@get@ids@@index#2\yquant@sep{%
   \ifstrempty{#2}{%
      \yquant@register@get@id\first{\trim@spaces{#1}[0]}%
   }{%
      \yquant@register@get@ids@range@get\first#1\yquant@register@get@ids@@index#2%
   }%
}

\protected\def\yquant@register@get@ids@range@getlast#1\yquant@register@get@ids@@index#2\yquant@sep{%
   \ifstrempty{#2}{%
      \yquant@register@get@id@high\last{\trim@spaces{#1}}%
      \yquant@register@get@id\last{\trim@spaces{#1}[\last]}%
   }{%
      \yquant@register@get@ids@range@get\last#1\yquant@register@get@ids@@index#2%
   }%
}

\def\yquant@register@get@ids@range@get#1#2\yquant@register@get@ids@@index#3\yquant@register@get@ids@@index{%
   \yquant@register@get@id#1{\trim@spaces{#2}[\trim@spaces{\trim@spaces#3}]}%
}

\let\yquant@register@multi=\empty%
\protected\def\yquant@register@multi@contiguous{}%

% splits \yquant@register@get@ids@list into a list of contiguous parts
\protected\def\yquant@register@multi@splitparts{%
   \begingroup%
      \let\registers=\yquant@register@get@ids@list%
      \yquant@sort@list\registers\yquant@sort@ascending%
      \let\newlist=\empty%
      \count2=-1 %
      \def\do##1{%
         \ifnum\count2=-1 %
            \count2=##1 %
            \count4=\count2 %
         \else%
            \advance\count2 by 1 %
            \ifnum##1>\count2 %
               % this is a discontiguous change (we disallow duplicate entries)
               \eappto\newlist{%
                  \yquant@register@multi@contiguous%
                     {\the\count4}{\the\numexpr\count2-1\relax}%
                     {\ifnum\count6<\count2 %
                         \ifnum\count4>\count6 %
                            0%
                         \else%
                            1%
                         \fi%
                      \else%
                         0%
                      \fi}%
               }%
               \count2=##1 %
               \count4=\count2 %
            \fi%
         \fi%
      }%
      \dolistloop\registers%
      % we disallow empty lists
      \eappto\newlist{%
         \yquant@register@multi@contiguous%
            {\the\count4}{\the\count2}%
            {\ifnum\count6>\count2 %
                0%
             \else%
                \ifnum\count4>\count6 %
                   0%
                \else%
                   1%
                \fi%
             \fi}%
      }%
      \expandafter%
   \endgroup%
   \expandafter\def\expandafter\yquant@register@get@ids@list\expandafter{%
      \newlist%
   }%
}

% splits \yquant@register@get@ids@list into a list of discontiguous parts
\protected\def\yquant@register@multi@splitparts@sepall{%
   \begingroup%
      \let\registers=\yquant@register@get@ids@list%
      \yquant@sort@list\registers\yquant@sort@ascending%
      \let\newlist=\empty%
      \def\do##1{%
         \eappto\newlist{%
            \yquant@register@multi@contiguous%
               {##1}{##1}%
               {\ifnum##1=\count6 %
                   1%
                \else%
                   0%
                \fi%
               }%
         }%
      }%
      \dolistloop\registers%
      \expandafter%
   \endgroup%
   \expandafter\def\expandafter\yquant@register@get@ids@list\expandafter{%
      \newlist%
   }%
}

\protected\def\yquant@register@multi@splitparts@sort{%
   \yquant@sort@list\yquant@register@get@ids@list\yquant@sort@ascending%
}

\protected\def\yquant@register@get@multiassingle{%
   \yquant@register@get@allowmultitrue%
   \let\yquant@register@multi@splitparts=\yquant@register@multi@splitparts@sepall%
   \preto\yquant@attrs@remaining{/yquant/operator/multi as single,}%
}

\protected\def\yquant@register@get@multiaslist{%
   \yquant@register@get@allowmultitrue%
   \let\yquant@register@multi@splitparts=\yquant@register@multi@splitparts@sort%
}

\let\yquant@register@multi@reset@original@splitparts=\yquant@register@multi@splitparts%
\protected\def\yquant@register@reset@multi{%
%   \yquant@register@get@allowmultifalse% not needed, as \yquant@circuit@operator automatically resets it
   \let\yquant@register@multi@splitparts=\yquant@register@multi@reset@original@splitparts%
}
% END_FOLD

% BEGIN_FOLD Getters: extract the requested information from the register with given id
\def\yquant@register@get@type#1{%
   \ifcsname\yquant@prefix registermap@#1\endcsname%
      \expandafter\expandafter\expandafter%
      \yquant@register@get@type@aux\csname\csname\yquant@prefix registermap@#1\endcsname\endcsname%
   \else%
      \expandafter\expandafter\expandafter%
      \yquant@register@get@type@aux\csname\yquant@prefix register@#1\endcsname%
   \fi%
}

\def\yquant@register@get@parent#1{%
   \ifcsname\yquant@prefix registermap@#1\endcsname%
      \expandafter\expandafter\expandafter%
      \yquant@register@get@type@aux\csname\yquant@prefix register@#1\endcsname%
   \else%
      \PackageError{yquant.sty}{Internal inconsistency detected}%
                   {Tried to get parent of a non-connected wire.}%
   \fi%
}

\def\yquant@register@get@type@aux#1#2#3#4#5#6{#1}

\def\yquant@register@get@x#1{%
   \ifcsname\yquant@prefix registermap@#1\endcsname%
      \expandafter\expandafter\expandafter%
      \yquant@register@get@x@aux\csname\csname\yquant@prefix registermap@#1\endcsname\endcsname%
   \else%
      \expandafter\expandafter\expandafter%
      \yquant@register@get@x@aux\csname\yquant@prefix register@#1\endcsname%
   \fi%
}

\def\yquant@register@get@x@aux#1#2#3#4#5#6{#2}

\def\yquant@register@get@height#1{%
   \expandafter\expandafter\expandafter%
   \yquant@register@get@height@aux\csname\yquant@prefix register@#1\endcsname%
}

\def\yquant@register@peek@height#1#2{%
   \expandafter\expandafter\expandafter%
   \yquant@register@get@height@aux\csname yquant@env#1@register@#2\endcsname%
}

\def\yquant@register@get@height@aux#1#2#3#4#5#6{\@firstofthree#3}

\def\yquant@register@get@depth#1{%
   \expandafter\expandafter\expandafter%
   \yquant@register@get@depth@aux\csname\yquant@prefix register@#1\endcsname%
}

\def\yquant@register@peek@depth#1#2{%
   \expandafter\expandafter\expandafter%
   \yquant@register@get@depth@aux\csname yquant@env#1@register@#2\endcsname%
}

\def\yquant@register@get@depth@aux#1#2#3#4#5#6{\@secondofthree#3}

\def\yquant@register@get@multispace#1{%
   \expandafter\expandafter\expandafter%
   \yquant@register@get@multispace@aux\csname\yquant@prefix register@#1\endcsname%
}

\def\yquant@register@get@multispace@aux#1#2#3#4#5#6{\@thirdofthree#3}

% The y parameter get macros exist in two forms: The protected one is used during the storage to the draw macro; it should never be executed. The env environment then maps them to their proper expandable forms.
\protected\def\yquant@register@get@y{%
   \PackageError%
      {yquant.sty}%
      {Execution of a get-y macro in an illegal context}%
      {get-y macros may not be called unless the yquant environment ends.}%
}

% This plays a similar role: It must never be expanded before the tikz command is invoked (because it does not exist).
\protected\def\nodepart{}

\def\yquant@register@get@y@unprotected#1{%
   \ifcsname\yquant@prefix registermap@#1\endcsname%
      \expandafter\expandafter\expandafter%
      \yquant@register@get@y@aux\csname\csname\yquant@prefix registermap@#1\endcsname\endcsname%
   \else%
      \expandafter\expandafter\expandafter%
      \yquant@register@get@y@aux\csname\yquant@prefix register@#1\endcsname%
   \fi%
}

\def\yquant@register@get@y@aux#1#2#3#4#5#6{#3}

% y distance between two registers.
\def\yquant@register@get@ydist#1#2{%
   \expandafter\yquant@abs\expandafter%
      {\the\dimexpr\yquant@register@get@y{#2}-\yquant@register@get@y{#1}\relax}%
}

\protected\def\yquant@register@get@y@@expandable{%
   \let\yquant@register@get@y=\yquant@register@get@y@unprotected%
}

\def\yquant@register@get@lastwire#1{%
   \ifcsname\yquant@prefix registermap@#1\endcsname%
      \expandafter\@firstoftwo%
   \else%
      \expandafter\@secondoftwo%
   \fi%
   {%
      \expandafter\expandafter\expandafter%
      \yquant@register@get@lastwire@aux\csname\csname\yquant@prefix registermap@#1\endcsname\endcsname%
   }{%
      \expandafter\expandafter\expandafter%
      \yquant@register@get@lastwire@aux\csname\yquant@prefix register@#1\endcsname%
   }%
}

\protected\def\yquant@register@get@lastwire@aux#1#2#3#4#5#6#7{%
   \def#7{#4}%
}

\def\yquant@register@get@style#1{%
   \ifcsname\yquant@prefix registermap@#1\endcsname%
      \expandafter\expandafter\expandafter%
      \yquant@register@get@style@aux\csname\csname\yquant@prefix registermap@#1\endcsname\endcsname%
   \else%
      \expandafter\expandafter\expandafter%
      \yquant@register@get@style@aux\csname\yquant@prefix register@#1\endcsname%
   \fi%
}

\def\yquant@register@get@style@aux#1#2#3#4#5#6{#5}

\protected\long\def\yquant@register@execclear@lastgate#1#2{%
   \ifcsname\yquant@prefix registermap@#1\endcsname%
      \expandafter%
      \yquant@register@execclear@lastgate@aux@i\csname\csname\yquant@prefix registermap@#1\endcsname\endcsname{#2}%
   \else%
      \expandafter%
      \yquant@register@execclear@lastgate@aux@i\csname\yquant@prefix register@#1\endcsname{#2}%
   \fi%
}

\def\yquant@register@execclear@lastgate@aux@i#1{%
   \expandafter\yquant@register@execclear@lastgate@aux@ii#1#1%
}

\long\def\yquant@register@execclear@lastgate@aux@ii#1#2#3#4#5#6#7#8{%
   \ifstrempty{#6}\relax{%
      #6{#8}%
      \xdef#7{\unexpanded{{#1}{#2}{#3}{#4}{#5}{}}}%
   }%
}

\def\yquant@register@get@typeywire#1{%
   \ifcsname\yquant@prefix registermap@#1\endcsname%
      \expandafter\@firstoftwo%
   \else%
      \expandafter\@secondoftwo%
   \fi%
   {%
      \expandafter\expandafter\expandafter%
      \yquant@register@get@typeywire@aux\csname\csname\yquant@prefix registermap@#1\endcsname\endcsname%
   }{%
      \expandafter\expandafter\expandafter%
      \yquant@register@get@typeywire@aux\csname\yquant@prefix register@#1\endcsname%
   }%
}

\protected\def\yquant@register@get@typeywire@aux#1#2#3#4#5#6#7#8#9{%
   \def#7{#1}%
   \def#8{#3}%
   \def#9{#4}%
}%

% Set #1 to the maximum x value found between #2 and #3
\protected\def\yquant@register@get@maxxrange#1#2#3{%
   \begingroup%
      \dimen0=-16383.99999pt %
      \yquant@for \yquant@register@get@maxx@i := #2 to #3 {%
         \dimen2=\yquant@register@get@x{\yquant@register@get@maxx@i}\relax%
         \ifdim\dimen0<\dimen2 %
            \dimen0=\dimen2 %
         \fi%
      }%
      \expandafter%
   \endgroup%
   \expandafter\def\expandafter#1\expandafter{\the\dimen0}%
}

% Set #1 to the maximum x value found in the list #2
\protected\def\yquant@register@get@maxxlist#1#2{%
   \begingroup%
      \dimen0=-16383.99999pt %
      \def\do##1{%
         \dimen2=\yquant@register@get@x{##1}\relax%
         \ifdim\dimen0<\dimen2 %
            \dimen0=\dimen2 %
         \fi%
      }%
      \dolistloop{#2}%
      \expandafter%
   \endgroup%
   \expandafter\def\expandafter#1\expandafter{\the\dimen0}%
}

\protected\def\yquant@register@flag@clean#1{%
   \ifstrequal{#1}{init}{%
      \advance\count8 by 1 %
   }\relax%
}
% END_FOLD

% BEGIN_FOLD Setters: change register information
\protected\long\def\yquant@register@set@@aux#1#2#3{%
   \xdef#1{\expandafter#2#1{#3}}%
}

\protected\def\yquant@register@set@type#1{%
   \ifcsname\yquant@prefix registermap@#1\endcsname%
      \expandafter\@firstoftwo%
   \else%
      \expandafter\@secondoftwo%
   \fi%
   {%
      \expandafter\yquant@register@set@@aux%
         \csname\csname\yquant@prefix registermap@#1\endcsname\endcsname%
   }{%
      \expandafter\yquant@register@set@@aux%
      \csname\yquant@prefix register@#1\endcsname%
   }%
   \yquant@register@set@type@aux%
}

\long\def\yquant@register@set@type@aux#1#2#3#4#5#6#7{%
   {#7}\unexpanded{{#2}{#3}{#4}{#5}{#6}}%
}

\protected\def\yquant@register@set@x#1{%
   \ifcsname\yquant@prefix registermap@#1\endcsname%
      \expandafter\@firstoftwo%
   \else%
      \expandafter\@secondoftwo%
   \fi%
   {%
      \expandafter\yquant@register@set@@aux%
         \csname\csname\yquant@prefix registermap@#1\endcsname\endcsname%
   }{%
      \expandafter\yquant@register@set@@aux%
      \csname\yquant@prefix register@#1\endcsname%
   }%
   \yquant@register@set@x@aux%
}

\long\def\yquant@register@set@x@aux#1#2#3#4#5#6#7{%
   \unexpanded{{#1}}{#7}\unexpanded{{#3}{#4}{#5}{#6}}%
}

\protected\def\yquant@register@update@height#1#2{%
   \unless\ifyquant@lang@attr@overlay@height%
      \ifdim#2>%
         \expandafter\expandafter\expandafter%
            \yquant@register@get@height@aux\csname\yquant@prefix register@#1\endcsname%
         \relax%
         \expandafter\yquant@register@set@@aux%
            \csname\yquant@prefix register@#1\endcsname%
            \yquant@register@set@height@aux{#2}%
      \fi%
   \fi%
}

\protected\def\yquant@register@set@height@remote#1#2#3{%
   \expandafter\yquant@register@set@@aux%
      \csname yquant@env#1@register@#2\endcsname%
      \yquant@register@set@height@aux{#3}%
}

\long\def\yquant@register@set@height@aux#1#2#3#4#5#6#7{%
   \unexpanded{{#1}{#2}}%
   {{#7}%
    {\unexpanded\expandafter{\@secondofthree#3}}%
    {\unexpanded\expandafter{\@thirdofthree#3}}}%
   \unexpanded{{#4}{#5}{#6}}%
}

\protected\def\yquant@register@update@depth#1#2{%
   \unless\ifyquant@lang@attr@overlay@depth%
      \ifdim#2>%
         \expandafter\expandafter\expandafter%
            \yquant@register@get@depth@aux\csname\yquant@prefix register@#1\endcsname%
         \relax%
         \expandafter\yquant@register@set@@aux%
            \csname\yquant@prefix register@#1\endcsname%
            \yquant@register@set@depth@aux{#2}%
      \fi%
   \fi%
}

\protected\def\yquant@register@set@depth@remote#1#2#3{%
   \expandafter\yquant@register@set@@aux%
      \csname yquant@env#1@register@#2\endcsname%
      \yquant@register@set@depth@aux{#3}%
}

\long\def\yquant@register@set@depth@aux#1#2#3#4#5#6#7{%
   \unexpanded{{#1}{#2}}%
   {{\unexpanded\expandafter{\@firstofthree#3}}%
    {#7}%
    {\unexpanded\expandafter{\@thirdofthree#3}}}%
   \unexpanded{{#4}{#5}{#6}}%
}

\protected\def\yquant@register@update@multispace#1#2#3{%
   \unless\ifnum#1<#2 %
      \PackageError{yquant.sty}{Internal inconsistency detected}%
                   {Setting multispace part in wrong order.}%
   \fi%
   \unless\ifyquant@lang@attr@overlay@multi%
      \begingroup%
         \edef\tmp{%
            \expandafter\expandafter\expandafter%
            \yquant@register@get@multispace@aux\csname\yquant@prefix register@#1\endcsname%
         }%
         \let\old=\tmp%
         \yquant@list@eupdateorinsert\tmp{#2}{#3}%
         \unless\ifx\old\tmp%
            \expandafter\yquant@register@set@@aux%
               \csname\yquant@prefix register@#1\endcsname%
               \yquant@register@set@multispace@aux\tmp%
         \fi%
      \endgroup%
   \fi%
}

\long\def\yquant@register@set@multispace@aux#1#2#3#4#5#6#7{%
   \unexpanded{{#1}{#2}}%
   {{\unexpanded\expandafter{\@firstofthree#3}}%
    {\unexpanded\expandafter{\@secondofthree#3}}%
    {#7}}%
   \unexpanded{{#4}{#5}{#6}}%
}

\protected\def\yquant@register@inject@extents#1#2{%
   % enlarge the last subcircuit that was created previously by height #1 and depth #2.
   % We enforce subcircuits to have registers, so no check needed.
   \expandafter\yquant@register@set@@aux%
      \csname yquant@env\the\yquant@env @register@1\endcsname%
      \yquant@register@inject@height@aux{#1}%
   \expandafter\yquant@register@set@@aux%
      \csname yquant@env\the\yquant@env @register@\csname yquant@env\the\yquant@env @registers\endcsname\endcsname%
      \yquant@register@inject@depth@aux{#2}%
}

\long\def\yquant@register@inject@height@aux#1#2#3#4#5#6#7{%
   \unexpanded{{#1}{#2}}%
   {{\the\dimexpr\@firstofthree#3+#7\relax}%
    {\unexpanded\expandafter{\@secondofthree#3}}%
    {\unexpanded\expandafter{\@thirdofthree#3}}}%
   \unexpanded{{#4}{#5}{#6}}%
}

\long\def\yquant@register@inject@depth@aux#1#2#3#4#5#6#7{%
   \unexpanded{{#1}{#2}}%
   {{\unexpanded\expandafter{\@firstofthree#3}}%
    {\the\dimexpr\@secondofthree#3+#7\relax}%
    {\unexpanded\expandafter{\@thirdofthree#3}}}%
   \unexpanded{{#4}{#5}{#6}}%
}

\protected\def\yquant@register@set@y#1{%
   \ifcsname\yquant@prefix registermap@#1\endcsname%
      \expandafter\@firstoftwo%
   \else%
      \expandafter\@secondoftwo%
   \fi%
   {%
      \expandafter\yquant@register@set@@aux%
         \csname\csname\yquant@prefix registermap@#1\endcsname\endcsname%
   }{%
      \expandafter\yquant@register@set@@aux%
      \csname\yquant@prefix register@#1\endcsname%
   }%
   \yquant@register@set@y@aux%
}

\long\def\yquant@register@set@y@aux#1#2#3#4#5#6#7{%
   \unexpanded{{#1}{#2}}{#7}\unexpanded{{#4}{#5}{#6}}%
}

\protected\def\yquant@register@set@lastwire#1{%
   \ifcsname\yquant@prefix registermap@#1\endcsname%
      \expandafter\@firstoftwo%
   \else%
      \expandafter\@secondoftwo%
   \fi%
   {%
      \expandafter\yquant@register@set@@aux%
         \csname\csname\yquant@prefix registermap@#1\endcsname\endcsname%
   }{%
      \expandafter\yquant@register@set@@aux%
      \csname\yquant@prefix register@#1\endcsname%
   }%
   \yquant@register@set@lastwire@aux%
}

\long\def\yquant@register@set@lastwire@aux#1#2#3#4#5#6#7{%
   \unexpanded{{#1}{#2}{#3}}{#7}\unexpanded{{#5}{#6}}%
}

\protected\def\yquant@register@set@typelastwire#1{%
   \ifcsname\yquant@prefix registermap@#1\endcsname%
      \PackageError{yquant.sty}{Internal inconsistency detected}%
                   {Setting type and lastwire was requested for a subcircuit.}%
   \fi%
   \expandafter\yquant@register@set@@aux%
      \csname\yquant@prefix register@#1\endcsname%
      \yquant@register@set@typelastwire@aux%
}

\long\def\yquant@register@set@typelastwire@aux#1#2#3#4#5#6#7{%
   {\@firstoftwo#7}\unexpanded{{#2}{#3}}{\@secondoftwo#7}\unexpanded{{#5}{#6}}%
}

\protected\def\yquant@register@set@style#1{%
   \ifcsname\yquant@prefix registermap@#1\endcsname%
      \expandafter\@firstoftwo%
   \else%
      \expandafter\@secondoftwo%
   \fi%
   {%
      \expandafter\yquant@register@set@@aux%
         \csname\csname\yquant@prefix registermap@#1\endcsname\endcsname%
   }{%
      \expandafter\yquant@register@set@@aux%
      \csname\yquant@prefix register@#1\endcsname%
   }%
   \yquant@register@set@style@aux%
}

\long\def\yquant@register@set@style@aux#1#2#3#4#5#6#7{%
   \unexpanded{{#1}{#2}{#3}{#4}}{#7}\unexpanded{{#6}}%
}

\protected\def\yquant@register@set@lastgate#1{%
   \ifcsname\yquant@prefix registermap@#1\endcsname%
      \expandafter\@firstoftwo%
   \else%
      \expandafter\@secondoftwo%
   \fi%
   {%
      \expandafter\yquant@register@set@@aux%
         \csname\csname\yquant@prefix registermap@#1\endcsname\endcsname%
   }{%
      \expandafter\yquant@register@set@@aux%
      \csname\yquant@prefix register@#1\endcsname%
   }%
   \yquant@register@set@lastgate@aux%
}

\long\def\yquant@register@set@lastgate@aux#1#2#3#4#5#6#7{%
   \unexpanded{{#1}{#2}{#3}{#4}{#5}}{#7}%
}

\long\def\yquant@register@set@typelastgate@aux#1#2#3#4#5#6#7{%
   {\@firstoftwo#7}\unexpanded{{#2}{#3}{#4}{#5}}{\@secondoftwo#7}%
}
% END_FOLD

==> yquant-shapes.tex <==
\long\def\pgf@sh@clippathhorz#1{%
   \csgdef{pgf@sh@cliphorz@\pgf@sm@shape@name}{#1}%
}
\let\pgf@sh@clippath=\pgf@sh@clippathhorz%
\long\def\pgf@sh@clippathvert#1{%
   \csgdef{pgf@sh@clipvert@\pgf@sm@shape@name}{#1}%
}
\def\pgf@sh@inheritclippath[from=#1]{%
   \global\csletcs{pgf@sh@cliphorz@\pgf@sm@shape@name}{pgf@sh@cliphorz@#1}%
   \global\csletcs{pgf@sh@clipvert@\pgf@sm@shape@name}{pgf@sh@clipvert@#1}%
}
\patchcmd%
   \pgfdeclareshape%
   {\let\anchorborder=\pgf@sh@anchorborder}%
   {\let\anchorborder=\pgf@sh@anchorborder%
    \let\clippathhorz=\pgf@sh@clippathhorz%
    \let\clippathvert=\pgf@sh@clippathvert%
    \let\clippath=\pgf@sh@clippath%
    \let\inheritclippath=\pgf@sh@inheritclippath}%
   {}%
   {\PackageError{yquant.sty}%
                 {Failed to patch \string\pgfdeclareshape}%
                 {yquant could not provide a necessary extension to pgf.}}%
% Every shape additionally provides information about how it should clip the wires. The clipping softpath instructions of shape #1 are stored into \pgfshapeclippath[horz|vert]result. The path is drawn with the tikz options #2 in place.
\protected\def\pgfshapeclippath#1#2{%
   % Ok, check whether #1 is known!
   \ifcsname pgf@sh@ns@#1\endcsname%
      \begin{pgfinterruptpath}%
         \edef\pgfreferencednodename{#1}% for use inside of anchors.
         % install the given style and extract whether we draw a line.
         \let\tikz@mode=\pgfutil@empty%
         \tikzset{every path/.try,#2}%
         \edef\oldpgflinewidth{\the\pgflinewidth}%
         \tikz@mode@drawfalse%
         \tikz@mode%
         \unless\iftikz@mode@draw%
            \pgflinewidth=0pt %
         \fi%
         % MW install special macros
         \csname pgf@sh@ma@#1\endcsname% MW
         % install special coordinates
         \csname pgf@sh@np@#1\endcsname%
         \pgfsettransform{\csname pgf@sh@nt@#1\endcsname}%
         \csname pgf@sh@cliphorz@\csname pgf@sh@ns@#1\endcsname\endcsname%
         \pgfsyssoftpath@getcurrentpath\pgfshapeclippathresult%
         \pgfprocessround{\pgfshapeclippathresult}{\pgfshapeclippathresult}%
         \global\let\pgfshapeclippathhorzresult=\pgfshapeclippathresult%
         \ifcsname pgf@sh@clipvert@\csname pgf@sh@ns@#1\endcsname\endcsname%
            % different clipping in vertical direction
            \pgfsyssoftpath@setcurrentpath\pgfutil@empty%
            \csname pgf@sh@clipvert@\csname pgf@sh@ns@#1\endcsname\endcsname%
            \pgfsyssoftpath@getcurrentpath\pgfshapeclippathresult%
            \pgfprocessround{\pgfshapeclippathresult}{\pgfshapeclippathresult}%
         \fi%
         \global\let\pgfshapeclippathvertresult=\pgfshapeclippathresult%
      \end{pgfinterruptpath}%
   \else%
      \pgferror{No shape named #1 is known}%
      \global\let\pgfshapeclippathhorzresult=\empty%
      \global\let\pgfshapeclippathvertresult=\empty%
   \fi%
}

\pgfdeclareshape{yquant-text}{%
   \inheritsavedanchors[from=rectangle]%
   \foreach \anc in {center, mid, base, north, south, west, mid west, base west, north west, south west, east, mid east, base east, north east, south east} {%
      \inheritanchor[from=rectangle]{\anc}%
   }%
   \inheritanchorborder[from=rectangle]%
   \inheritbackgroundpath[from=rectangle]%
   \clippath{%
      % all pgf temporaries may be overwritten by \pgfpathrectanglecorners
      \begingroup%
         % the outer sep may depend on the line width (though there may not be any line)
         \pgflinewidth=\oldpgflinewidth%
         \global\@tempdima=\pgfkeysvalueof{/pgf/outer xsep} %
         \global\@tempdimb=\pgfkeysvalueof{/pgf/outer ysep} %
      \endgroup%
      \advance\@tempdima by -.5\pgflinewidth%
      \advance\@tempdimb by -.5\pgflinewidth%
      \pgfpathrectanglecorners%
         {\southwest%
          \advance\pgf@x by \@tempdima%
          \advance\pgf@y by \@tempdimb%
         }%
         {\northeast%
          \advance\pgf@x by -\@tempdima%
          \advance\pgf@y by -\@tempdimb%
         }%
   }%
}

\pgfdeclareshape{yquant-rectangle}{%
   % BEGIN_FOLD Saved anchors
   \saveddimen\xradius{%
      \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/tikz/x radius}}%
      \ifdim\wd\pgfnodeparttextbox=0pt %
         \pgf@xa=0pt %
      \else%
         \pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/inner xsep}}%
      \fi%
      \ifdim\dimexpr.5\wd\pgfnodeparttextbox+\pgf@xa\relax>\pgf@x%
         \pgf@x=\dimexpr.5\wd\pgfnodeparttextbox+\pgf@xa\relax%
      \fi%
   }%
   \saveddimen\yradius{%
      \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/tikz/y radius}}%
      \ifdim\dimexpr\ht\pgfnodeparttextbox+\dp\pgfnodeparttextbox\relax=0pt %
         \pgf@xa=0pt %
      \else%
         \pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/inner ysep}}%
      \fi%
      \@tempdima=\dimexpr.5\ht\pgfnodeparttextbox+.5\dp\pgfnodeparttextbox+\pgf@xa\relax%
      \ifdim\@tempdima>\pgf@x%
         \pgf@x=\@tempdima%
      \fi%
   }%
   \savedanchor\stext{%
      \pgfqpoint%
         {-.5\wd\pgfnodeparttextbox}%
         {-\dimexpr.5\ht\pgfnodeparttextbox-.5\dp\pgfnodeparttextbox\relax}%
   }%
   % END_FOLD
   % BEGIN_FOLD Operator anchors
   \global\cslet{pgf@anchor@yquant-rectangle@center}\pgfpointorigin%
   \anchor{text}{\stext}%
   \anchor{north}%
          {\pgfqpoint{0pt}%
                     {\yradius}}%
   \anchor{north east}%
          {\pgfqpoint{\xradius}%
                     {\yradius}}%
   \anchor{east}%
          {\pgfqpoint{\xradius}%
                     {0pt}}%
   \anchor{south east}%
          {\pgfqpoint{\xradius}%
                     {-\yradius}}%
   \anchor{south}%
          {\pgfqpoint{0pt}%
                     {-\yradius}}%
   \anchor{south west}%
          {\pgfqpoint{-\xradius}%
                     {-\yradius}}%
   \anchor{west}%
          {\pgfqpoint{-\xradius}% \dimexpr not really necessary...
                     {0pt}}%
   \anchor{north west}%
          {\pgfqpoint{-\xradius}%
                     {\yradius}}%
   \anchorborder{%
      \@tempdima=\pgf@x%
      \@tempdimb=\pgf@y%
      \pgfpointborderrectangle{\pgfqpoint{\@tempdima}{\@tempdimb}}%
                              {\pgfqpoint{\xradius}{\yradius}}%
   }%
   % END_FOLD
   % BEGIN_FOLD Path
   \backgroundpath{%
      \pgfpathrectanglecorners%
         {\pgfqpoint{-\xradius}{\yradius}}%
         {\pgfqpoint{\xradius}{-\yradius}}%
   }%
   \clippath{%
      \pgfpathrectanglecorners%
         {\pgfqpoint{-\dimexpr\xradius+.5\pgflinewidth\relax}%
                    {\dimexpr\yradius+.5\pgflinewidth\relax}}%
         {\pgfqpoint{\dimexpr\xradius+.5\pgflinewidth\relax}%
                    {-\dimexpr\yradius+.5\pgflinewidth\relax}}%
   }%
   % END_FOLD
}

\pgfdeclareshape{yquant-circle}{%
   \inheritsavedanchors[from=yquant-rectangle]%
   \foreach \anc in {center, north, east, south, west, text} {%
      \inheritanchor[from=yquant-rectangle]{\anc}%
   }%
   \anchor{north east}%
          {\pgfqpoint{.707107\dimexpr\xradius\relax}%
                     {.707107\dimexpr\yradius\relax}}%
   \anchor{south east}%
          {\pgfqpoint{.707107\dimexpr\xradius\relax}%
                     {-.707107\dimexpr\yradius\relax}}%
   \anchor{south west}%
          {\pgfqpoint{-.707107\dimexpr\xradius\relax}%
                     {-.707107\dimexpr\yradius\relax}}%
   \anchor{north west}%
          {\pgfqpoint{-.707107\dimexpr\xradius\relax}%
                     {.707107\dimexpr\yradius\relax}}%
   \anchorborder{%
      \@tempdima=\pgf@x%
      \@tempdimb=\pgf@y%
      \pgfpointborderellipse{\pgfqpoint{\@tempdima}{\@tempdimb}}%
                            {\pgfqpoint{.707107\dimexpr\xradius\relax}%
                                       {.707107\dimexpr\yradius\relax}}%
   }%
   \backgroundpath{%
      \pgfpathellipse{\pgfpointorigin}%
                     {\pgfqpoint{\xradius}{0pt}}%
                     {\pgfqpoint{0pt}{\yradius}}%
   }%
   \clippath{%
      \pgfpathellipse{\pgfpointorigin}%
                     {\pgfqpoint{\dimexpr\xradius+.5\pgflinewidth}{0pt}}%
                     {\pgfqpoint{0pt}{\dimexpr\yradius+.5\pgflinewidth}}%
   }%
}

\pgfdeclareshape{yquant-slash}{%
   \saveddimen\xradius{%
      \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/tikz/x radius}}%
   }%
   \saveddimen\yradius{%
      \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/tikz/y radius}}%
   }%
   \foreach \anc in {center, north, north east, east, south east, south, south west, west, north west} {%
      \inheritanchor[from=yquant-rectangle]{\anc}%
   }%
   \inheritanchorborder[from=yquant-rectangle]%
   \backgroundpath{%
      \pgfpathmoveto{\pgfqpoint{\xradius}{\yradius}}%
      \pgfpathlineto{\pgfqpoint{-\xradius}{-\yradius}}%
   }%
   \clippath{%
      % we need to clip to the line; but this is not possible, we can only clip to the inner of a path. For this reason, calculate the rectangle that represents the line.
      % TODO: for round line endings, this is not a rectangle. Only a problem if the yradius is so short that the slash ends within a wire.
      \ifcsname yquant@math@cache1@\xradius @\yradius @\the\pgflinewidth\endcsname%
         \letcs\tmp{yquant@math@cache1@\xradius @\yradius @\the\pgflinewidth}%
         \dimen2=\expandafter\@firstoftwo\tmp%
         \dimen4=\expandafter\@secondoftwo\tmp%
      \else%
         % cos(arctan(x)) = 1/sqrt(1+x^2)
         % sin(arctan(x)) = x/sqrt(1+x^2)
         \dimen2=\xradius %
         \dimen4=\yradius %
         % if we divide by a dimension, it is internally converted to sp, so we divide by its pt-value and again by 65536. Same for multiplication. etex fuses muldiv to 64bit, so we don't get overflows.
         \dimen0=\dimexpr\dimen4*\dimen4/\dimen2*65536/\dimen2\relax%
         % calculate the sqrt; but \pgfmathsqrt@ expects a real number without dimension suffix. It internally does \expandafter\pgfmath@x#1pt\relax, so just gobble the additional pt.
         \pgfmathsqrt@{\the\dimexpr1pt+\dimen0\relax\@gobbletwo}%
         \pgfmathreciprocal@\pgfmathresult%
         \dimen2=\dimexpr.5\pgflinewidth*\dimexpr\pgfmathresult pt\relax/65536\relax%
         \dimen4=\dimexpr\dimexpr\yradius\relax*\dimen2/\dimexpr\xradius\relax\relax%
         \csxdef{yquant@math@cache1@\xradius @\yradius @\the\pgflinewidth}%
                {{\the\dimen2}{\the\dimen4}}%
      \fi%
      \pgfpathmoveto{\pgfqpoint{-\dimexpr\xradius+\dimen4\relax}%
                               {-\dimexpr\yradius-\dimen2\relax}}%
      \pgfpathlineto{\pgfqpoint{\dimexpr\xradius-\dimen4\relax}%
                               {\dimexpr\yradius+\dimen2\relax}}%
      \pgfpathlineto{\pgfqpoint{\dimexpr\xradius+\dimen4\relax}%
                               {\dimexpr\yradius-\dimen2\relax}}%
      \pgfpathlineto{\pgfqpoint{-\dimexpr\xradius-\dimen4\relax}%
                               {-\dimexpr\yradius+\dimen2\relax}}%
      \pgfpathclose%
   }%
}

\pgfdeclareshape{yquant-swap}{%
   \inheritsavedanchors[from=yquant-slash]%
   \foreach \anc in {center, north, north east, east, south east, south, south west, west, north west} {%
      \inheritanchor[from=yquant-rectangle]{\anc}%
   }%
   \inheritanchorborder[from=yquant-rectangle]%
   \backgroundpath{%
      \pgfpathmoveto{\pgfqpoint{-\xradius}{\yradius}}%
      \pgfpathlineto{\pgfqpoint{\xradius}{-\yradius}}%
      \pgfpathmoveto{\pgfqpoint{\xradius}{\yradius}}%
      \pgfpathlineto{\pgfqpoint{-\xradius}{-\yradius}}%
   }%
   \clippathhorz{%
      % we need to clip to the line; but this is not possible, we can only clip to the inner of a path. For this reason, calculate the rectangle that represents the line.
      % TODO: for round line endings, this is not a rectangle. Only a problem if the yradius is so short that the slash ends within a wire.
      \ifcsname yquant@math@cache1@\xradius @\yradius @\the\pgflinewidth\endcsname%
         \letcs\tmp{yquant@math@cache1@\xradius @\yradius @\the\pgflinewidth}%
         \dimen2=\expandafter\@firstoftwo\tmp%
         \dimen4=\expandafter\@secondoftwo\tmp%
      \else%
         % cos(arctan(x)) = 1/sqrt(1+x^2)
         % sin(arctan(x)) = x/sqrt(1+x^2)
         \dimen2=\xradius %
         \dimen4=\yradius %
         % if we divide by a dimension, it is internally converted to sp, so we divide by its pt-value and again by 65536. Same for multiplication. etex fuses muldiv to 64bit, so we don't get overflows.
         \dimen0=\dimexpr\dimen4*\dimen4/\dimen2*65536/\dimen2\relax%
         % calculate the sqrt; but \pgfmathsqrt@ expects a real number without dimension suffix. It internally does \expandafter\pgfmath@x#1pt\relax, so just gobble the additional pt.
         \pgfmathsqrt@{\the\dimexpr1pt+\dimen0\relax\@gobbletwo}%
         \pgfmathreciprocal@\pgfmathresult%
         \dimen2=\dimexpr.5\pgflinewidth*\dimexpr\pgfmathresult pt\relax/65536\relax%
         \dimen4=\dimexpr\dimexpr\yradius\relax*\dimen2/\dimexpr\xradius\relax\relax%
         \csxdef{yquant@math@cache1@\xradius @\yradius @\the\pgflinewidth}%
                {{\the\dimen2}{\the\dimen4}}%
      \fi%
      \dimen6=\dimexpr\dimen2*\dimexpr\xradius\relax/\dimexpr\yradius\relax+%
                      \dimen2*\dimexpr\yradius\relax/\dimexpr\xradius\relax\relax%
      \pgfpathmoveto{\pgfqpoint{-\dimexpr\xradius+\dimen4\relax}%
                               {\dimexpr\yradius-\dimen2\relax}}%
      \pgfpathlineto{\pgfqpoint{-\dimexpr\xradius-\dimen4\relax}%
                               {\dimexpr\yradius+\dimen2\relax}}%
      \pgfpathlineto{\pgfqpoint{\dimexpr\xradius-\dimen4\relax}%
                               {\dimexpr\yradius+\dimen2\relax}}%
      \pgfpathlineto{\pgfqpoint{\dimexpr\xradius+\dimen4\relax}%
                               {\dimexpr\yradius-\dimen2\relax}}%
      \pgfpathlineto{\pgfqpoint{\dimen6}{0pt}}%
      \pgfpathlineto{\pgfqpoint{\dimexpr\xradius+\dimen4\relax}%
                               {-\dimexpr\yradius-\dimen2\relax}}%
      \pgfpathlineto{\pgfqpoint{\dimexpr\xradius-\dimen4\relax}%
                               {-\dimexpr\yradius+\dimen2\relax}}%
      \pgfpathlineto{\pgfqpoint{-\dimexpr\xradius-\dimen4\relax}%
                               {-\dimexpr\yradius+\dimen2\relax}}%
      \pgfpathlineto{\pgfqpoint{-\dimexpr\xradius+\dimen4\relax}%
                               {-\dimexpr\yradius-\dimen2\relax}}%
      \pgfpathlineto{\pgfqpoint{-\dimen6}{0pt}}%
      \pgfpathclose%
   }%
   \clippathvert{%
      % we need to clip to the line; but this is not possible, we can only clip to the inner of a path. For this reason, calculate the rectangle that represents the line.
      % TODO: for round line endings, this is not a rectangle. Only a problem if the yradius is so short that the slash ends within a wire.
      \ifcsname yquant@math@cache1@\xradius @\yradius @\the\pgflinewidth\endcsname%
         \letcs\tmp{yquant@math@cache1@\xradius @\yradius @\the\pgflinewidth}%
         \dimen2=\expandafter\@firstoftwo\tmp%
         \dimen4=\expandafter\@secondoftwo\tmp%
      \else%
         % cos(arctan(x)) = 1/sqrt(1+x^2)
         % sin(arctan(x)) = x/sqrt(1+x^2)
         \dimen2=\xradius %
         \dimen4=\yradius %
         % if we divide by a dimension, it is internally converted to sp, so we divide by its pt-value and again by 65536. Same for multiplication. etex fuses muldiv to 64bit, so we don't get overflows.
         \dimen0=\dimexpr\dimen4*\dimen4/\dimen2*65536/\dimen2\relax%
         % calculate the sqrt; but \pgfmathsqrt@ expects a real number without dimension suffix. It internally does \expandafter\pgfmath@x#1pt\relax, so just gobble the additional pt.
         \pgfmathsqrt@{\the\dimexpr1pt+\dimen0\relax\@gobbletwo}%
         \pgfmathreciprocal@\pgfmathresult%
         \dimen2=\dimexpr.5\pgflinewidth*\dimexpr\pgfmathresult pt\relax/65536\relax%
         \dimen4=\dimexpr\dimexpr\yradius\relax*\dimen2/\dimexpr\xradius\relax\relax%
         \csxdef{yquant@math@cache1@\xradius @\yradius @\the\pgflinewidth}%
                {{\the\dimen2}{\the\dimen4}}%
      \fi%
      \dimen6=\dimexpr\dimen4*\dimexpr\xradius\relax/\dimexpr\yradius\relax+%
                      \dimen4*\dimexpr\yradius\relax/\dimexpr\xradius\relax\relax%
      \pgfpathmoveto{\pgfqpoint{-\dimexpr\xradius+\dimen4\relax}%
                               {\dimexpr\yradius-\dimen2\relax}}%
      \pgfpathlineto{\pgfqpoint{-\dimexpr\xradius-\dimen4\relax}%
                               {\dimexpr\yradius+\dimen2\relax}}%
      \pgfpathlineto{\pgfqpoint{0pt}{\dimen6}}%
      \pgfpathlineto{\pgfqpoint{\dimexpr\xradius-\dimen4\relax}%
                               {\dimexpr\yradius+\dimen2\relax}}%
      \pgfpathlineto{\pgfqpoint{\dimexpr\xradius+\dimen4\relax}%
                               {\dimexpr\yradius-\dimen2\relax}}%
      \pgfpathlineto{\pgfqpoint{\dimexpr\xradius+\dimen4\relax}%
                               {-\dimexpr\yradius-\dimen2\relax}}%
      \pgfpathlineto{\pgfqpoint{\dimexpr\xradius-\dimen4\relax}%
                               {-\dimexpr\yradius+\dimen2\relax}}%
      \pgfpathlineto{\pgfqpoint{0pt}{-\dimen6}}%
      \pgfpathlineto{\pgfqpoint{-\dimexpr\xradius-\dimen4\relax}%
                               {-\dimexpr\yradius+\dimen2\relax}}%
      \pgfpathlineto{\pgfqpoint{-\dimexpr\xradius+\dimen4\relax}%
                               {-\dimexpr\yradius-\dimen2\relax}}%
      \pgfpathclose%
   }%
}

\pgfdeclareshape{yquant-oplus}{%
   \inheritsavedanchors[from=yquant-slash]%
   \foreach \anc in {center, north, north east, east, south east, south, south west, west, north west} {%
      \inheritanchor[from=yquant-circle]{\anc}%
   }%
   \inheritanchorborder[from=yquant-circle]%
   \backgroundpath{%
      \pgfpathmoveto{\pgfqpoint{0pt}{\yradius}}%
      \pgfpathlineto{\pgfqpoint{0pt}{-\yradius}}%
      \pgfpathmoveto{\pgfqpoint{-\xradius}{0pt}}%
      \pgfpathlineto{\pgfqpoint{\xradius}{0pt}}%
      \pgfpathellipse{\pgfpointorigin}%
                     {\pgfqpoint{\xradius}{0pt}}%
                     {\pgfqpoint{0pt}{\yradius}}%
   }%
   \inheritclippath[from=yquant-circle]%
}

\pgfdeclareshape{yquant-measure}{%
   \saveddimen\xradius{%
      \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/tikz/x radius}}%
      \ifdim.5\wd\pgfnodeparttextbox>\pgf@x%
         \pgf@x=.5\wd\pgfnodeparttextbox%
      \fi%
   }%
   \saveddimen\yradius{%
      \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/tikz/y radius}}%
      \ifdim\dimexpr\ht\pgfnodeparttextbox+\dp\pgfnodeparttextbox\relax=0pt %
         \ifdim\pgf@x<1.25mm %
            \pgf@x=1.25mm %
         \fi%
      \else%
         \pgf@y=\dimexpr.5\ht\pgfnodeparttextbox+.5\dp\pgfnodeparttextbox+2pt\relax%
         \ifyquant@config@internal@multi@main%
            \advance\pgf@y by 1.25mm %
         \fi%
         \ifdim\pgf@x<\pgf@y%
            \pgf@x=\pgf@y%
         \fi%
      \fi%
   }%
   \savedanchor\stext{%
      \ifyquant@config@internal@multi@main%
         \pgfqpoint%
            {-.5\wd\pgfnodeparttextbox}%
            {\dp\pgfnodeparttextbox}%
      \else%
         \pgfqpoint%
            {-.5\wd\pgfnodeparttextbox}%
            {-\dimexpr.5\ht\pgfnodeparttextbox-.5\dp\pgfnodeparttextbox\relax}%
      \fi%
   }%
   \saveddimen\textheight{%
      \pgf@x=\ht\pgfnodeparttextbox%
   }%
   \savedmacro\main{%
      \ifyquant@config@internal@multi@main%
         \def\main{\noexpand\yquant@config@internal@multi@maintrue}%
      \else%
         \ifdim\dimexpr\ht\pgfnodeparttextbox+\dp\pgfnodeparttextbox\relax=0pt%
            \def\main{\noexpand\yquant@config@internal@multi@maintrue}%
         \else%
            \def\main{\noexpand\yquant@config@internal@multi@mainfalse}%
         \fi%
      \fi%
   }%
   \foreach \anc in {center, north, north east, east, south east, south, south west, west, north west} {%
      \inheritanchor[from=yquant-rectangle]{\anc}%
   }%
   \anchor{text}{%
      \stext%
      \main%
      \ifyquant@config@internal@multi@main%
         \pgf@y=\dimexpr-\yradius+1pt+\pgf@y\relax%
      \fi%
   }%
   \inheritanchorborder[from=yquant-rectangle]%
   \inheritbackgroundpath[from=yquant-rectangle]%
   \inheritclippath[from=yquant-rectangle]%
   \beforebackgroundpath{%
      \main%
      % we only draw the meter symbol if this is the main part of a multi-register (or there is no text)
      \ifyquant@config@internal@multi@main%
         % Make sure the meter does not extend beyond the box (we are in a scope here)
         \path [clip]%
            (-\xradius, \yradius) rectangle (\xradius, -\yradius);%
         % The position of the meter symbol depends on the presence of the text. If there is no text, we just vertically center. If there is some text, we shift the symbol upwards from the text until there is no overlap any more.
         \csname pgf@anchor@yquant-measure@text\endcsname%
         \advance\pgf@y by \textheight\relax%
         \ifdim\pgf@y<-1.15mm %
            \@tempdima=-1.15mm %
         \else%
            \@tempdima=\dimexpr\pgf@y+2pt\relax%
         \fi%
         \path [/yquant/operators/every measure meter]%
            (-2.25mm, \@tempdima) arc[start angle=160, end angle=20,%
                                      x radius=2.25mm, y radius=1.4mm]%
            (0, \@tempdima) -- ++(1.6mm, 2.3mm);%
      \fi%
   }%
}

\pgfdeclareshape{yquant-dmeter}{%
   \saveddimen\xradius{%
      \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/tikz/x radius}}%
      \ifdim\wd\pgfnodeparttextbox=0pt %
         \pgf@xa=0pt %
      \else%
         \pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/inner xsep}+.5mm}%
      \fi%
      \ifdim\dimexpr.5\wd\pgfnodeparttextbox+\pgf@xa\relax>\pgf@x%
         \pgf@x=\dimexpr.5\wd\pgfnodeparttextbox+\pgf@xa\relax%
      \fi%
   }%
   \saveddimen\yradius{%
      \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/tikz/y radius}}%
      \ifdim\dimexpr\ht\pgfnodeparttextbox+\dp\pgfnodeparttextbox\relax=0pt %
         \pgf@xa=0pt %
      \else%
         \pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/inner ysep}}%
      \fi%
      \@tempdima=\dimexpr.5\ht\pgfnodeparttextbox+.5\dp\pgfnodeparttextbox+\pgf@xa\relax%
      \ifdim\@tempdima>\pgf@x%
         \pgf@x=\@tempdima%
      \fi%
   }%
   \savedanchor\stext{%
      \pgfqpoint%
         {-\dimexpr.5\wd\pgfnodeparttextbox+1mm\relax}%
         {-\dimexpr.5\ht\pgfnodeparttextbox-.5\dp\pgfnodeparttextbox\relax}%
   }%
   \foreach \anc in {center, north, south, south west, west, north west, text} {%
      \inheritanchor[from=yquant-rectangle]{\anc}%
   }%
   \foreach \anc in {north east, east, south east} {%
      \inheritanchor[from=yquant-circle]{\anc}%
   }%
   \anchorborder{%
      \@tempdima=\pgf@x%
      \@tempdimb=\pgf@y%
      \ifdim\pgf@x>\dimexpr\xradius-3mm\relax%
         \pgfpointborderellipse{\pgfqpoint{\dimexpr\@tempdima-\xradius+3mm\relax}%
                                          {\@tempdimb}}%
                               {\pgfqpoint{3mm}%
                                          {.707107\dimexpr\yradius\relax}}%
         \advance\pgf@x by \dimexpr\xradius-3mm\relax%
      \else%
         \pgfpointborderrectangle{\pgfqpoint{\@tempdima}{\@tempdimb}}%
                                 {\pgfqpoint{\xradius}{\yradius}}%
      \fi%
   }%
   \backgroundpath{%
      \pgfpathmoveto{\pgfqpoint{-\xradius}{\yradius}}%
      \pgfpathlineto{\pgfqpoint{\dimexpr\xradius-3mm\relax}{\yradius}}%
      \pgfpatharc{90}{-90}{3mm and \yradius}%
      \pgfpathlineto{\pgfqpoint{-\xradius}{-\yradius}}%
      \pgfpathclose%
   }%
   \clippath{%
      \pgfpathmoveto{\pgfqpoint{-\dimexpr\xradius+.5\pgflinewidth\relax}%
                               {\dimexpr\yradius+.5\pgflinewidth\relax}}%
      \pgfpathlineto{\pgfqpoint{\dimexpr\xradius-3mm\relax}%
                               {\dimexpr\yradius+.5\pgflinewidth\relax}}%
      \pgfpatharc{90}{-90}{3mm+.5\pgflinewidth and \yradius+.5\pgflinewidth}%
      \pgfpathlineto{\pgfqpoint{-\dimexpr\xradius+.5\pgflinewidth\relax}%
                               {-\dimexpr\yradius+.5\pgflinewidth\relax}}%
      \pgfpathclose%
   }%
}

\pgfdeclareshape{yquant-line}{%
   \saveddimen\xradius{%
      % we only need this for the border anchor; the value is automatically correct in the paths.
      \pgf@x=.5\pgflinewidth%
   }%
   \saveddimen\yradius{%
      \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/tikz/y radius}+.5*\yquant@config@register@sep}%
   }%
   \foreach \anc in {center, north, north east, east, south east, south, south west, west, north west} {%
      \inheritanchor[from=yquant-rectangle]{\anc}%
   }%
   \inheritanchorborder[from=yquant-rectangle]%
   \backgroundpath{%
      % manually shorten for the bounding box
      \pgf@xa=\dimexpr\yradius-\pgf@shorten@end@additional\relax%
      \pgf@ya=\dimexpr\yradius-\pgf@shorten@start@additional\relax%
      \pgf@shorten@end@additional=0pt %
      \pgf@shorten@start@additional=0pt %
      \pgfpathmoveto{\pgfqpoint{0pt}{\pgf@xa}}%
      \pgfpathlineto{\pgfqpoint{0pt}{-\pgf@ya}}%
   }%
   \clippath{%
      \@tempdima=\dimexpr\yradius-\pgf@shorten@end@additional\relax%
      \@tempdimb=\dimexpr\yradius-\pgf@shorten@start@additional\relax%
      \pgfpathrectanglecorners%
         {\pgfqpoint{-.5\pgflinewidth}{\@tempdima}}%
         {\pgfqpoint{.5\pgflinewidth}{-\@tempdimb}}%
   }%
}

% BEGIN_FOLD Gapped brace decoration
\def\pgfdecorationsegmentfromto{0-1}%

\protected\def\yquant@gappedbrace@extract#1-#2\yquant@sep{%
   \dimdef\from{#1\pgfdecoratedremainingdistance}%
   \dimdef\to{#2\pgfdecoratedremainingdistance}%
}

\def\yquant@gappedbrace@shiftloop#1{%
   \yquant@gappedbrace@extract#1\yquant@sep%
   \unless\ifdim\pgfdecorationsegmentaspect\pgfdecoratedremainingdistance<\from %
      \unless\ifdim\pgfdecorationsegmentaspect\pgfdecoratedremainingdistance>\to %
         % be careful about arch positions at the border
         \ifdim\dimexpr\to-\from\relax<2\pgfdecorationsegmentamplitude %
            % The arch is larger than the segment. We do not draw a line to it or an end line and place it in the mid of the segment, even if it is too short (this issues one extra \pgfpathmoveto command, but catching this rare case is not worth the effort).
            \edef\pgfdecorationsegmentaspect{\pgfmath@tonumber{\dimexpr%
               .5\dimexpr\from+\to\relax*65536/\pgfdecoratedremainingdistance%
            \relax}}%
         \else%
            % The segment is large enough to cover the whole arch. But maybe we are too close at the border?
            \ifdim\dimexpr\pgf@xc-\pgfdecorationsegmentamplitude\relax<\from %
               \pgf@xc=\dimexpr\from+\pgfdecorationsegmentamplitude\relax%
            \fi%
            \ifdim\dimexpr\pgf@xc+\pgfdecorationsegmentamplitude\relax>\to %
               \pgf@xc=\dimexpr\to-\pgfdecorationsegmentamplitude\relax%
            \fi%
            \edef\pgfdecorationsegmentaspect{\pgfmath@tonumber{\dimexpr%
               \dimexpr\pgf@xc*65536/\pgfdecoratedremainingdistance%
            \relax}}%
         \fi%
         \expandafter\expandafter\expandafter\listbreak%
      \fi%
   \fi%
}

% Assumes all decoration macros and lengths are filled. Checks whether the arch is too close at a corner and shifts it appropriately. Upon exit, \pgfdecorationsegmentaspect is modified.
\protected\def\yquant@gappedbrace@calcshift{%
   \pgf@xc=\pgfdecorationsegmentaspect\pgfdecoratedremainingdistance%
   \expandafter\forcsvlist\expandafter\yquant@gappedbrace@shiftloop%
      \expandafter{\pgfdecorationsegmentfromto}%
}

\def\yquant@gappedbrace@loop#1{%
   \yquant@gappedbrace@extract#1\yquant@sep%
   \unless\ifdim\from=0pt %
      \pgfpathmoveto{%
         \pgfqpoint{\from}{.5\pgfdecorationsegmentamplitude}%
      }%
   \fi%
   \unless\ifdim\pgfdecorationsegmentaspect\pgfdecoratedremainingdistance<\from %
      \unless\ifdim\pgfdecorationsegmentaspect\pgfdecoratedremainingdistance>\to %
         % be careful about arch positions at the border
         \ifdim\dimexpr\to-\from\relax<2\pgfdecorationsegmentamplitude %
            % The arch is larger than the segment. We do not draw a line to it or an end line and place it in the mid of the segment, even if it is too short (this issues one extra \pgfpathmoveto command, but catching this rare case is not worth the effort).
            \pgfpathmoveto{%
               \pgfqpoint{\dimexpr.5\dimexpr\from+\to\relax-\pgfdecorationsegmentamplitude\relax}%
                         {.5\pgfdecorationsegmentamplitude}%
            }%
            \edef\to{\the\pgfdecoratedremainingdistance}% to prevent the final line, we do not need "to" any more
         \else%
            % The segment is large enough to cover the whole arch. But maybe we are too close at the border?
            \ifdim\dimexpr\pgf@xc-\pgfdecorationsegmentamplitude\relax<\from %
               \pgf@xc=\dimexpr\from+\pgfdecorationsegmentamplitude\relax%
            \fi%
            \ifdim\dimexpr\pgf@xc+\pgfdecorationsegmentamplitude\relax>\to %
               \pgf@xc=\dimexpr\to-\pgfdecorationsegmentamplitude\relax%
            \fi%
            % Both cases can't occur at the same time in this \else clause.
            \pgfpathlineto{%
               \pgfqpoint{\dimexpr\pgf@xc-\pgfdecorationsegmentamplitude\relax}%
                         {.5\pgfdecorationsegmentamplitude}%
            }%
         \fi%
         \pgfpathcurveto{%
            \pgfqpoint{\dimexpr\pgf@xc-.5\pgfdecorationsegmentamplitude\relax}%
                      {.5\pgfdecorationsegmentamplitude}%
         }{%
            \pgfqpoint{\dimexpr\pgf@xc-.15\pgfdecorationsegmentamplitude\relax}%
                      {.7\pgfdecorationsegmentamplitude}%
         }{%
            \pgfqpoint{\pgf@xc}{\pgfdecorationsegmentamplitude}%
         }%
         \pgfpathcurveto{%
            \pgfqpoint{\dimexpr\pgf@xc+.15\pgfdecorationsegmentamplitude\relax}%
                      {.7\pgfdecorationsegmentamplitude}%
         }{%
            \pgfqpoint{\dimexpr\pgf@xc+.5\pgfdecorationsegmentamplitude\relax}%
                      {.5\pgfdecorationsegmentamplitude}%
         }{%
            \pgfqpoint{\dimexpr\pgf@xc+\pgfdecorationsegmentamplitude\relax}%
                      {.5\pgfdecorationsegmentamplitude}%
         }%
      \fi%
   \fi%
   \unless\ifdim\to=\pgfdecoratedremainingdistance %
      \pgfpathlineto{%
         \pgfqpoint{\to}{.5\pgfdecorationsegmentamplitude}%
      }%
   \fi%
}

% This is a variant of the brace in pathreplacing that allows for holes
\pgfdeclaredecoration{gapped brace}{final}{%
   \state{final}{%
      \pgf@xc=\pgfdecorationsegmentaspect\pgfdecoratedremainingdistance%
      \pgfpathmoveto\pgfpointorigin% required for "raise" key
      \pgfpathcurveto{%
         \pgfqpoint{.15\pgfdecorationsegmentamplitude}{.3\pgfdecorationsegmentamplitude}%
      }{%
         \pgfqpoint{.5\pgfdecorationsegmentamplitude}{.5\pgfdecorationsegmentamplitude}%
      }{%
         \pgfqpoint{\pgfdecorationsegmentamplitude}{.5\pgfdecorationsegmentamplitude}%
      }%
      \expandafter\forcsvlist\expandafter\yquant@gappedbrace@loop%
         \expandafter{\pgfdecorationsegmentfromto}%
      \pgfpathlineto{%
         \pgfqpoint{\dimexpr\pgfdecoratedremainingdistance-\pgfdecorationsegmentamplitude\relax}%
                   {.5\pgfdecorationsegmentamplitude}%
      }%
      \pgfpathcurveto{%
         \pgfqpoint{\dimexpr\pgfdecoratedremainingdistance-.5\pgfdecorationsegmentamplitude\relax}%
                   {.5\pgfdecorationsegmentamplitude}%
      }{%
         \pgfqpoint{\dimexpr\pgfdecoratedremainingdistance-.15\pgfdecorationsegmentamplitude\relax}%
                   {.3\pgfdecorationsegmentamplitude}%
      }{%
         \pgfqpoint{\pgfdecoratedremainingdistance}{0pt}%
      }%
   }%
}%

\protected\def\yquant@gappedbrace@timer{%
   \ifdim\tikz@time pt=-1pt %
      % first set \pgfdecoratedremainingdistance appropriately
      \pgfpointdiff\tikz@timer@start\tikz@timer@end%
      \pgfmathsqrt@{\dimexpr\pgf@x*\pgf@x/65536+\pgf@y*\pgf@y/65536\relax\@gobbletwo}%
      \pgfdecoratedremainingdistance=\pgfmathresult pt %
      % now perform the transformation
      \yquant@gappedbrace@calcshift%
      % and finally let us return the desired position, just ignoring \tikz@time...
      \pgftransformlineattime{\pgfdecorationsegmentaspect}{\tikz@timer@start}{\tikz@timer@end}%
   \else%
      \pgftransformlineattime{\tikz@time}{\tikz@timer@start}{\tikz@timer@end}%
   \fi%
}

\pgfkeys{%
   /pgf/decoration/from to/.store in=\pgfdecorationsegmentfromto%
}
% END_FOLD

\pgfdeclareshape{yquant-init}{%
   \saveddimen\xradius{%
      \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/tikz/x radius}}%
      % inner xsep is between the brace tip and the right end of the text. Check if the decoration is raised (will define \def\tikz@dec@shift{\pgftransformyshift{#1}})
      \iftikz@decoratepath%
         \ifx\tikz@dec@shift\relax%
            \pgf@xa=\pgfdecorationsegmentamplitude %
         \else%
            \pgfmathsetlength\pgf@xa{\expandafter\@secondoftwo\tikz@dec@shift+\pgfdecorationsegmentamplitude}%
         \fi%
         \pgfmathaddtolength\pgf@xa{\pgfkeysvalueof{/pgf/inner xsep}}%
      \else%
         \pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/inner xsep}}%
      \fi%
      % outer xsep is (a lower bound) from the left end of the border to the left end of the text
      \pgfmathsetlength\pgf@xb{\pgfkeysvalueof{/pgf/outer xsep}}%
      \@tempdima=.5\dimexpr\wd\pgfnodeparttextbox+\pgf@xa+\pgf@xb\relax%
      \ifdim\@tempdima>\pgf@x%
         \pgf@x=\@tempdima%
      \fi%
   }%
   \saveddimen\yradius{%
      \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/tikz/y radius}}%
      \@tempdima=.5\dimexpr\ht\pgfnodeparttextbox+\dp\pgfnodeparttextbox\relax%
      \ifdim\@tempdima>\pgf@x%
         \pgf@x=\@tempdima%
      \fi%
      \iftikz@decoratepath%
         \ifdim2\pgfdecorationsegmentamplitude>\pgf@x%
            \pgf@x=2\pgfdecorationsegmentamplitude%
         \fi%
      \fi%
   }%
   \savedanchor\stext{%
      \iftikz@decoratepath%
         % \pgf@x is still \yradius...
         % first set \pgfdecoratedremainingdistance appropriately
         \pgfdecoratedremainingdistance=2\pgf@x%
         % now perform the transformation
         \yquant@gappedbrace@calcshift%
         \pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/inner xsep}+\pgfdecorationsegmentamplitude}%
         \unless\ifx\tikz@dec@shift\relax%
            \pgfmathaddtolength\pgf@xa{\expandafter\@secondoftwo\tikz@dec@shift}%
         \fi%
         \pgfqpoint%
            {-\dimexpr\wd\pgfnodeparttextbox+\pgf@xa\relax}%
            {\dimexpr.5\pgfdecoratedremainingdistance% = \yradius
                     -\pgfdecorationsegmentaspect\pgfdecoratedremainingdistance% - aspect
                     -.5\ht\pgfnodeparttextbox+.5\dp\pgfnodeparttextbox% center there
             \relax}%
       \else%
         \pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/inner xsep}}%
         \pgfqpoint%
            {-\dimexpr\wd\pgfnodeparttextbox+\pgf@xa\relax}%
            {-.5\dimexpr\ht\pgfnodeparttextbox-\dp\pgfnodeparttextbox\relax}%
       \fi%
   }%
   % BEGIN_FOLD Operator anchors
   \foreach \anc in {center, north, north east, east, south east, south, south west, west, north west} {%
      \inheritanchor[from=yquant-rectangle]{\anc}%
   }%
   \anchor{text}{%
      \stext%
      \advance \pgf@x by \xradius\relax%
   }%
   \inheritanchorborder[from=yquant-rectangle]%
   % END_FOLD
   % BEGIN_FOLD Path
   \backgroundpath{%
      \pgfpathmoveto{\pgfqpoint{\xradius}{\yradius}}%
      \pgfpathlineto{\pgfqpoint{\xradius}{-\yradius}}%
      \pgfpointtransformed{\pgfqpoint{-\xradius}{\yradius}}%
      \pgf@protocolsizes{\pgf@x}{\pgf@y}%
      \pgfpointtransformed{\pgfqpoint{-\xradius}{-\yradius}}% for rotations
      \pgf@protocolsizes{\pgf@x}{\pgf@y}%
   }%
   \clippath{%
      \pgfpathrectanglecorners%
         {\pgfqpoint{-\dimexpr\xradius\relax}%
                    {\dimexpr\yradius\relax}}%
         {\pgfqpoint{\dimexpr\xradius+.5\pgflinewidth\relax}%
                    {-\dimexpr\yradius\relax}}%
   }%
   % END_FOLD
}

\pgfdeclareshape{yquant-output}{%
   % Almost the same as in yquant-input, only a minimal change in \stext's x position
   \saveddimen\xradius{%
      \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/tikz/x radius}}%
      % inner xsep is from the brace tip and the left end of the text. Check if the decoration is raised (will define \def\tikz@dec@shift{\pgftransformyshift{#1}})
      \iftikz@decoratepath%
         \ifx\tikz@dec@shift\relax%
            \pgf@xa=\pgfdecorationsegmentamplitude %
         \else%
            \pgfmathsetlength\pgf@xa{\expandafter\@secondoftwo\tikz@dec@shift+\pgfdecorationsegmentamplitude}%
         \fi%
         \pgfmathaddtolength\pgf@xa{\pgfkeysvalueof{/pgf/inner xsep}}%
      \else%
         \pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/inner xsep}}%
      \fi%
      % outer xsep is (a lower bound) from the left end of the border to the left end of the text
      \pgfmathsetlength\pgf@xb{\pgfkeysvalueof{/pgf/outer xsep}}%
      \@tempdima=.5\dimexpr\wd\pgfnodeparttextbox+\pgf@xa+\pgf@xb\relax%
      \ifdim\@tempdima>\pgf@x%
         \pgf@x=\@tempdima%
      \fi%
   }%
   \saveddimen\yradius{%
      \pgfmathsetlength\pgf@x{\pgfkeysvalueof{/tikz/y radius}}%
      \@tempdima=.5\dimexpr\ht\pgfnodeparttextbox+\dp\pgfnodeparttextbox\relax%
      \ifdim\@tempdima>\pgf@x%
         \pgf@x=\@tempdima%
      \fi%
      \iftikz@decoratepath%
         \ifdim2\pgfdecorationsegmentamplitude>\pgf@x%
            \pgf@x=2\pgfdecorationsegmentamplitude%
         \fi%
      \fi%
   }%
   \savedanchor\stext{%
      \iftikz@decoratepath%
         % \pgf@x is still \yradius...
         % first set \pgfdecoratedremainingdistance appropriately
         \pgfdecoratedremainingdistance=2\pgf@x%
         % now perform the transformation
         \yquant@gappedbrace@calcshift%
         \pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/inner xsep}+\pgfdecorationsegmentamplitude}%
         \unless\ifx\tikz@dec@shift\relax%
            \pgfmathaddtolength\pgf@xa{\expandafter\@secondoftwo\tikz@dec@shift}%
         \fi%
         \pgfqpoint%
            {\dimexpr\pgf@xa\relax}%
            {\dimexpr.5\pgfdecoratedremainingdistance% = \yradius
                     -\pgfdecorationsegmentaspect\pgfdecoratedremainingdistance% - aspect
                     -.5\ht\pgfnodeparttextbox+.5\dp\pgfnodeparttextbox% center there
             \relax}%
       \else%
         \pgfmathsetlength\pgf@xa{\pgfkeysvalueof{/pgf/inner xsep}}%
         \pgfqpoint%
            {\dimexpr\pgf@xa\relax}%
            {-.5\dimexpr\ht\pgfnodeparttextbox-\dp\pgfnodeparttextbox\relax}%
       \fi%
   }%
   % BEGIN_FOLD Operator anchors
   \foreach \anc in {center, north, north east, east, south east, south, south west, west, north west} {%
      \inheritanchor[from=yquant-init]{\anc}%
   }%
   \anchor{text}{%
      \stext%
      \advance \pgf@x by -\xradius\relax%
   }%
   \inheritanchorborder[from=yquant-init]%
   % END_FOLD
   % BEGIN_FOLD Path
   \backgroundpath{%
      \pgfpathmoveto{\pgfqpoint{-\xradius}{\yradius}}%
      \pgfpathlineto{\pgfqpoint{-\xradius}{-\yradius}}%
      \pgfpointtransformed{\pgfqpoint{\xradius}{\yradius}}%
      \pgf@protocolsizes{\pgf@x}{\pgf@y}%
      \pgfpointtransformed{\pgfqpoint{\xradius}{-\yradius}}% for rotations
      \pgf@protocolsizes{\pgf@x}{\pgf@y}%
   }%
   \clippath{%
      \pgfpathrectanglecorners%
         {\pgfqpoint{-\dimexpr\xradius+.5\pgflinewidth\relax}%
                    {\dimexpr\yradius\relax}}%
         {\pgfqpoint{\dimexpr\xradius\relax}%
                    {-\dimexpr\yradius\relax}}%
   }%
   % END_FOLD
}

==> yquant-tools.tex <==
% from TeXbook, appendix D
\protected\def\yquant@futurenonspacelet#1{%
   \def\yquant@futurenonspacelet@cs{#1}%
   \afterassignment\yquant@futurenonspacelet@i\let\yquant@futurenonspacelet@next= %
}

\def\yquant@futurenonspacelet@i{%
   \expandafter\futurelet\yquant@futurenonspacelet@cs\yquant@futurenonspacelet@ii%
}

\def\yquant@futurenonspacelet@ii{%
   \expandafter\ifx\yquant@futurenonspacelet@cs\@sptoken%
      \expandafter\yquant@futurenonspacelet@iii%
   \else%
      \expandafter\yquant@futurenonspacelet@next%
   \fi%
}

\def\yquant@futurenonspacelet@iii{%
   \afterassignment\yquant@futurenonspacelet@i%
   \let\@eattoken= %
}

% a bit faster than nested \@firstoftwo/\@secondoftwo
% note \@thirdofthree is defined in the latex kernel already.
\long\def\@firstofthree#1#2#3{#1}%
\long\def\@secondofthree#1#2#3{#2}%
\long\def\@firstoffour#1#2#3#4{#1}%
\long\def\@secondoffour#1#2#3#4{#2}%
\long\def\@thirdoffour#1#2#3#4{#3}%
\long\def\@fourthoffour#1#2#3#4{#4}%
\long\def\@thirdandfourthoffour#1#2#3#4{#3#4}%
\long\def\@secondandthirdoffive#1#2#3#4#5{{#2}{#3}}
\long\def\@firstoffive#1#2#3#4#5{#1} % unused
\long\def\@secondoffive#1#2#3#4#5{#2}
\long\def\@thirdoffive#1#2#3#4#5{#3}
\long\def\@fourthoffive#1#2#3#4#5{#4} % unused
\long\def\@fifthoffive#1#2#3#4#5{#5}

% Loop #1 from min(#2, #3) to max(#2, #3), executing #4
\protected\def\yquant@for #1:=#2to#3#{%
   \yquant@for@aux#1{#2}{#3}%
}

% Loop #1 from max(#2, #3) down to min(#2, #3), executing #4
\protected\def\yquant@fordown #1:=#2downto#3#{%
   \yquant@fordown@aux#1{#2}{#3}%
}

\long\def\yquant@for@aux#1#2#3#4{%
   \ifnum#2<#3\relax%
      \numdef#1{#2}%
      % to allow for things like \yquant@for \i := \i to ..., expand the boundaries
      \expandafter\yquant@for@loop\expandafter#1\expandafter{\the\numexpr#3+1\relax}{#4}%
   \else%
      \numdef#1{#3}%
      \expandafter\yquant@for@loop\expandafter#1\expandafter{\the\numexpr#2+1\relax}{#4}%
   \fi%
}

\long\def\yquant@fordown@aux#1#2#3#4{%
   \ifnum#2>#3\relax%
      \numdef#1{#2}%
      % to allow for things like \yquant@for \i := \i to ..., expand the boundaries
      \expandafter\yquant@fordown@loop\expandafter#1\expandafter{\the\numexpr#3-1\relax}{#4}%
   \else%
      \numdef#1{#3}%
      \expandafter\yquant@fordown@loop\expandafter#1\expandafter{\the\numexpr#2-1\relax}{#4}%
   \fi%
}

\long\def\yquant@for@loop#1#2#3{%
   \loop%
      \ifnum#1<#2\relax%
         #3%
         \numdef#1{#1+1}%
   \repeat%
}

\long\def\yquant@fordown@loop#1#2#3{%
   \loop%
      \ifnum#1>#2\relax%
         #3%
         \numdef#1{#1-1}%
   \repeat%
}

\def\yquant@for@break{%
   \fi%
   \iffalse%
}

% Def #1 to be the minimum of #2, ... until \relax
\protected\def\yquant@min#1{%
   \def#1{2147483647}%
   \def\yquant@min@var{#1}%
   \yquant@min@loop%
}

\def\yquant@min@loop#1{%
   \unless\ifx#1\relax\relax%
      \ifnum#1<\yquant@min@var\relax%
         \expandafter\edef\yquant@min@var{#1}%
      \fi%
      \expandafter\yquant@min@loop%
   \fi%
}

% Def #1 to be the maximum of #2, ... until \relax
\protected\def\yquant@max#1{%
   \def#1{-2147483647}%
   \def\yquant@max@var{#1}%
   \yquant@max@loop%
}

\def\yquant@max@loop#1{%
   \unless\ifx#1\relax\relax%
      \ifnum#1>\yquant@max@var\relax%
         \expandafter\edef\yquant@max@var{#1}%
      \fi%
      \expandafter\yquant@max@loop%
   \fi%
}

% Cleanup global tokens after environment
\protected\def\yquant@cleanup@csadd#1{%
   \csxappto{\yquant@prefix cleanup}{\expandafter\noexpand\csname#1\endcsname}%
}

\def\yquant@cleanup#1#2{%
   \global\undef#1%
   \unless\ifx|#2%
      \expandafter\yquant@cleanup\expandafter#2%
   \fi%
}

% Executes #3 if #1 (single token!) is equal (\ifx) to the first token of #2, and #4 else.
\def\ifyquant@firsttoken#1#2{%
   % First check whether #2 is present at all...
   \ifstrempty{#2}{%
      \expandafter\@secondoftwo%
   }{%
      \ifyquant@firsttoken@aux#1#2\yquant@sep%
   }%
}

\def\ifyquant@firsttoken@aux#1#2#3\yquant@sep{%
   \ifx#1#2%
      \expandafter\expandafter\expandafter\@firstoftwo%
   \else%
      \expandafter\expandafter\expandafter\@secondoftwo%
   \fi%
}

% Executes #3 if #1 begins with #2, and #4 else - non-expandable
\protected\def\ifyquant@beginswith#1#2{%
   \def\ifyquant@beginswith@##1#2##2\yquant@end{%
      \ifstrempty{##1}%
   }%
   \ifyquant@beginswith@#1#2\yquant@end%
}

% absolute value of a dimension
\def\yquant@abs#1{%
   \ifdim#1<0pt %
      \the\dimexpr-\dimexpr#1\relax\relax%
   \else%
      #1%
   \fi%
}

% Sortlist related macros.
\newcount\yquant@sort@count

\protected\def\yquant@sort@clear{%
   % Probably cleanup used macros?
   \yquant@sort@count=0 %
}

\protected\def\yquant@sort@eadd#1{%
   \csedef{yquant@sort@item\the\yquant@sort@count}{#1}%
   \advance \yquant@sort@count by 1 %
}

% Perform quicksort on the stored sortlist.
% #1: compare macro that expands to ##3 if its second argument is strictly larger than its first or to ##4 else
\protected\def\yquant@sort#1{%
   \let\yquant@sort@cmp=#1%
   \expandafter\yquant@sort@aux\expandafter0\expandafter{\the\numexpr\yquant@sort@count-1\relax}%
}

% Returns the first item in the unordered sortlist when compared according to #1 and stores it in #2.
\protected\def\yquant@sort@findfirst#1#2{%
   \ifnum\yquant@sort@count<1 %
      \let#2=\empty%
   \else%
      \letcs#2{yquant@sort@item0}%
      \count0=1 %
      \loop%
         \ifnum\count0<\yquant@sort@count\relax%
            \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter#1%
               \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
               \expandafter\expandafter\expandafter#2%
               \expandafter\expandafter\expandafter}%
               \expandafter\expandafter\expandafter{%
                  \csname yquant@sort@item\the\count0\endcsname%
               }%
               \relax{%
               \letcs#2{yquant@sort@item\the\count0}%
            }%
            \advance\count0 by 1 %
      \repeat%
   \fi%
}

\def\yquant@sort@ascending#1#2{%
   \ifnum#2>#1 %
      \expandafter\@firstoftwo%
   \else%
      \expandafter\@secondoftwo%
   \fi%
}

\protected\def\yquant@sort@aux#1#2{%
   \ifnum#1<#2\relax%
      \yquant@sort@divide{#1}{#2}%
      \edef\cmd{%
         \noexpand\yquant@sort@aux{#1}{\the\numexpr\count0-1\relax}%
         \noexpand\yquant@sort@aux{\the\numexpr\count0+1\relax}{#2}%
      }%
      \cmd%
   \fi%
}

\def\iftrue@hidden{\iftrue}%
\def\iffalse@hidden{\iffalse}%
\protected\def\yquant@sort@divide#1#2{%
   \count0=#1\relax% i
   \count2=#2\relax% j
   \advance\count2 by -1 %
   \letcs\yquant@sort@pivot{yquant@sort@item#2}%
   \loop%
      % search an item from the left that is larger or equal to the pivot
      {% protect the outer loop from finding \repeat
         \loop%
            \ifnum\count0<#2\relax%
               \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\yquant@sort@cmp%
                  \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
                  \expandafter\expandafter\expandafter\yquant@sort@pivot%
                  \expandafter\expandafter\expandafter}%
                  \expandafter\expandafter\expandafter{%
                     \csname yquant@sort@item\the\count0\endcsname%
                  }{%
                     \expandafter\iffalse@hidden%
                  }{%
                     \advance\count0 by 1 %
                     \expandafter\iftrue@hidden%
                  }%
            \else%
               \expandafter\iffalse@hidden%
            \fi%
         \repeat%
         \expandafter%
      }%
      \expandafter\count\expandafter0\expandafter=\the\count0\relax%
      % search an item from the right that is small than the pivot
      {% protect the outer loop from finding \repeat
         \loop%
            \ifnum\count2>#1\relax%
               \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\yquant@sort@cmp%
                  \expandafter\expandafter\expandafter\expandafter\expandafter\expandafter\expandafter{%
                  \expandafter\expandafter\expandafter\yquant@sort@pivot%
                  \expandafter\expandafter\expandafter}%
                  \expandafter\expandafter\expandafter{%
                     \csname yquant@sort@item\the\count2\endcsname%
                  }{%
                     \advance\count2 by -1 %
                     \expandafter\iftrue@hidden%
                  }{%
                     \expandafter\iffalse@hidden%
                  }%
            \else%
               \expandafter\iffalse@hidden%
            \fi%
         \repeat%
         \expandafter%
      }%
      \expandafter\count\expandafter2\expandafter=\the\count2\relax%
      \ifnum\count0<\count2 %
         % swap item i <> item j
         \letcs\tmp{yquant@sort@item\the\count0}%
         \csletcs{yquant@sort@item\the\count0}{yquant@sort@item\the\count2}%
         \cslet{yquant@sort@item\the\count2}\tmp%
      \fi%
      \ifnum\count0<\count2 %
   \repeat%
   \letcs\tmp{yquant@sort@item\the\count0}%
   \csletcs{yquant@sort@item\the\count0}{yquant@sort@item#2}%
   \cslet{yquant@sort@item#2}\tmp%
}

% Add an internal etoolbox list to the sorted items
\def\yquant@sort@addlist#1{%
   \forlistloop\yquant@sort@addlist@aux#1%
}

\protected\def\yquant@sort@addlist@aux#1{%
   \csdef{yquant@sort@item\the\yquant@sort@count}{#1}%
   \advance\yquant@sort@count by 1 %
}

% Sorts an internal etoolbox list #1 using macro #2
\protected\def\yquant@sort@list#1#2{%
   \begingroup%
      \yquant@sort@count=0 %
      \yquant@sort@addlist#1%
      \yquant@sort#2%
      \let#1=\empty%
      \count0=0 %
      \loop%
         \ifnum\count0<\yquant@sort@count%
            \expandafter\expandafter\expandafter\listadd%
            \expandafter\expandafter\expandafter#1%
            \expandafter\expandafter\expandafter{%
               \csname yquant@sort@item\the\count0\endcsname%
            }%
            \advance\count0 by 1 %
      \repeat%
      \expandafter%
   \endgroup%
   \expandafter\def\expandafter#1\expandafter{#1}%
}

\protected\def\yquant@sort@dolistloop{%
   \count0=0 %
   \loop%
      \ifnum\count0<\yquant@sort@count%
         \expandafter\expandafter\expandafter\do%
         \expandafter\expandafter\expandafter{%
            \csname yquant@sort@item\the\count0\endcsname%
         }%
         \advance\count0 by 1 %
   \repeat%
}

\begingroup
\catcode`\|=3
\catcode`\&=3
\gdef\yquant@list@delim{|}

\protected\gdef\yquant@list@dequeue#1#2{%
   \expandafter\ifblank\expandafter{#1}{%
      \let#2=\empty%
   }{%
      \expandafter\yquant@list@dequeue@i#1\etb@lst@q@end{#1}{#2}\def%
   }%
}%

\protected\gdef\yquant@list@dequeue@i#1|#2\etb@lst@q@end#3#4#5{%
   \def#4{#1}%
   #5#3{#2}%
}

\protected\gdef\yquant@list@gdequeue#1#2{%
   \expandafter\ifblank\expandafter{#1}{%
      \let#2=\empty%
   }{%
      \expandafter\yquant@list@dequeue@i#1\etb@lst@q@end{#1}{#2}\gdef%
   }%
}

\protected\gdef\yquant@list@eupdateorinsert#1#2#3{%
   % the list items are of the form <number>:<value>. If an item is present where <number> = #2, then set its <value> to #3, if #3 is greater. If no item is present, add it.
   \begingroup%
      \def\etb@tempa##1|#2:##2|##3&{%
         \endgroup%
         \ifstrempty{##3}{%
            \eappto#1{#2:#3|}%
         }{%
            \ifdim##2<#3 %
               \yquant@list@ereplace#1{#2:##2}{#2:#3}%
            \fi%
         }%
      }%
   \expandafter\etb@tempa\expandafter|#1|#2:#3|&%
}

\protected\gdef\yquant@list@ereplace#1#2#3{%
   \begingroup%
      \def\etb@tempa##1|#2|##2&{%
         \endgroup%
         \ifstrempty{##1}{%
            \edef#1{%
               \unexpanded{##1}|#3|\unexpanded{##2}%
            }%
         }{%
            \edef#1{%
               \unexpanded\expandafter{\@gobble##1}|#3|\unexpanded{##2}%
            }%
         }%
      }%
   \expandafter\etb@tempa\expandafter|#1&
}

% expands to the contents of a list ranging from #1 to #2 (ascending)
\gdef\yquant@list@range#1#2{%
   \ifnum#1>#2 %
      \expandafter\@firstoftwo%
   \else%
      \expandafter\@secondoftwo%
   \fi{}{%
      #1|%
      \expandafter\yquant@list@range\expandafter{\the\numexpr#1+1\relax}{#2}%
   }%
}
\endgroup

% performs #3 if #1 is a subset of #2; else, performs #4
\protected\def\ifyquant@registersubset#1#2{%
   \begingroup%
      \let\yquant@register@multi=\@fourthoffour
      \def\yquant@register@multi@contiguous##1##2##3{\yquant@list@range{##1}{##2}}%
      \edef\listA{#1}%
      \edef\listB{#2}%
      \let\ifsuccess=\iftrue%
      \forlistloop\yquant@registersubset@loop\listA%
      \expandafter%
   \endgroup%
   \ifsuccess%
      \expandafter\@firstoftwo%
   \else%
      \expandafter\@secondoftwo%
   \fi%
}

\protected\def\yquant@registersubset@loop#1{%
   \ifinlist{#1}\listB\relax{%
      \let\ifsuccess=\iffalse%
      \listbreak%
   }%
}

\def\ifyquant@OR#1#2{%
   #1%
      \expandafter\@firstoftwo%
   \else%
      #2%
         \expandafter\expandafter\expandafter\@firstoftwo%
      \else%
         \expandafter\expandafter\expandafter\@secondoftwo%
      \fi%
   \fi%
}

% #1 is a pgf soft path. We extract the maximum x position at the y position specified in #2 and assign it to \dimen0, which is translated to the user coordinate system.
\protected\def\yquant@softpath@extractmaxxat#1#2{%
   \begingroup%
      \dimen0=-16000pt %
      \dimen2=#2 %
      \pgftransforminvert%
      \let\pgfsyssoftpath@movetotoken=\yquant@softpath@extractmaxxat@moveto%
      \let\pgfsyssoftpath@linetotoken=\yquant@softpath@extractmaxxat@lineto%
      \let\pgfsyssoftpath@curvetosupportatoken=\yquant@softpath@extractmaxxat@curveto%
      \let\pgfsyssoftpath@rectcornertoken=\yquant@softpath@extractmaxxat@rectto%
      \let\pgfsyssoftpath@closepath=\@gobbletwo%
      % the specialroundtoken (undocumented) is \@gobbletwo by default.
      #1%
      \expandafter%
   \endgroup%
   \expandafter\dimen\expandafter0\expandafter=\the\dimen0  %
}

\protected\def\yquant@softpath@extractmaxxat@update#1{%
   \ifdim\dimen0<#1 %
      \dimen0=#1 %
   \fi%
}

\protected\def\yquant@softpath@extractmaxxat@moveto#1#2{%
   \pgfpointtransformed{\pgfqpoint{#1}{#2}}%
   \dimen4=\pgf@x %
   \dimen6=\pgf@y %
}

\protected\def\yquant@softpath@extractmaxxat@lineto#1#2{%
   \pgfpointtransformed{\pgfqpoint{#1}{#2}}%
   \ifyquant@OR{\ifdim\dimen4>\dimen0 }{\ifdim\pgf@x>\dimen0 }{%
      \ifdim\dimen6=\dimen2 %
         \yquant@softpath@extractmaxxat@update{\dimen4}%
      \else%
         \ifdim\dimen6<\dimen2 %
            \unless\ifdim\pgf@y<\dimen2 %
               \expandafter\yquant@softpath@extractmaxxat@update\expandafter{\the\dimexpr%
                  \dimen4+% x0
                  \dimexpr\pgf@x-\dimen4\relax*% (x1-x0)
                  \dimexpr\dimen2-\dimen6\relax/\dimexpr\pgf@y-\dimen6\relax% (y-y0)/(y1-y0)
               \relax}%
            \fi%
         \else%
            \unless\ifdim\pgf@y>\dimen2 %
               \expandafter\yquant@softpath@extractmaxxat@update\expandafter{\the\dimexpr%
                  \dimen4+% x0
                  \dimexpr\pgf@x-\dimen4\relax*% (x1-x0)
                  \dimexpr\dimen2-\dimen6\relax/\dimexpr\pgf@y-\dimen6\relax% (y-y0)/(y1-y0)
               \relax}%
            \fi%
         \fi%
      \fi%
   }\relax%
   \dimen4=\pgf@x%
   \dimen6=\pgf@y%
}

\protected\def\yquant@softpath@extractmaxxat@curveto@checkx{%
   % \dimen11 holds our only candidate for t. Is it within the curve?
   \unless\ifdim\dimen11<0pt %
      \unless\ifdim\dimen11>1pt %
         % it is. \dimen4: x0, \pgf@xa: xa, \pgf@xb: xb, \pgf@xc: x1
         \begingroup%
            \dimen12=\dimexpr1pt-\dimen11\relax% 1 - t
            \dimen13=\dimexpr\dimen11*\dimen11/65535\relax% t^2
            \dimen14=\dimexpr\dimen12*\dimen12/65535\relax% (1 - t)^2
            \dimen255=\dimexpr\dimen13*\dimen11/65535*\pgf@xc/65535+% t^3 x1
                              3\dimen13*\dimen12/65535*\pgf@xb/65535+% t^2(1 - t) xb
                              \dimen14*\dimen12/65535*\dimen4/65535+% (1 - t)^3 x0
                              3\dimen11*\dimen14/65535*\pgf@xa/65535% 3t(1 - t)^2 xa
                      \relax%
            \expandafter%
         \endgroup%
         \expandafter\yquant@softpath@extractmaxxat@update\expandafter{\the\dimen255}%
      \fi%
   \fi%
}

\protected\def\yquant@softpath@extractmaxxat@curveto#1#2\pgfsyssoftpath@curvetosupportbtoken#3#4\pgfsyssoftpath@curvetotoken#5#6{%
   % There's really no good way to do this apart from solving the Bézier curve (a third-order polynomial). Let's do it. (Yes, this is inefficient, but if someone substitutes the rectangular box of a subcircuit by a more fancy design, this is not our fault).
   % Parametrized by t, the x coordinates of the curve are
   % x0 + 3 (xa - x0) t + 3 (x0 - 2xa + xb) t^2 + (3xa - 3xb + x1 - x0) t^3
   % where x0 = \dimen4 (the moveto point), xa = #1, xb = #3, x1 = #5.
   % Likewise for y:
   %       y0 = \dimen6 (the moveto point), ya = #2, yb = #4, y1 = #6.
   \pgfpointtransformed{\pgfqpoint{#1}{#2}}%
   \pgf@xa=\pgf@x%
   \pgf@ya=\pgf@y%
   \pgfpointtransformed{\pgfqpoint{#3}{#4}}%
   \pgf@xb=\pgf@x%
   \pgf@yb=\pgf@y%
   \pgfpointtransformed{\pgfqpoint{#5}{#6}}%
   \pgf@xc=\pgf@x%
   \pgf@yc=\pgf@y%
   % We first solve the third-order polynomial for t using the y value, then plug it back into the x value.
   % TODO: this is accurate to approx. 3 digits. Can this be improved by reformulating Cardanos formula to involve less divisions?
   \begingroup%
      % We need so may dimensions that we break with TeX's convention for their use.
      % for the multiplications with and divisions by dimensions, we exploit that eTeX fuses muldiv to 64 bits. Further note that each dimension has a scaling factor of 65535 for sp<->pt conversion. This is why don't factor out divisions (which would be more efficient, but not give the benefit of 64bit accuracy).
      % a = 3(ya - yb) + (y1 - y0)
      \dimen1=\dimexpr3\pgf@ya-3\pgf@yb+\pgf@yc-\dimen6\relax%
      \ifdim\dimen1=0pt %
         % this is only a quadratic curve!
         % b = 3(y0 - 2ya + yb)
         \dimen3=\dimexpr3\dimexpr\dimen6-2\pgf@ya+\pgf@yb\relax*65535\relax%
         % c: 3(ya - y0)
         \dimen5=\dimexpr3\dimexpr\pgf@ya-\dimen6\relax*65535\relax%
         % d: y0 - <desired y>
         \dimen7=\dimexpr\dimexpr\dimen6-\dimen2\relax*65535\relax%
         % check the discriminant of the equation
         \dimen8=\dimexpr\dimen3*\dimen3/65535-4\dimen3*\dimen7/65535\relax%
         \unless\ifdim\dimen8<0pt%
            % there are two potential candidates, (-c +- sqrt(c^2 - 4b d))/2b
            \pgfmathsqrt@{\the\dimen8\@gobbletwo}%
            \dimen11=\dimexpr\dimexpr-\dimen5+\pgfmathresult pt\relax*65535/%
                             \dimexpr2\dimen3\relax\relax%
            \yquant@softpath@extractmaxxat@curveto@checkx%
            \dimen11=\dimexpr\dimexpr-\dimen5-\pgfmathresult pt\relax*65535/%
                             \dimexpr2\dimen3\relax\relax%
            \yquant@softpath@extractmaxxat@curveto@checkx%
         \fi%
      \else%
         % We will simplify by directly dividing all coefficients by a
         % b = 3(y0 - 2ya + yb)
         \dimen3=\dimexpr3\dimexpr\dimen6-2\pgf@ya+\pgf@yb\relax*65535/\dimen1\relax%
         % c: 3(ya - y0)
         \dimen5=\dimexpr3\dimexpr\pgf@ya-\dimen6\relax*65535/\dimen1\relax%
         % d: y0 - <desired y>
         \dimen7=\dimexpr\dimexpr\dimen6-\dimen2\relax*65535/\dimen1\relax%
         % Note that now our a value (\dimen1) is no longer needed, it is one.
         % check the discriminant of the equation
         % Q = (3c - b^2)/9
         \dimen8=\dimexpr\dimexpr3\dimen5-\dimen3*\dimen3/65535\relax/9\relax%
         % R = (9bc - 27d - 2b^3)/54 = bc/6 - d/2 - b^3/27
         \dimen9=\dimexpr\dimen3*\dimen5/393210-% 6*65535
                          .5\dimen7-%
                          \dimen3*\dimen3/65535*\dimen3/1769445% 27*65535
                  \relax%
         % D = Q^3 + R^2
         \dimen10=\dimexpr\dimen8*\dimen8/65535*\dimen8/65535+\dimen9*\dimen9/65535\relax%
         \ifdim\dimen10>0pt %
            % only one real root: y_1 = S + T - b/3a
            % S = cbrt(R + sqrt(Q^3 + R^2))
            % T = cbrt(R - sqrt(Q^3 + R^2))
            \pgfmathsqrt@{\the\dimen10\@gobbletwo}%
            \dimen12=\dimexpr\dimen9+\pgfmathresult pt\relax%
            \dimen13=\dimexpr\dimen9-\pgfmathresult pt\relax%
            \ifdim\dimen12>0pt %
               \pgfmathpow@{\the\dimen12\@gobbletwo}{.3333333333}%
               \dimen11=\pgfmathresult pt %
            \else%
               \pgfmathpow@{\the\dimexpr-\dimen12\relax\@gobbletwo}{.3333333333}%
               \dimen11=-\pgfmathresult pt %
            \fi%
            \ifdim\dimen13>0pt %
               \pgfmathpow@{\the\dimen13\@gobbletwo}{.3333333333}%
               \dimen11=\dimexpr\dimen11+\pgfmathresult pt-.33333333333\dimen3\relax%
            \else%
               \pgfmathpow@{\the\dimexpr-\dimen13\relax\@gobbletwo}{.3333333333}%
               \dimen11=\dimexpr\dimen11-\pgfmathresult pt-.33333333333\dimen3\relax%
            \fi%
            \yquant@softpath@extractmaxxat@curveto@checkx%
         \else%
            \ifdim\dimen10=0pt %
               % easiest case, three real roots, two of which are equal:
               % y_1 = 2cbrt(R) - b/3a
               % y_2, x_3 = -cbrt(R) - b/3a
               \ifdim\dimen9>0pt %
                  \pgfmathpow@{\the\dimen9\@gobbletwo}{.3333333333}%
                  \dimen15=\pgfmathresult pt %
               \else%
                  \pgfmathpow@{\the\dimexpr-\dimen9\relax\@gobbletwo}{.3333333333}%
                  \dimen15=-\pgfmathresult pt %
               \fi%
               \dimen11=\dimexpr2\dimen15-.33333333333\dimen3\relax%
               \yquant@softpath@extractmaxxat@curveto@checkx%
               % check the next candidate
               \dimen11=\dimexpr-\dimen15-.33333333333\dimen3\relax%
               \yquant@softpath@extractmaxxat@curveto@checkx%
            \else%
               % nastiest case, three distinct real roots which we can find only by taking a complex-valued cube root.
               % p + i q = cbrt(R + i sqrt(|D|))
               \pgfmathsqrt@{\the\dimexpr-\dimen10\relax\@gobbletwo}%
               \dimen10=\pgfmathresult pt %
               % Let us first find the absolute value
               \dimen12=\dimexpr\dimen9*\dimen9/65535+\dimen10*\dimen10/65535\relax%
               \pgfmathpow@{\the\dimen12\@gobbletwo}{.1666666667}%
               \dimen12=\pgfmathresult pt%
               % then we need 1/3 the argument of R + i sqrt(|D|).
               \pgfmathatantwo@{\the\dimen10\@gobbletwo}{\the\dimen9\@gobbletwo}%
               \dimen13=.3333333333\dimexpr\pgfmathresult pt\relax%
               % and then the real and imaginary parts as cosine and sine.
               \pgfmathcos@{\the\dimen13\@gobbletwo}%
               \dimen14=\dimexpr\pgfmathresult\dimen12\relax%
               \pgfmathsin@{\the\dimen13\@gobbletwo}%
               \dimen15=\dimexpr\pgfmathresult\dimen12\relax%
               % Now the candidates are
               % y_1 = 2p - b/3a
               % y_2 = -p - sqrt(3)q - b/3a
               % y_3 = -p + sqrt(3)q - b/3a
               \dimen11=\dimexpr2\dimen14-.33333333333\dimen3\relax%
               \yquant@softpath@extractmaxxat@curveto@checkx%
               \dimen11=\dimexpr-\dimen14-1.732050808\dimen15-.33333333333\dimen3\relax%
               \yquant@softpath@extractmaxxat@curveto@checkx%
               \dimen11=\dimexpr-\dimen14+1.732050808\dimen15-.33333333333\dimen3\relax%
               \yquant@softpath@extractmaxxat@curveto@checkx%
            \fi%
         \fi%
      \fi%
      % Now after all these calculations, \dimen0 was updated within the group. Make available outside.
      \expandafter%
   \endgroup%
   \expandafter\dimen\expandafter0\expandafter=\the\dimen0  %
   \dimen4=\pgf@xc %
   \dimen6=\pgf@yc %
}

\protected\def\yquant@softpath@extractmaxxat@rectto#1#2\pgfsyssoftpath@rectsizetoken#3#4{%
   % #1: lower left x, #2: lower left y, #3: width, #4: height
   \pgfpointtransformed{\pgfqpoint{#1}{#2}}%
   \pgf@xa=\pgf@x%
   \pgf@ya=\pgf@y%
   \pgfpointtransformed{\pgfqpoint{\dimexpr#1+#3\relax}{\dimexpr#2+#4\relax}}%
   % (\pgf@xa, \pgf@ya) one corner, (\pgf@x, \pgf@y) other corner
   \ifdim\pgf@y>\pgf@ya %
      \unless\ifdim\pgf@ya>\dimen2 %
         \unless\ifdim\pgf@y<\dimen2 %
            \ifdim\pgf@x>\pgf@xa %
               \yquant@softpath@extractmaxxat@update\pgf@x%
            \else%
               \yquant@softpath@extractmaxxat@update\pgf@xa%
            \fi%
         \fi%
      \fi%
   \else%
      \unless\ifdim\pgf@ya<\dimen2 %
         \unless\ifdim\pgf@y>\dimen2 %
            \ifdim\pgf@x>\pgf@xa %
               \yquant@softpath@extractmaxxat@update\pgf@x%
            \else%
               \yquant@softpath@extractmaxxat@update\pgf@xa%
            \fi%
         \fi%
      \fi%
   \fi%
}
